On the Complexity of Verifying Regular Properties on Flat Counter Systems

Among the approximation methods for the verification of counter systems, one of them consists in model-checking their flat unfoldings. Unfortunately, the complexity characterization of model-checking problems for such operational models is not always well studied except for reachability queries or for Past LTL. In this paper, we characterize the complexity of model-checking problems on flat counter systems for the specification languages including first-order logic, linear mu-calculus, infinite automata, and related formalisms. Our results span different complexity classes (mainly from PTime to PSpace) and they apply to languages in which arithmetical constraints on counter values are systematically allowed. As far as the proof techniques are concerned, we provide a uniform approach that focuses on the main issues.

==> mu-pspace-hard.tex <==
We will proof the \pspace-hardness of satisfiability of $\lmc$ formula by a reduction from the emptyness problem of alternating finite automata. The
alternating finite automata we consider are over two alphabets $\aalphabet=\{a,b\}, $and their language is a subset of $a^*b$. The emptiness problem
for these automata are shown to be \pspace-hard. For the reduction, we give an algorithm to construct a $\lmc$ formula $\aformula_{\fsa}$
corresponding to an alternating finite automaton $\fsa$ with $\alang(\fsa)\subseteq \alang(a^* b)$ such that $\aformula$ is satisfiable iff
$\alang(\fsa)$ is non-empty. We also assume, without loss of generality, that the set of states $\states$ of $\fsa=\tuple{\states,\edges,\astate_1,F}$
consists of three disjoint subsets $\states_1$, $\states_2$ and $F$ such that $\astate_1\in\states_1$ and for all state $\astate\in\states_2$,
$\edges(\astate,b)\in F$ and $\edges(\astate,b)=\perp$. Let $\size{\states_1}=N$ and $\states_1=\{\astate_1,\astate_2,\ldots,\astate_N\}$. The
algorithm is presented below.

\begin{algorithm}
\caption{Inputs $\fsa$ Alternating finite automaton}
\label{algo:afa-mu}
\begin{algorithmic}[1]
  \STATE (init):
  \FOR{i=1 to N}
    \STATE $\aformulabis_i=a\wedge\edges(\astate_i,a)[\astate_j\rightarrow \mynext X_j]$ for all $\astate_j\in\states_1$.
    \STATE $\aformulabis_i=a\wedge\edges(\astate_i,a)[\astate_j\rightarrow \mynext b]$ for all $\astate_j\in\states_2$.
  \ENDFOR
  \STATE (substitute):
  \FOR{j=N to 2}
     \STATE $G=\mu X_j \aformulabis_j$
     \FOR{k=1 to i-1}
       \STATE $\aformulabis_k=\aformulabis_k[X_j\rightarrow G]$.
     \ENDFOR
  \ENDFOR
  \STATE return $\mu X_1.\aformulabis_1$.
\end{algorithmic}
\end{algorithm}

We denote by $\fsa_i$ for $i\in[1,N]$, the alternating finite state automaton obtained by replacing $\astate_1$ with $\astate_i$ in $\fsa$. Thus,
$\fsa_1$ is same as $\fsa$.  To prove the correctness of the the formula $\aformula$ returned by Algorithm~\ref{algo:afa-mu}, we will first prove the
following lemma about the section \textbf{(init)} of the algorithm.
\begin{lemma}
After the \textbf{(init)} section of the algorithm, for all $i\in[1,N]$, $\aformulabis_i$ is satisfiable, iff $\alang(\fsa_i)$ is non-empty.
\end{lemma}
\begin{proof}
We will prove this by induction.
\begin{itemize}
  \item [Base Case]: Consider for some $i\in[1,N]$, $\edges(\astate_i,a)$ containes state $\astate'\in \states_2$.
\emph{Here, $\edges(\astate_i,a)$ might contain $X_j$ for some $j$ which we haven't proved anything about. Is this induction hypothesis wrong?}
\end{itemize}
\end{proof}


==> muDef.tex <==
\subsection{Definitions}
For defining linear $\mu$-calculus, we assume a countably infinite set of variables $\varset$. Variables will be typically denoted by
$\avar_1,\avar_2,\ldots$. We also assume the same set of propositional symbols denoted as $\varprop$.  A formula in \defstyle{linear $\mu$-calculus ($\lmc$)} is
constructed as following:
$$
\begin{array}{lcl}
\aformula & ::= & p \mid~ \avar_1 \mid~ \neg \aformula~ \mid~ \aformula \wedge \aformula'~ \mid~ \mynext \aformula~ \mid~ \myprevious\aformula ~\mid~
\mu\avar_1.\aformula(\avar_1) ~\mid~ \nu\avar_1.\aformula(\avar_1)
\end{array}
$$ where $a\in \varprop$ and $\avar_1$ occurs positively in $\aformula(\avar_1)$ in the definition of $\mu\avar_1.\aformula(\avar_1)$ and
$\nu\avar_1.\aformula(\avar_1)$.  The operators $\mu\avar_1.\aformula(\avar_1)$ and $\nu\avar_1.\aformula(\avar_1)$ are called \defstyle{fixpoint
  operator}. For defining the satisfaction relation of a $\lmc$ formula over a word $\aword\in\powerset{\varprop}$, we need a labelling function
$\blabelling:\nat\rightarrow\powerset{\varset}$ which returns the set of propositional variables that are true at the specified position.
$$
\begin{array}{rcl}
%
\aword,i \models_{\blabelling}~ \avarprop & ~\defeq~ & \avarprop \in \aword(i)\\
%
\aword,i \models_{\blabelling}~ \avar_1 & ~\defeq~ & \avar_1\in\blabelling(i) \\
%
\aword,i \models_{\blabelling}~ \mynext \aformula & ~\defeq~ & \aword,i+1 \models_{\blabelling}~ \aformula \\
%
\aword,i \models_{\blabelling}~ \myprevious \aformula & ~\defeq~ & i>0 \mbox{ and } \aword,i-1 \models_{\blabelling}~ \aformula \\
%
\end{array}
$$

For defining the satisfaction of the \defstyle{fixpoint operator}, we need to define some more notions about the labelling function.  For two
labelling functions $\blabelling_1$ and $\blabelling_2$, we say that, $\blabelling_1$ and $\blabelling_2$ \defstyle{agree except on} $\avar$ if for
all $i> 0$ and for all $\avar'\in\varset$ different from $\avar$, $\avar'\in\blabelling_1(i)$ iff $\avar'\in\blabelling_2(i)$. For a given word
$\aword\in\powerset{\varprop}$, a labelling function $\blabelling$, and a formula $\aformula(\avar_1)$ with $\avar_1$ occuring positively in it, we
say that the labelling $\blabelling'$ is a \defstyle{fixpoint} of the equation $\avar_1=\aformula(\equiv)$, $\blabelling$ and $\blabelling'$ agree
except on $\avar_1$ and $\aword,i\models_{\blabelling'}\aformula$ iff $\aword,i\models_{\blabelling'}\avar_1$. $\blabelling'$ is the \defstyle{least}
fixpoint solution if whenever $g$ is also a fixpoint solution then $\aword,i\models_{g}\avar_1$ if $\aword,i\models_{\blabelling'}\avar_1$. On the
other hand, $\blabelling'$ is the \defstyle{greatest} fixpoint solution if whenever $g$ is also a fixpoint solution then $\aword,i\models_{g}\avar_1$
only if $\aword,i\models_{\blabelling'}\avar_1$. Now we can define the satisfaction relation for fixpoint operators as following:
$$
\begin{array}{rcl}
%
\aword,i \models_{\blabelling}~ \mu\avar_1.\aformula(\avar_1) & ~\defeq~ & \aword,i\models_{\blabelling'}\avar_1, where $\blabelling'$ is the least
fixpoint solution of \avar_1=\aformula(\avar_1)\\
%
\aword,i \models_{\blabelling}~ \nu\avar_1.\aformula(\avar_1) & ~\defeq~ & \aword,i\models_{\blabelling'}\avar_1, where $\blabelling'$ is the greatest
fixpoint solution of \avar_1=\aformula(\avar_1)\\
%
\end{array}
$$

Note that for a sentence $\aformula$, the satisfaction of $\aformula$ on $\aword$ at position $i$ does not depend on the labelling function
$\blabelling$. Thus, for a sentence $\aformula$ and a word $\aword$ we say, $\aword,0\models\aformula$ if for some $\blabelling$,
$\aword,0\models_{\blabelling}\aformula$.

We define a \buchi~automaton as usual by the tuple $\bauto=\tuple{\states,\Sigma,\astate_0,\edges,F}$ with a finite set of states $\astate$, a finite
set of alphabets $\Sigma=\powerset{\varprop}$, an initial state $\astate_0\in\states$, a set of final sets $F\subseteq\states$ and the transition
function $\edges\subseteq\states\times\Sigma\times\states$. The set of words accepted by $\bauto$ denoted as
$\languageof{\bauto}\subseteq\Sigma^{\omega}$. For a word $\aword\in\Sigma^{\omega}$, $\aword\in\languageof{\bauto}$ iff the run of $\bauto$ on
$\aword$ visits some state $\astate_f\in F$ infinitely often.

\begin{theorem}\cite{Vardi88}
Given an $\lmc$ sentence $\aformula$, we can construct a \buchi~automaton $\bauto_{\aformula}$ whose number of states is at most exponential in the
size of $\aformula$ such that for any word $\aword\in(\powerset{\varprop})^{\omega}$, $\aword\in\languageof{\bauto_{\aformula}}$ iff
$\aword,0\models\aformula$.
\end{theorem} 



==> proof-lemma-membershi-gen.tex <==
For the proof we present the algorithm described before formally.
\begin{algorithm}
\caption{Inputs $\aspecification$, $\acps=\pair{\cpschema}{\aconstraintsystem}$, $\vect{y}\in[0,\amap_{\mathcal{L}}(\aspecification,\acps)]^{k-1}$}
\label{algo:gen-pspace}
\begin{algorithmic}[1]
  \STATE Let $\bauto_{\aspecification}=\tuple{\states,\aalphabet,\edges,\astate_i,F}$
  \FOR{each $\astate_f\in F$ and each $j\in[1,\length{\aloop_k}]$}
%  \STATE Guess $\astate_f\in F$ and $j\in[1,\length{\aloop_k}]$.
     \STATE Construct $\fsa_1=\tuple{\states,\aalphabet,\astate_0,\edges,\{\astate_f\}}$ and
         $\fsa_2=\tuple{\states,\aalphabet,\astate_f,\edges,\{\astate_f\}}$.  
     \STATE Check $\aseg_1(\aloop_1)^{\vect{y}[1]}\ldots\aseg_{k-1}(\aloop_{k-1})^{\vect{y}[k-1]}\aseg_k\aloop_k[1,j]\in\alang(\fsa_1)$
     \STATE Check $\alang(\fsa_2)\cap\alang(\aloop_k[j+1,\length{\aloop_k}]\aloop_k^{*}\aloop_k[1,j])\neq\emptyset$
     \IF {both the checks return true}
        \STATE return TRUE.
     \ENDIF
  \ENDFOR
  \STATE return FALSE.
\end{algorithmic}
\end{algorithm}

\begin{lemma}
Algorithm~\ref{algo:gen-pspace} returns true iff
$\aword=\aseg_1(\aloop_1)^{\vect{y}[1]}\ldots\aseg_{k-1}(\aloop_{k-1})^{\vect{y}[k-1]}\aseg_k\aloop_k^{\omega}\in\alang(\aspecification)$.
\end{lemma}
\begin{proof}
First observe that by the nice \buchi~ property,
%%Property~\ref{prop}, 
we know that $\aword\in\alang(\aspecification)$ iff $\aword\in\bauto_{\aspecification}$. Thus, in the rest we
will prove that Algorithm~\ref{algo:gen-pspace} returns true iff $\aword\in\alang(\bauto_{\aspecification})$. 

First let us assume that
$\aword=\aseg_1(\aloop_1)^{\vect{y}[1]}\ldots\aseg_{k-1}(\aloop_{k-1})^{\vect{y}[k-1]}\aseg_k\aloop_k^{\omega}\in\alang(\bauto_{\aspecification})$. Thus,
there is an accepting run $\arun\in\edges^{\omega}$ for $\aword$ in $\bauto_{\aspecification}$. According to the \buchi~acceptance condition there exists
a state $\astate_f\in F$ which is visited infinitely often. In $\aword$ only $\aloop_k$ is taken infinitely many times. Thus, $\aloop_k$ being of
finite size, there exists a position $j\in[1,\length{\aloop_k}]$ such that transitions of the form $\astate\labtrans{\aloop_k(j)}\astate_f$ for some
$\astate\in\states$ occurs infinitely many times in $\arun$. Thus, for $\arun$ to be an accepting run, there exists
$\aword'=\alang(\aseg_1(\aloop_1)^{\vect{y}[1]}\ldots\aseg_{k-1}(\aloop_{k-1})^{\vect{y}[k-1]}\aseg_k\aloop_k[1,j])$, which has a run in $\bauto_{\aspecification}$ from
$\astate_i$ to $\astate_f$ and there must exists words $\aword''\in\alang(\aloop_k[j+1,\length{\aloop_k}]\aloop_k^{*}\aloop_k[1,j])$ which has a run
from $\astate_f$ to $\astate_f$. In effect, $\aword'\in\alang(\fsa_1)$ and $\alang(\fsa_{2})\cap\aword''\neq\emptyset$. Thus, there
exists at least one choice of $\astate_f$ and $j$, for which both the checks return true and hence the algorithm returns true.

Now let us assume that the algorithm returns true. Thus, there exists $\astate_f\in F$ and $j\in[1,\length{\aloop_k}]$ such that
$\aword'\in\alang(\fsa_1)$ and $\alang(\fsa_{2})\cap\aword''\neq\emptyset$.
Since, $\alang(\fsa_{2})\cap\aword''\neq\emptyset$, there exists a word
$\aword_1=\aloop_k[j+1,\length{\aloop_k}]\aloop_k^{n}\aloop_k[1,j]\in\alang(\fsa_{loop})$ for some $n$. Consider the word
$\aword_2=\aword'.(\aword_1)^{\omega}$. Clearly, $\aword_2\in\alang(\acps)$. Also, note that $\aword'$ has a run $\arun'$ starting from $\astate_i$ to
$\astate_f$ and $\aword_1$ has a run $\arun''$ starting from $\astate_f$ to $\astate_f$. Thus, we can compose $\arun=\arun'\arun''^{\omega}$ to obtain
a run for $\aword_2$. Note that $\arun$ follows transitions from $\edges$ and visits $\astate_f\in F$ infinitely many times. Thus,
$\aword=\aseg_1(\aloop_1)^{\vect{y}[1]}\ldots\aseg_{k-1}(\aloop_{k-1})^{\vect{y}[k-1]}\aseg_k\aloop_k^{\omega}\in\alang(\bauto_{\aspecification})$.  
\qed
\end{proof}
%\marginpar{\bf Use PSPACE, NP, P etc. only for the complexity of {\em decision} problems.}

\begin{lemma}
Algorithm~\ref{algo:gen-pspace} runs in nondeterministic polynomial space.
\end{lemma}
%% 
\begin{proof}
%% Since, 
%% by Property~\ref{prop},
The proof is standard and we recall standard arguments in the presence
of the nice \buchi~ property.
Indeed, by the nice \buchi~ property, 
$\bauto_{\aspecification}$ can be of exponential size in the size of the input, so we cannot  
construct the transition relation of
$\bauto_{\aspecification}$ explicitly, instead we do it on-the-fly.
%%  Instead we will generate the transitions of $\bauto_{\aspecification}$ using the properties described in
%% Property~\ref{prop} as and when needed. 
Let us consider each step of the algorithm and show that each iteration of the {\bf for} loop 
can be done in polynomial space.
\begin{enumerate}
\itemsep 0 cm 
  \item $\fsa_1$ and $\fsa_2$ are essentially copies of $\bauto_{\aspecification}$ and hence their transition 
  relations are also not constructed
    explicitly. But, 
    by the nice \buchi~ property, 
    %% by Property~\ref{prop}, 
    their states can be represented in polynomial space.
  \item Checking $\aword'\in\alang(\fsa_1)$ can be done by simulating $\fsa_1$ on $\aword'$. Note that for simulating $\fsa_1$, at any position we
    only need to store the previous state and the letter 
    at current position to obtain the next state of $\fsa_1$. Thus, this can be performed in
    polynomial space in $\size{\aspecification}$ and $\size{\acps}+\size{\vect{y}}$.
  \item Checking $\alang(\fsa_2)\cap\alang(\aword'')\neq\emptyset$ can be done by constructing a finite state automata $\fsa_{loop}$ for
    $\alang(\aword'')$ and checking for reachability of final state in the automaton 
     $\fsa_2\times\fsa_{loop}$. Note that $\size{\fsa_{loop}}$ is
    polynomial, but since $\size{\fsa_2}$ is can be of exponential size, 
    $\size{\fsa_2\times\fsa_{loop}}$ can be also of exponential magnitude. 
    However, the graph accessibility problem (GAP) is in \nlogspace, so
    $\alang(\fsa_2)\cap\alang(\aword'')\neq\emptyset$ can also be done in nondeterministic 
    polynomial space.
\end{enumerate}
Thus, the whole procedure can be completed in nondeterministic polynomial space.
%% By Savitch's Theorem, it can be also done in deterministic polynomial space. 
\qed
\end{proof}

By using the above lemmas and applying Savitch's theorem, we obtain that for any $\aspeclanguage$, satisfying the nice BA property, the membership problem for $\aspeclanguage$ is in \pspace.


==> section-ETL.tex <==
\section{Extended Temporal Logic, Alternating B\"uchi Automata}



==> section-automata.tex <==
\section{Automata as Specification}

In this section we will investigate the model-checking problem for different types of automata on both flat Kripke structures and flat counter
systems. 
According to the definitions presented above, we will be in particular looking at the following problems: 
\begin{itemize}
  \item $\mc{FSA}{\flatks}$
  \item $\mc{FSA}{\flatcs}$
  \item $\mc{BA}{\flatks}$
  \item $\mc{BA}{\flatcs}$
\end{itemize}

\subsection{Finite State Automata and \buchi~Automata}
Note that for finite state automata, since they accept only finite words, we will be looking only at finite runs in the system.
First we will provide a construction for synchronous product of a flat Kripke structure and a finite state automaton, such that a word in the language
of the product automaton also yields us a word in the language of the finite state automaton and a path in the Kripke structure. For this purpose, we
assume that the finite state automaton $\fsa$ is defined over the alphabet $\Sigma$ and the labelling function $\alabelling$ of the flat Kripke
structure $\asys$ is defined as $\alabelling:\states \rightarrow \Sigma$. Let us define the construction formally.

Consider a finite state automaton $\fsa$ defined as $\fsa=\tuple{\states,\Sigma,\edges,\astate_i,F}$, a flat Kripke structure
$\asys=\tuple{\states',\edges',\alabelling}$ where $\edges'\subseteq\states'\times\states'$ and $\alabelling:\states' \rightarrow \Sigma$ and an
initial configuration of $\asys$, $\astate'_i$. Note that since $\asys$ is flat, we have a partial ordering on the loops occuring in $\asys$. Let us
assume there are $k$ loops in $\asys$. We pick an arbitrary numbering of the loops such that each loop is identified as $\aloop_i,
i\in\interval{1}{k}$ and if there is a path from $\aloop_i$ to $\aloop_j$ then $i<j$. We denote the synchronous product of $\fsa$ and $\asys$ along
with sets $\hat{\states'}\subseteq\states'$ and $\hat{F}\subseteq F$ as
$\fsa\times\asys=\tuple{\states\times\states',\Sigma',(\astate_i,\astate'_i),\tilde\Delta,\tilde F}$, where
$\Sigma'=\Sigma\times\{t_1,t_2,\ldots,t_k,\epsilon\}$ where $\{t_1,t_2,\ldots,t_k\}$ are additional propositional symbols such that
$\{t_1,t_2,\ldots,t_k\}\cap\Sigma=\emptyset$, and $\tilde\Delta\subseteq(\states\times\states')\times\Sigma'\times(\states\times\states')$. A
transition $(\tuple{\astate_1,\astate'_1}\labtrans{a,t}\tuple{\astate_2,\astate'_2})\in\tilde\Delta$ iff:
\begin{enumerate}
%  \item $\astate_1,\astate_2\in\states$, $\astate'_1,\astate'_2\in\states'$, $a\in \Sigma$
  \item $\tuple{\astate_1,a,\astate_2}\in\edges$.
  \item $\tuple{\astate'_1,\astate'_2}\in\edges'$.
  \item If $\tuple{\astate'_1,\astate'_2}=\aloop_i(0)$ for any $i\in [1,k]$, then $t=t_i$ otherwise $t=\epsilon$.
  \item $a=\alabelling(\astate'_1)$.
  \item $\tilde F=\hat{F}\times\hat{\states'}$.
\end{enumerate}
The acceptance condition of $\fsa\times\asys$ is same as that of finite state automaton. The product is thus, a finite state automaton.  Since,
$\fsa\times\asys$ is defined over the alphabet $\Sigma'=\Sigma\times\{t_1,t_2,\ldots,t_k,\epsilon\}$, we obtain that
$\languageof{\fsa\times\asys}\subseteq\Sigma'^{*}$. We define as before, for $a'\in\Sigma'$, $\pi_1(a')\in\Sigma$ and
$\pi_2(a')\in\{t_1,t_2,\ldots,t_k,\epsilon\}$. We extend the projection operator for alphabets to words as : for $\aword'\in\Sigma'^{*}$ with
$\length{\aword'}=n$, we have $\pi_1(\aword')=\pi_1(\aword'(1)).\pi_1(\aword'(2))\ldots\pi_1(\aword'(n))=\aword\in\Sigma^{*}$.  Note that the
construction only deals with the underlying structure of $\fsa$ and $\asys$. Hence, we can perform similar kind of product with \buchi~automaton,
since a \buchi~automaton differs from a finite state automaton in only the acceptance condition. Thus, for a given \buchi~automaton, $\bauto$, and a
flat Kripke structure, $\asys$, $\bauto\times\asys$ is a \buchi~automaton. Also, it is possible to perfom the same kind of operation with path schemas
and flat counter system by ignoring guards and updates. Now we will prove some features of the construction.

\begin{lemma}
\label{product-automata}
Given $\aword'\in(\Sigma')^{*}$, $\aword'\in\languageof{\fsa\times\asys}$ iff the following two conditions are true
\begin{enumerate}
\item[I.] Let $\arun\in(\states\times\states')^*$ be the sequence of states, visited in the accepting run of $\aword'$. Then $\pi_2(\arun)$ is a path
  in $\asys$ ending with a state in $\hat{\states'}$
\item[II.] $\pi_1(\aword')\in\languageof{\fsa}$ and the accepting run of $\pi_1(\aword')$ in $\fsa$ ends in a state in $\hat{F}$
\end{enumerate}
\end{lemma}
\begin{proof}
Consider any word $\aword'\in\languageof{\fsa\times\asys}$. Let us assume that the accepting run for $\aword'$ in $\fsa\times\asys$ be
$$
\arun'= \pair{\astate_1}{\astate'_1}\labtrans{\aword'(1)}\pair{\astate_2}{\astate'_2}\labtrans{\aword'(2)}\cdots\labtrans{\aword'(n)}\pair{\astate_n}{\astate'_n}
$$ 
where $\astate_1=\astate_i$, $\astate'_1=\astate'_i$, $\astate_n\in \hat{F}$ and $\astate'_n\in\hat{\states'}$. Note that by condition (2), in the
construction of $\fsa\times\asys$,
$$
\arun''= \astate'_1\labtrans{}\astate'_2\labtrans{}\cdots\labtrans{}\astate'_n
$$ 
is a path in $\asys$ starting with the given initial state $\astate'_i$ and ending in $\astate'_n\in\hat{\states'}$. Similarly, note that according
to condition (1) in the construction,
$$
\arun= \astate_1\labtrans{\pi_1(\aword'(1))}\astate_2\labtrans{\pi_1(\aword'(2))}\cdots\labtrans{\pi_1(\aword'(n))}\astate_n
$$ 
is a run in $\fsa$. Since $\astate_1=\astate_i$, and $\astate_n\in \hat{F}\subseteq F$, $\arun$ is indeed an accepting run in $\fsa$. Thus,
$\pi_1(\aword')\in\languageof{\fsa}.$ with a run ending in a state in $\hat{F}$.

For the other side, assume that there exists a word $\aword'\in(\Sigma')^{*}$, such that both the conditions (I) and (II) are satisfied. Since,
condition (II) is satisfied, we know we have an accepting run $\arun$ in $\fsa$ for the word $\pi_1(\aword')$. Let
$$
\arun= \astate_1\labtrans{\pi_1(\aword'(1))}\astate_2\labtrans{\pi_1(\aword'(2))}\cdots\labtrans{\pi_1(\aword'(n))}\astate_n
$$
be the run in $\fsa$. Since, it is an accepting run, $\astate_1=\astate_i$ and $\astate_n\in \hat{F}\subseteq F$.
Again, since condition (I) is satisfied by $\aword'$ and by construction we have the path 
$$
\arun'= \astate'_1\labtrans{}\astate'_2\labtrans{}\cdots\labtrans{}\astate'_n
$$
in $\asys$ such that $\pi_1(\aword'(j))=\alabelling(\astate'_j)$ for all $j\in[1,n]$ and $\astate'_1=\astate'_i$ and $\astate'_n\in\hat{\states'}$. Combining $\arun$ and $\arun'$, we get the run,
$$
\arun''= \pair{\astate_1}{\astate'_1}\labtrans{\aword'(1)}\pair{\astate_2}{\astate'_2}\labtrans{\aword'(2)}\cdots\labtrans{\aword'(n)}\pair{\astate_n}{\astate'_n}
$$ 
Note that by construction of $\fsa\times\asys$, $\arun''$ is a run in $\fsa\times\asys$ as it follows $\tilde\delta$. Since, the first state of the
run is the initial state of the automaton, $\pair{\astate_1}{\astate'_1}=\pair{\astate_i}{\astate'_i}$ and $\pair{\astate_n}{\astate'_n}\in\tilde F$,
$\arun''$ is an accepting run. Hence, $\aword'\in\languageof{\fsa\times\asys}$.
\end{proof}

Observe that given $\fsa$ and $\asys$, the time required to construct $\fsa\times\asys$ is at most $\size{\fsa}\times\size{\asys}$. This is due to the
fact that the states of $\asys$ and the transitions of $\fsa$ are labelled with same alphabet $\Sigma$ and for each of the transitions of $\fsa$ it
requires at most one iteration of the set of transitions in $\asys$. Thus, the construction can be in fact done in time which is polynomial in the
size of the input. Also, note that $\size{\fsa\times\asys}$ is atmost $\size{\fsa}\times\size{\asys}$.

\begin{lemma}
$\mc{FSA}{\flatks}$ is in \ptime.
\end{lemma}
\begin{proof}
Given a finite state automata $\fsa$ and a flat Kripke structure, $\asys$ and an initial position $\astate'_i$ in $\asys$, the \ptime algorithm
proceeds by computing $\fsa\times\asys$ with the final state sets $\hat{\states'}=\states'$ and $\hat{F}=F$. As observed previously, $\fsa\times\asys$ is
a finite state automaton. The algorithm then performs the emptiness checking on the product automaton and outputs the result.

The construction of $\fsa\times\asys$ takes time atmost $\size{\fsa}\times\size{\asys}$ and the emptiness checking of finite state automaton takes
time at most $(\size{\fsa}\times\size{\asys})^2$. Thus, the total time taken by the algorithm is polynomial in the size of the input. Now lets check
the correctness of the algorithm.

First note that, since flat Kripke structure does not have any guards and updates on the transition, a path in the Kripke structure is also a run in
the flat Kripke structure. By Lemma~\ref{product-automata}, we know that the existence of a word $\aword'\in\languageof{\fsa\times\asys}$, implies
that there exists a run (or path) $\arun$ in $\asys$, such that $\blabelling(\statesof{\arun})\in\languageof{\fsa}$ and vice-versa. Thus, the \ptime~
algorithm described above returns true iff there exists a run $\arun$ in $\asys$ such that $\blabelling(\statesof{\arun})\in\languageof{\fsa}$.  \qed
\end{proof}

Since, \buchi~automata differs from finite state automta in only the acceptance condition, we can apply the above \ptime~algorithm for the problem $\mc{BA}{\flatks}$
also, with the exception being that the emptiness checking procedure performed on the product automaton is that of \buchi~automaton emptiness checking.

Given a \buchi~automaton $\bauto$, and a flat Kripke structure $\asys$, and an initial position $\astate'_i$ in $\asys$, we first construct
$\bauto\times\asys$ with the final state sets $\hat{\states'}=\states'$ and $\hat{F}=F$. As stated earlier, $\bauto\times\asys$ has a
\buchi~acceptance condition and hence the product automaton is a \buchi~automaton. The algorithm then proceeds by applying the \ptime~algorithm for
emptiness checking for \buchi~automaton on the product automaton and return the result. The proof that it returns true iff there exists a run $\arun$
in $\asys$ such that $\blabelling(\statesof{\arun})\in\languageof{\bauto}$ proceeds similarly as in the case of finite state automata. Thus, we have that

\begin{lemma}
$\mc{BA}{\flatks}$ is in \ptime.
\end{lemma}

Now, we will look at the case with counters. But, instead we will first provide a \np~algorithm for path schemas from flat counter system.  The
algorithm starts by computing a system of linear equations $\aconstraintsystem$, which characterizes the runs respecting the the path schema
$\aschema$ and are also, valid with respect to the counter values, updates and guards. The equations have $k-1$ variables, $k$ being the number of loops
in $\aschema$. A solution $(m_1,m_2,\cdots,m_{k-1})$ of $\aconstraintsystem$ corresponds to a run in $\aschema$ where $\aloop_i$ is taken exactly $m_i$
times for all $i\in[1,k]$. Let us show that the construction of $\aconstraintsystem$ can be done in polynomial time.
\begin{theorem}\cite{DemriDharSangnier12}
\label{thm:constraint}
Let $\aschema$ be a path schema from a flat counter system $\asys$, then the constraint system $\aconstraintsystem$ characterizing the valid runs in
$\aschema$ has
\begin{itemize}
  \item $k-1$ variables.
  \item at most $\length{\aschema}\times 2 \times\size{\aschema}^2$ conjuncts
  \item the greatest absolute value of the constants are bounded by $2n\times K(K+2)\times(\length{\aschema}+1)$, where $K$ is the maximum absolute
    value of the constants occurring in $\aschema$.
\end{itemize}
\end{theorem}

The algorithm then proceeds by constructing a formula $\aformula$ with $k-1$ variables for the Parikh image of a language such that the solutions
corresponds to the runs $\arun$ for which $\blabelling(\statesof{\arun})\in\languageof{\fsa}$. The theorem below states that formula characterizing
the Parikh image of a language of a finite state automaton can be constructed efficiently.
\begin{theorem}\cite{Verma&Seidl&Schwentick05}
\label{thm:parikh}
Given a finite state automaton $\fsa$, let $\aformula$ be the exsistential Presburger formula characterizing the Parikh image of $\languageof{\fsa}$. $\aformula$
can be
\begin{itemize}
  \item constructed in time bounded by $\size{\fsa}^{2}$.
  \item the greatest absolute value of the constant in $\aformula$ is bounded by $\size{\fsa}$.
\end{itemize}
\end{theorem}
At last, it tries to find a solution to the conjunction of $\aformula$ and $\aconstraintsystem$. In effect, of all the solutions of
$\aconstraintsystem$ (which can also be thought of as runs in the system), the conjunction is satisfied only by the solutions (or runs) that also
satisfies the condition of the problem. Then, the algorithm non-deterministically selects a solution and checks whether
$\aconstraintsystem\wedge\aformula$ is satisfiable or not. The following theorem shows that $\aconstraintsystem\wedge\aformula$ admits a small
solution.
\begin{theorem}\cite{DemriDharSangnier12}
\label{thm:small-sol} 
Given $\aschema$ from $\asys$ and $\fsa$, if $\aconstraintsystem$ characterizes the valid runs in $\aschema$ and $\aformula$ characterizes the Parikh
image of a projection of $\languageof{\fsa}$, then $\aconstraintsystem\wedge\aformula$ has a solution iff $\aconstraintsystem\wedge\aformula$ has a solution where the
value of each variable is bounded by $2^{p(\size{\aschema})}$ for some polynomial $p(\cdot)$.
\end{theorem}

The algorithm is presented formally in Algortihm~\ref{algo:fsa-cps}. The algorithm is given as input a path schema $\aschema$ representing finite runs
in a flat counter system $\asys=\tuple{\states',\counters,\edges',\alabelling}$, a finite state automaton,
$\fsa=\tuple{\states,\Sigma,\edges,\astate_i,F}$ and two sets of final states one from $\aschema$, $\hat{\states'}\subseteq\states'$ and the other
from $\fsa$, $\hat{F}\subseteq F$. 
%It is worth mentioning here that, without loss of geneality, we can assume that $\aschema$ does not have any
%disjunction in the guards of the transitions, as the disjunction in the guards can be removed by polynomial size guesses using the procedure described
%in \cite{DemriDharSangnier12}.

\begin{algorithm}
\caption{Inputs $\aschema$, $\fsa$, $\hat{\states'}$,$\hat{F}$}
\label{algo:fsa-cps}
\begin{algorithmic}[1]
  \STATE Construct the system of linear equations $\aconstraintsystem$  with variables $\avariable_1,\avariable_2,\cdots,\avariable_{k-1}$ characterizing the runs in the path schema $\aschema$ (assuming $\aschema$ contains $k-1$ loops).
  \STATE Construct the synchronous product, $\aschema\times\fsa$ with the sets of final states, $\hat{\states'}$,$\hat{F}$ for $\aschema$ and $\fsa$ respectively.
  \STATE Construct $\aformula$  with variables $\avariable_1,\avariable_2,\cdots,\avariable_{k-1}$ characterizing the Parikh images of $\pi_2(\languageof{\aschema\times\fsa})$.
  \STATE Guess $\vect{y}\in[1,2^{P(\size{\aschema}+\size{\aformula})}]^{k-1}$.
  \STATE Check whether $\vect{y}\models\aconstraintsystem\wedge\aformula$.
\end{algorithmic}
\end{algorithm}
\begin{lemma}
Algorithm~\ref{algo:fsa-cps} returns true iff there exists a valid run $\arun$ respecting $\aschema$ ending in a state $\astate'\in\hat{\states'}$, such
that there exists an accepting run of $\blabelling(\statesof{\arun})$ ending in a state $\astate\in\hat{F}$.
\end{lemma}
\begin{proof}
First let us assume that Algorithm~\ref{algo:fsa-cps} returns true. Thus, $\aconstraintsystem\wedge\aformula$ is satisfiable. Consider the solution to
be $\vect{y}$. Thus, $\vect{y}$ is a solution to both $\aconstraintsystem$ and $\aformula$. Since, $\vect{y}$ represent the number of times each loop
$\aloop_i$ of $\aschema$ is taken, we get an unique run $\arun$, from the solution $\vect{y}$. Since $\vect{y}$ satisfies $\aconstraintsystem$,
$\arun$ is a valid run respecting $\aschema$. Also, since, $\vect{y}$ satisfies $\aformula$, we know that $\languageof{\aschema\times\fsa}$ is
non-empty. By Lemma~\ref{product-automata}, , this implies that there exists a run $\arun'$ in $\aschema$, such that
$\blabelling(\statesof{\arun'})\in\languageof{\fsa}$. Thus, to check that the run is valid with respect to counters, we need to make sure that
$\arun'=\arun$. Note that $\pi_2(\languageof{\aschema\times\fsa})\subseteq\{t_1,t_2\cdots,t_{k-1},\epsilon\}^{*}$. Also, note that by construction,
for any word $\aword\in\languageof{\aschema\times\fsa}$, the number of times $t_i$ for $i\in[1,k-1]$, appears in $\pi_2(\aword)$ is exactly the number
of times loop $\aloop_i$ is taken in realizing $\pi_1(\aword)$. Since, $\aformula$ is constructed on $\pi_2(\aschema\times\fsa)$ and $\vect{y}$
satisfies $\aformula$, we have that $\blabelling(\statesof{\arun})\in\languageof{\fsa}$.

For the other side let us assume, there exists a run $\arun$ respecting $\aschema$ and ending in $\astate'\in\hat{\states'}$, such that there exists
an accepting run of $\blabelling(\statesof{\arun})$ ending in a state $\astate\in\hat{F}$. Thus, $\languageof{\aschema\times\fsa}\neq\emptyset$. By
the previous arguement, $iter_p(\wordof{\arun})$ satisfies $\aformula$. Since, $\arun$ is also a valid run, $iter_p(\wordof{\arun})$ also satisfies
$\aconstraintsystem$. Thus, $\aconstraintsystem\wedge\aformula$ is satisfiable. Thus, the algorithm returns true.
\qed
\end{proof}

\begin{lemma}
Algorithm~\ref{algo:fsa-cps} is in \np.
\end{lemma}
\begin{proof}
First note that the single guess in the algorithm is $\vect{y}$ is of polynomial size, since their components have values bounded by some exponential
expression and can be represented using polynomially many bits.

Now let us verify that all the checks are done in polynomial time too.
\begin{itemize}
\item According to Theorem~\ref{thm:constraint}, the number of conjuncts in $\aconstraintsystem$, is bounded by a polynomial in
  $\size{\aschema}^2$. Construction of each conjunct requires at most one pass of $\aschema$. Hence, the time required for building
  $\aconstraintsystem$ is at most $\size{\aschema}^3$.
\item Construction of $\aschema\times\fsa$ takes time at most $\size{\aschema}\times\size{\fsa}$.
\item Computing the projection $\pi_2(\languageof{\aschema\times\fsa})$, requires only applying $\pi_2$ for every transition label in
  $\aschema\times\fsa$. Thus, by Theorem~\ref{thm:parikh}, the time required to build $\aformula$ is at most $\size{\fsa}^2$.
\item Finally, $\vect{y}\models\aconstraintsystem\times$ can be checked in polynomial time since the values of $\vect{y}$ are of exponential magnitude
  and the combined constraint system is of polynomial size.
\end{itemize}
\qed
\end{proof}

Note that, for the general problem of $\mc{FSA}{\cps}$, since the run can end at any state of the path schema, and the finite state automaton can
accept by any of its accepting states, we can use the same algorithm as above. For a given path schema $\aschema$ in a flat counter system
$\asys=\tuple{\states',\counters,\edges',\alabelling}$, a finite state automaton, $\fsa=\tuple{\states,\Sigma,\edges,\astate_i,F}$, we run
Algorithm~\ref{algo:fsa-cps} with inputs $\aschema$, $\fsa$ and the two sets of final states as $\states'$, $F$ respectively. Clearly, this gives a
\np~algorithm for the problem.
\begin{lemma}
$\mc{FSA}{\cps}$ is in \np.
\end{lemma}
The \np-Hardness of the problem can be established by a reduction from the satisfiability problem.
\begin{lemma}
$\mc{FSA}{\cps}$ is \np-Hard.
\end{lemma}
\begin{proof}
The proof is by reduction from the problem SAT. Let $\aformula$ be a Boolean formula in CNF, built over the propositional variables in
$AP=\{p_1,\cdots,p_n\}$. Let $\aformula=H_1\wedge H_2\wedge\cdots\wedge H_m$ where each $H_i=l^1_i\vee l^2_i\vee l^3_i$. Here each $l^j_i$ is either
$p_k$ or $\neg p_k$ for $k\in[1,n]$. We build a path schema $\aschema\in\cps$, an initial configuration $\aconf_0$ (all counters will be equal to
zero) and an automaton $\fsa$, such that there exists a run $\arun$, where $wrd(\arun)\in\languageof{\fsa}$ and $wrd(\arun)$ is a prefix of a word in
$\languageof{\aschema}$ iff $\aformula$ is satisfiable. The path schema $\aschema$ and $\fsa$ is as described in Figure~\ref{fig:nphard-schema}. We
have $2n$ counters and one loop for each counter. The true valuation of the propositional variable $p_i$ is encoded by the fact that the loop
incrementing counter $x_i$ is visited twice and the loop incrementing $x'_i$ is visited once. If $p_i$ has a valuation of false is encoded by the fact
that $x_i$ is incremented to $1$ and $x'_i$ is incremented to $2$. The guard $\aguard$ is defined as a formula that establishes the correspondence
between the truth value of $p_i$ and the number of times the loop incrementing $x_i$ or $x'_i$ is visited. First we define the formulas for
$i\in[1,m]$, $C_i=var(l^1_i)+var(l^2_i)+var(l^3_i)$ where $var(l^j_i)=x_k$ if $l^j_i=p_k$ and $var(l^j_i)=x'_k$ otherwise.
$$
\aguard=\wedge^n_{i=1}1\leq x_i\leq 2\wedge\wedge^n_{i=1}1\leq x'_i\leq 2\wedge\wedge^n_{i=1}x_i+x'_i=3\wedge\wedge^m_{i=1}C_i> 3
$$ The first two parts ensures that the loops are taken either once or twice. The next part of $\aguard$ ensures that the loops corresponding to $x_i$
and $x'_i$ are taken in such way that only one of them is $2$. The last part guard ensures that each of the $m$ clauses are satisfied and within each
clause at least one of the literal is true.
\begin{figure}
\label{fig:nphard-schema}
\input{nphard_reach.tikz}
\end{figure}
\begin{figure}
\label{fig:nphard-fsa}
\input{nphard_fsa.tikz}
\end{figure}
Let us check the correctness of the reduction. It is clear from the construction that the automaton $\fsa$ checks for reachability of the state
$\astate_f$ in the path schema. That is, for any run $\arun$ respecting $\aschema$, it is easy to see that $wrd(\arun)\in\languageof{\fsa}$ iff
$\arun$ reaches $\astate_f$. So, in effect we have to check that $\astate_f$ is reachable in $\aschema$ iff $\aformula$ is satisfiable.

Let $v:AP\rightarrow{\top,\perp}$ be a valuation satisfying $\aformula$. Let us consider the run $\arun$ respecting $\aschema$ such that
$\loopsof{\aschema}{\arun}[i] = 2$, if $v(p_i) = \top$ for $i\in[1,n]$ and $\loopsof{\aschema}{\arun}[i] = 1$ for $i\in[n+1,2n]$. Otherwise
$\loopsof{\aschema}{\arun}[i] = 1$ for all $i\in[1,n]$ and $\loopsof{\aschema}{\arun}[i] = 2$ for $i\in[n+1,2n]$. It is easy to check that the guard
$\aguard$ is satisfied by the run $\arun$. Hence the state $\astate_f$ is reachable. Conversely, if there is a run $\arun$ respecting $\aschema$ and
starting with configuration $\aconf_0$ such that it visits $\astate_f$, then the guard $\aguard$ ensures that the valuation $v$ satisfies $\aformula$
where for all $i\in [1,n]$ ,we have $v(p_i)=\top \defeq \loopsof{\aschema}{\arun}[i]\geq 2$.  \qed
\end{proof}
Thus, from the previous lemmas we have that,
\begin{theorem}
$\mc{FSA}{\cps}$ is \np-Complete.
\end{theorem}
We know that, there are finitely many path schemas in a flat counter system and every run in the counter system follow one of such path schemas.
% Also,presented in \cite{DemriDharSangnier12}, there is a \np~procedure to eliminate the disjunction in the guards of such path schema.
Thus, we can non-deterministically select a path schema and apply the \np~procedure for $\mc{FSA}{\cps}$, which gives us a
\np~algorithm for deciding $\mc{FSA}{\flatcs}$.
\begin{theorem}
$\mc{FSA}{\flatcs}$ is \np-Complete.
\end{theorem}
Since \buchi~automata are finite state automata with different acceptance condition, the above procedure can also be applied in the case of
$\mc{BA}{\cps}$ with a little modification to allow $\omega$-words. Consider an accepting run over the word $\aword$ in a \buchi~automaton. The word
can be split into two parts $\aword',\aword''\in\Sigma^{*}$ with $\aword=\aword'.(\aword'')^{\omega}$ such that $\aword'$ has a run from an initial
state $\astate_i$ to a final state $\astate_f$ and $\aword''$ has a run from $\astate_f$ to $\astate_f$.  The algorithm proceeds by guessing such
break up of the accepting run of a $\omega$-word in the language of \buchi~automaton. It then considers the \buchi~automaton as finite state automaton
and performs Algorithm~\ref{algo:fsa-cps} on both parts of the run to check the validity of the runs with respect to the counters in path schema.

The algorithm is presented formally in Algortihm~\ref{algo:bauto-cps}. The algorithm is given as input a path schema $\aschema$ in a flat counter system
$\asys=\tuple{\states',\counters,\edges',\alabelling}$, a \buchi~automaton $\bauto=\tuple{\states,\Sigma,\edges,\astate_i,F}$.

\begin{algorithm}
\caption{Inputs $\aschema$, $\bauto$}
\label{algo:bauto-cps}
\begin{algorithmic}[1]
  \STATE Guess a state $\astate_f\in F$ of $\bauto$ and a position $j$ in $\aloop_k$(last loop) of $\aschema$.
  \STATE Run Algorithm \ref{algo:fsa-cps} with input $\aschema'=\aseg_1 \aloop_1^+ \cdots \aseg_k \aloop_k^+\aloop_k[1,j]$, $\bauto$, and the two sets of final states as $\{\aloop_k(j)\}$, $\{\astate_f\}$ respectively. Here we change the accepting condition of $\bauto$ to consider it as a finite state automaton.
  \IF {Algorithm \ref{algo:fsa-cps} returns false}
      \STATE ABORT.
  \ENDIF
  \STATE Run Algorithm \ref{algo:fsa-cps} with input $\aschema''=\aloop_k[j,\length{\aloop_k}].\aloop_k^{+}\aloop_k[1,j]$, $\bauto_{\astate_f}$ and the two sets of final states as $\{\aloop_k(j)\}$, $\astate_f$ respectively. Also, change the acceptance condition of $\bauto$ to consider it as a finite state automaton.
  \IF {Algorithm \ref{algo:fsa-cps} returns true}
      \STATE return true.
  \ELSE
      \STATE ABORT.
  \ENDIF  
\end{algorithmic}
\end{algorithm}
Clearly, it is in \np, as the algorithm performs two guesses on states of the given input structures and two calls to the \np~algorithm,
Algorithm~\ref{algo:fsa-cps}. It remains to prove the correctness of the algorithm.
\begin{lemma}
\label{lemma:fsa-cps-correct}
Algorithm~\ref{algo:bauto-cps} return true iff there exists an infinite valid run $\arun$ respecting $\aschema$ such that,
$\blabelling(\statesof{\arun})\in\languageof{\bauto}$.
\end{lemma}
\begin{proof}
Let us assume that the algorithm returns true. This implies that both the calls to Algorithm~\ref{algo:fsa-cps} returns true. Let the guessed states
in $\aschema'$ be $\aloop_{k}(j)$ and the guessed state from $\bauto$ be $\astate_f$. Since the first call to Algorithm~\ref{algo:fsa-cps} returned
true, by Lemma~\ref{product-automata}, we know that, there exists a run $\arun'$ respecting $\aschema'$ and ending in $\aloop_{k}(j)$, such that,
$\blabelling(\statesof{\arun'})$ has an accepting run in $\bauto$ which starts from $\astate_i$ and ends in $\astate_f$. Similarly, since the second
call to Algorithm~\ref{algo:fsa-cps} returned true, again by Lemma~\ref{product-automata}, we know that, there exists a run $\arun''$ respecting the path
schema $\aschema''=\aloop_k[j,\length{\aloop_k}].\aloop_k^{+}\aloop_k[1,j]$ (iterations of the last loop) which starts and ends at $\aloop_{k}(j)$, such that,
$\blabelling(\statesof{\arun''})$ has a run in $\bauto$ which statrts from $\astate_f$ and ends in $\astate_f$. Both the runs are valid with respect
to the counter values as they satisfy $\aconstraintsystem$ in both the calls to Algorithm~\ref{algo:fsa-cps}. Now consider the infinite run,
$$
\arun=\arun'.\arun''.\arun''.\arun''\cdots
$$ 
Clearly, $\aword=\blabelling(\statesof{\arun})$ has an accepting run in $\bauto$ as the run starts from $\astate_i$ and visits $\astate_f$
inifinitely often.  Again, $\arun'$ repects $\aschema$ but ends in $\aloop_k(j)$ whereas all subsequent runs $\arun''$ starts from $\aloop_k(j)$ stays
in $\aloop_k$ and ends in $\aloop_k(j)$ from where the next copy of $\arun''$ starts. Thus, $\arun$ is indeed an infinite run respecting
$\aschema$. Since $\aloop_k$ in $\aschema$ has to be taken infinitely many times (which is ensured by the constraint system), we can join infinite
copies of $\arun''$ as they stay only within $\aloop_k$. $\arun$ is valid with respect to the counter values in $\aschema$.
 
Now, let us assume that there exists an infinite run $\arun$ respecting $\aschema$ such that $\blabelling(\statesof{\arun})\in\languageof{\bauto}$. First note that by the
conditions of $\aschema$, $\arun$ takes $\aloop_k$ infinitely many times. Also, by the acceptance condition of $\bauto$, for some $\astate_f\in F$,
$\astate_f$ occurs infinitely often in the accepting run of $\blabelling(\statesof{\arun})$. Since, there are only finitely many outgoing edges from any
$\astate_f\in F$ in $\bauto$, there should be at least one such outgoing edge with label $a\in\Sigma$, which is taken infinitely many times. Since only,
the finitely many nodes of $\aloop_k$ appears infinitely many times in $\arun$, there should be some node $\aloop_k(j)$ with
$\alabelling(\aloop_k(j))=a$, which is considered after  $\astate_f$ in $\bauto$. Let us partition $\arun$ into parts according to the nodes
$\aloop_k(j)$ which corresponds to $\astate_f$ in $\bauto$. we have,
$$
\arun=\arun'.\arun''_1.\arun''_2.\arun''_3\cdots
$$ 
First note that, $\arun''_1=\arun''_2=\arun''_3=\cdots$, as it essentially visits the same loop $\aloop_k$ an equal number of times. Now, by
construction of the partitions of $\arun$, $\arun'$ is a valid run in $\aschema$ which starts from the initial position and ends at $\aloop_k(j)$ and
$\blabelling(\statesof{\arun'})$ has a run in $\bauto$ starting from $\astate_i$ and ending in $\astate_f$. Thus, assuming the non-deterministic guess
to be correct, the first call to Algorithm~\ref{algo:fsa-cps} returns true. Also, $\arun''$ is a run in $\aschema$ which starts from $\aloop_k(j)$ and
ends in $\aloop_k(j)$ staying only within $\aloop_k$. $\blabelling(\statesof{\arun''})$ has a run from $\astate_f$ to $\astate_f$ in $\bauto$. Thus,
the second call to Algorithm~\ref{algo:fsa-cps} also returns true. Thus, the algorithm return true.  
\qed
\end{proof}
Thus, by the previous algorithm and the \np-Hardness of $\mc{FSA}{\cps}$, we can conclude,
\begin{theorem}
$\mc{BA}{\cps}$ is \np-Complete.
\end{theorem}

\subsection{The Curious Case of n-\buchi~Automata}

For n-\buchi~automata, we define the problem $\mc{n-BA}{\csfrag}$, as:
\begin{description}
\itemsep 0 cm 
\item[Input:] A counter system or its fragment $\asys$, a configuration $\aconf_0$ and $n$ \buchi~automata,
  $\bauto_1,\bauto_2,\cdots,\bauto_n$;
\item[Output:] Does there exist a finite run $\arun$ starting from $\aconf_0$, such that
  $\blabelling(\statesof{\arun})\in\languageof{\bauto_1\cap\bauto_2\cap\cdots\cap\bauto_n}$?
\end{description}

Unlike the previous two cases of finite state automata and \buchi~automata, no \ptime~algorithm is known for the problem $\mc{n-BA}{\flatks}$. It
is infact, \np-Hard.
\begin{lemma}
\label{nBA-np-hard}
$\mc{n-BA}{\flatks}$ is \np-hard.
\end{lemma}
\begin{proof}
The proof is by a reduction from the problem SAT. Let $\aformula$ be a Boolean formula built over the propositional variables
$\{\avarprop_1,\avarprop_2,\cdots,\avarprop_n\}$. We build a flat Kripke structure $\asys$ with an initial configuration and $m$ \buchi~automata such
that $\aformula$ is satisfiable iff there is a run in $\asys$ starting from the initial configuration such that the word formed from the labellings of
the states of the run is in $\languageof{\bauto_1\cap\bauto_2\cap\cdots\cap\bauto_m}$. The flat Kripke structure $\asys$ is the one described in
Figure~\ref{fig:nphardness} so that the truth of the propositional variable $\avarprop_i$ is encoded by the fact that the loop containing $\astate_i$
is visited at least once.
\begin{figure}
  \begin{center}
    \input{nphard.tikz}
  \end{center}
  \caption{A flat Kripke structure $\asys$}
  \label{fig:nphardness}
\end{figure}
Note that the labels of the states in $\asys$ are from the set, $\{\astate_i,\astate_1,\cdots,\astate_n,\astate_f\}$. Hence for the automata that we
will construct, the alphabet is assumed to be $\Sigma=\{\astate_i,\astate_1,\cdots,\astate_n,\astate_f\}$. Let $\aformula$ be in CNF. Thus,
$\aformula=\wedge_{i\leq m}(H_i)$, where $H_i$ are the clauses of the form $(l^1_i\vee l^2_i\vee l^3_i)$. Each literal $l^j_i$ can be either $p_k$ or
$\neg p_k$. We will have $m$ \buchi~automata, one for each clause $H_i$. The automata $\bauto_i$ for $H_i=(l^1_i\vee l^2_i\vee l^3_i)$ is defined as
in Figure~\ref{fig:clause}.
\begin{figure}
  \begin{center}
    \input{clause.tikz}
  \end{center}
  \caption{A \buchi~automaton for clause $H_i=(l^1\vee l^2\vee l^3)$}
  \label{fig:clause}
\end{figure}
The automata for any literal $\fsa_l$ is defined as in Figure~\ref{fig:literal}. Each of the automaton actually checks whether the corrsponding loop
in $\asys$ is visited or not.
\begin{figure}
  \begin{center}
    \input{literal.tikz}
  \end{center}
  \caption{A \buchi~automaton for literal $l$ related to $\avarprop_j,j\in[1,n]$}
  \label{fig:literal}
\end{figure}

Intuitively, each automaton represents one clause and by definition of the problem, each of the automata has to accept, i.e. all the clauses have to
satisfy. Each clause automaton selects one of the literal automaton non-deterministically and check that the literal is satisfied. The
non-deterministic choice encodes the disjunction of the formula.

Let us check the correctness of the reduction.  Let $v: AP \rightarrow \set{\top, \perp}$ be a valuation satisfying $\aformula$. Let us consider the
run $\arun$ in $\asys$ such that $\arun$ visits the $i^{th}$ loop iff $v(\avarprop_i) = \top$. Since $\aformula$ is satisfied by the valuation $v$, each
of its clause $H_i$ for $1\leq i\leq m$ is also satisfied. Also, in each clause, at least one of the literals is satisfied. It is easy to see that by
the construction $\arun$ satisfies the same automaton for literals. Thus, for $i\in[1,m]$, all the \buchi~automaton,
$\blabelling(\statesof{\arun})\in\languageof{H_i}$. Thus, $\blabelling(\statesof{\arun})\in\languageof{H_1\cap H_2\cap \cdots\cap H_m}$.  

Conversely, if there is a run $\arun$ in $\asys$ such that $\alabelling(\statesof{\arun})\in\languageof{H_1\cap\cdots\cap H_m}$, we fix the valuation
$v$ where for all $i \in \interval{1}{n}$, we have $v(\avarprop_i) = \top$ iff the $i^{th}$ loop is visited by $\arun$. By construction, this implies
that in every clause automaton $H_i$ at least one of the literal automata has an accepting run. Thus, in the formula $\aformula$, at least one literal
of each of the clause is satisfied by the valuation $v$. Thus, $\aformula$ is satisfiable.  
\qed
\end{proof}

Instead of showing that $\mc{n-BA}{\flatks}$ is in \np, we will prove a more general result. We will give an \np~algortihm for the problem
$\mc{n-BA}{\flatcs}$. But, first we will give a \np~algortihm for the problem $\mc{n-BA}{\cps}$. The goal is to find a valid run $\arun$ in $\aschema$
such that $\blabelling(\statesof{\arun})\in\languageof{\bauto^1}\cap\languageof{\bauto^2}\cap\cdots\cap\languageof{\bauto^n}$. Thus, the algorithm
computes formulas $\aformula_i$ charachterizing the parikh image of $\pi_2(\languageof{\flatks\times\bauto^i})$ for $i\in[1,n]$. A solution to
$\aformula_1\wedge\aformula_2\wedge\cdots\aformula_n$ gives, as before, a word accepted by all the \buchi~automata and respecting $\aschema$. To check
that $\arun$ is also a valid run, the algorithm checks to see if the same solution satisfies $\aconstraintsystem$, by checking the satisfiability of
$\aconstraintsystem\wedge\bauto^1\wedge\bauto^2\wedge\cdots\wedge\bauto^n$.

The algorithm is presented formally in Algortihm~\ref{algo:nBA-np}. The algorithm is given as input a path schema $\aschema$ in a flat counter system
$\asys=\tuple{\states',\counters,\edges',\alabelling}$ and $n$ \buchi~automata, $\bauto^1,\bauto^2,\cdots,\bauto^n$ where for all $j\in[1,n]$,
$\bauto^j=\tuple{\states_j,\Sigma,\edges_j,\astate_i,F_j}$.

\begin{algorithm}
\caption{Inputs $\aschema$, $\bauto^1,\bauto^2,\cdots,\bauto^n$}
\label{algo:nBA-np}
\begin{algorithmic}[1]
  \STATE Construct the system of linear equations $\aconstraintsystem$  with variables $\avariable_1,\avariable_2,\cdots,\avariable_{k-1}$ characterizing the runs in the path schema $\aschema$ (assuming $\aschema$ contains $k$ loops).
  \FOR{$i = 1 \to n$}
    \STATE Guess $j\in[1,\length{\aloop_k}]$ and $\astate_f^i\in F_i$
    \STATE Construct the synchronous product, $\aschema\times\bauto^i$ with the sets of final states, $\{\aloop_k(j)\}$,$\{\astate_f\}$ for $\aschema$ and $\bauto^i$ respectively.
    \STATE Construct $\aformula_i$  with variables $\avariable_1,\avariable_2,\cdots,\avariable_{k-1}$ characterizing the Parikh images of $\pi_2(\languageof{\aschema\times\bauto_i})$.
    \STATE Construct the synchronous product of path schema $u=\aloop_k[j,\length{\aloop_k}].\aloop_k^{\omega}$ and automaton $\bauto^i_{\astate_f^i}$ and the two sets of final states as $\{\aloop_k(j)\}$, $\{\astate_f^i\}$ respectively.
    \STATE Continue if $\languageof{u\times\bauto^i_{\astate_f^i}}$ is non-empty. Otherwise ABORT.
  \ENDFOR
  \STATE Guess $\vect{y}\in[1,2^{P(\cdot)}]$.
  \STATE Check whether $\vect{y}$ satisfies $\aconstraintsystem\wedge\aformula_1\wedge\aformula_2\wedge\cdots\wedge\aformula_n$.
\end{algorithmic}
\end{algorithm}

Now, we will prove the correctness of the algorithm.
\begin{lemma}
Algorithm~\ref{algo:nBA-np} returns true iff there exists a run $\arun$ in $\asys$ such that $\blabelling(\statesof{\arun})\in\languageof{\bauto^1\cap\cdots\cap\bauto^n}$.
\end{lemma}
\begin{proof}
Let us assume that there exists a valid infinite run $\arun$ respecting $\aschema$ such that
$\blabelling(\statesof{\arun})\in\languageof{\bauto^1\cap\cdots\cap\bauto^n}$. We will prove that Algorithm~\ref{algo:nBA-np} returns true. In fact we
will show that $\aconstraintsystem\wedge\aformula_1\wedge\aformula_2\wedge\cdots\wedge\aformula_n$ is satisfiable. In that case there exists a
solution and without loss of generality we may assume that the solution is the guessed vector $\vect{y}$ in the algorithm, and thus, the algorithm returns true.

Since $\arun$ is a valid run respecting $\aschema$ and $\aconstraintsystem$ characterizes all valid runs in $\aschema$,
$\vect{y}=\loopsof{\aschema}{\arun}$ satisfies $\aconstraintsystem$. Not that $\vect{y}$ contains $k-1$ elements. Since,
$\blabelling(\statesof{\arun})\in\languageof{\bauto^1\cap\cdots\cap\bauto^n}$, we have that, for all $i\in[1,n]$,
$\blabelling(\statesof{\arun})\in\languageof{\bauto^i}$. Let $\aword=\blabelling(\statesof{\arun})$. $\aword$ has an infinite accepting run in
$\bauto^i$ visiting some final state infinitely often and $\arun$ respects $\aschema$. Let the state be $\astate^i_f\in F_i$. Thus, by
Lemma~\ref{product-automata}, there exists a word $\aword\in\languageof{\bauto^i\times\aschema}$, such that
$\pi_1(\aword)=\blabelling(\statesof{\arun})$. As observed in the proof of~\ref{lemma:fsa-cps-correct}, $\aword$ can be split into two finite parts
such that $\aword=\aword'(\aword'')^{\omega}$ and $\pi_1(\aword')$ has a run from initial state $\astate_i$ to the final state $\astate^i_F$ of
$\bauto^i$ guessed in Step 3. Also, the run in $\aschema$ corresponding to $\aword'$, ends in $\aloop_k(j)$. Thus, $\vect{y}$ also
satisfies$\aformula_i$. Also, note that according to the partition of $\aword$, the corresponding run of $\aword''$ in $\aschema$ starts and ends in
$\aloop_k(j)$ and in $\bauto^i$ starts and ends in $\astate^i_f$. Hence, $\languageof{u\times\bauto^i_{\astate^i_f}}$ is non-empty and the loop is
executed without aborting. Thus, for every $i\in[1,n]$, $\vect{y}$ satisfies $\aformula_i$ and
$\vect{y}\models\aconstraintsystem\wedge\aformula_1\wedge\cdots\wedge\aformula_n$.

Now let us assume that the algorithm returns true. Let $\vect{y}$ be the guessed solution to
$\aconstraintsystem\wedge\aformula_1\wedge\cdots\wedge\aformula_n$. The run $\arun$ be a run in $\aschema$ such that
$\loopsof{\aschema}{\arun}=\vect{y}$. Since $\vect{y}\models\aconstraintsystem$, $\arun$ is a valid run. $\vect{y}$ also satisfies $\aformula_i$ for
all $i\in[1,n]$. Thus, there exists a word $\aword'\in\languageof{\bauto^i_{\astate^i_f}\times\aschema}$ such that $\aword'$ has a run in $\bauto^i$
starting from the initial state $\astate_i$ to $\astate^i_f$. Again, since the algorithm didn't abort at any iteration of the loop, there also exists
a word $\aword''\in\languageof{u\times\bauto^i_{\astate^i_f}}$, such that it has a run starting and ending at $\astate^i_f$ in $\bauto^i$. Note that
the word $\aword=\aword'.(\aword'')^{\omega}$ is a word in $\languageof{\bauto^i}$. Since, $\vect{y}\models\aformula_i$,
$\aword=\blabelling(\statesof{\arun})$. Thus, for all $i\in[1,n]$, $\blabelling(\statesof{\arun})\in\bauto^i$.  
\qed
\end{proof}

\begin{lemma}
\label{nBA-in-np}
Algorithm~\ref{algo:nBA-np} is in \np.
\end{lemma}
\begin{proof}
From Theorem~\ref{thm:constraint}, we know that construction of $\aconstraintsystem$ in Step 1, takes time bounded by $\length{\aschema}\times 2
\times\size{\aschema}^2$. Also, for each $i\in[1,n]$, we know that, construction of $\aschema\times\bauto^i$ also takes time at most
$\size{\aschema}\times\size{\bauto^i}$. Again, construction of $\aformula_i$ takes time at most
$\size{\aschema\times\bauto^i}\leq\size{\aschema}\times\size{\bauto^i}$. Similarly, in Step 6, the construction of $u\times\bauto^i_{\astate_f^i}$ also
takes time at most $\size{u}\times\size{\bauto^i_{\astate_f^i}}\leq \size{\aschema}\times\size{\bauto^i}$. The time taken for checking the emptiness of
$u\times\bauto^i_{\astate_f^i}$ is bounded by $\size{u\times\bauto^i_{\astate_f^i}}^2\leq (\size{u}\times\size{\bauto^i_{\astate_f^i}})^2\leq
(\size{\aschema}\times\size{\bauto^i})^2$. Thus, the execution of the loop takes time which is bounded by $\length{\aschema}\times
2\times\size{\aschema}^2+(3\times\size{\aschema}+\size{\aschema}^2)\times(\size{\bauto^1}+\cdots+\size{\bauto^n})$. Also, $\vect{y}$ though is
exponential, but requires only polynomially many bits and it only requires arithmatic operation on polynomially many bits to check whether $\vect{y}$
is a solution. Thus, the algorithm terminates in polynomial time in the size of the input and also makes guesses that are polynomial in size.
\qed
\end{proof}

As observed before, there are exponentially many path schemas in a flat counter system and that every run in the flat counter system follows some path
schema. So, a possible \np~algorithm for $\mc{n-BA}{\flatcs}$ can non-deterministically choose one of the path schemas and apply the algorithm for
$\mc{n-BA}{\cps}$. From Lemma~\ref{fsa-np-hard} and Lemma~\ref{nBA-in-np} we can conclude that,
\begin{theorem}
$\mc{n-BA}{\flatcs}$ is \np-Complete.
\end{theorem}

Since, flat Kripke structures are a special type of flat counter system, we also have the following:
\begin{theorem}
$\mc{n-BA}{\flatks}$ is \np-Complete.
\end{theorem}



==> section-gmc.tex <==
\section{Global Model-Checking}
\label{section-gmc}

As an additional corollary, we can solve the global model-checking problem with existential
Presburger formulae. We knew that Presburger formulae exist for global model-checking~\cite{demri-model-10} 
for Past LTL (and therefore for FO) but we can conclude that they are structurally simple and we provide an 
alternative proof. Moreover, the question has been open for $\lmc$  since the decidability status of 
MC($\lmc$, $\flatcs$) has been only resolved in the present work. First, let us recall what is
the global model-checking problem over flat counter systems with specification language 
$\mathcal{L}$ (written GMC($\mathcal{L}$, $\flatcs$)):
\begin{description}
\itemsep 0 cm
\item[input:]  a flat counter system $\asys$ of dimension $n$, 
               a control state $\astate$, 
               a specification $\aspecification$ from $\mathcal{L}$,
\item[output:] compute a Presburger formula $\aformula(\avariableter_1, \ldots, \avariableter_n)$ 
               whose solutions are exactly the counter values $\avect$ such that
                 there is a run  $\arun$ starting at $\pair{\astate}{\avect}$ and  such that
                 $\arun \models \aspecification$?
\end{description}
Being able to compute such a formula $\aformula(\avariableter_1, \ldots, \avariableter_n)$  amounts to have
a powerful symbolic representation of an infinite set of configurations sharing the same non-trivial
property. Let us consider also the variant problem known as the 
existential global model-checking problem over flat counter systems with specification language 
$\mathcal{L}$ (written EGMC($\mathcal{L}$, $\flatcs$)):
\begin{description}
\itemsep 0 cm
\item[input:]  a flat counter system $\asys$, 
               a control state $\astate$, 
               a specification $\aspecification$ from $\mathcal{L}$;
\item[question:] are there counter values $\avect$ such that
                 there is a run  $\arun$ starting at $\pair{\astate}{\avect}$ verifying
                 $\arun \models \aspecification$?
\end{description}

Existential global model-checking problem is a decision problem roughly equivalent to model-checking
as stated below. 

\begin{lemma} Let $\mathcal{L}$ be a specification language among FO, BA, ABA, ETL or $\lmc$.
Then, there is a logspace reduction from  EGMC($\mathcal{L}$, $\flatcs$) to  MC($\mathcal{L}$, $\flatcs$)
[resp. from MC($\mathcal{L}$, $\flatcs$) to  EGMC($\mathcal{L}$, $\flatcs$)]. 
\end{lemma}

\begin{proof} (sketch) Let $\asys$, $\astate$ and  $\aspecification$ be an instance of 
 EGMC($\mathcal{L}$, $\flatcs$). In order to build an instance of  MC($\mathcal{L}$, $\flatcs$) for the reduction,
it is sufficient to add a sequence of $n$ loops leading to $\astate$ 
such that each loop increment only the $i$th counter and to start
from a configuration with only zero counter values. In that way, this initial sequence of $n$ loops initializes
the counter values (note that flatness is preserved). For 
the reduction in the other direction, for each transition from the initial
control state $\astate$, we add in the guard a conjunction of linear constraints specifying exactly
what are the initial counter values. Since these transitions might be reused afterwards in the run,
we first start by copying the state $\astate$, leading to two states $\astate$ and $\astate'$ so that
$\astate$ has no more incoming transitions but  $\astate'$ has. 
\end{proof}


\begin{theorem} (I) EGMC(FO, $\flatcs$) and EGMC($\lmc$, $\flatcs$) are \pspace-com\-ple\-te. 
(II) EGMC(BA, $\flatcs$) is \np-complete.
\end{theorem}  

Let us conclude this section by a solution for the global model-checking problem itself.

\begin{corollary}  \label{corollary-global-model-checking}
Let $\mathcal{L}$ be a specification language among FO, BA, ABA, ETL or $\lmc$.
Given a flat counter system $\asys$, a control state $\astate$ and a specification
$\aspecification$ in  $\mathcal{L}$,  one can effectively build an existential Presburger formula
 $\aformula(\avariableter_1, \ldots,\avariableter_n)$
that represents the initial counter values $\avect$ such that there is
an infinite run $\arun$ starting at $\pair{\astate}{\vec{\avect}}$ and
$\arun \models \aspecification$.
\end{corollary}

\ifconference
\else
\input{proof-corollary-global-model-checking}
\fi
 
It also worth noting that the proof of Corollary~\ref{corollary-global-model-checking}
combined with Theorem~\ref{theorem-pottier91} provides an alternative to
Theorem~\ref{thm:stuttering-buchi} (but the bound in Theorem~\ref{thm:stuttering-buchi} is sharper).




==> section-others.tex <==
\section{Other Results}

Alternating \buchi~Automaton(ABA) over uniformly periodic path is in \ptime. By a reduction to the non-emptiness checking for ABA over 1 letter. 

%% 
%% \subsection{Stephane's rememberings}
%% 
%% \begin{enumerate}
%% 
%% \item A problem in \ptime:
%%       \begin{description}
%%       \item[input:] a path schema with a single loop from a CS, an ABA A with alphabet from AT/Q.
%%       \item[question:] check whether the unique run, if any, is accepted by A.  
%%       \end{description}
%%      Cf. email from Sept. 21st.
%% 
%% 
%% \item What about the similar problem with alternating parity automata?
%% 
%% 
%% \item We do not know the complexity for Freeze LTL over flat counter systems. 
%%
%% 
%% 
%% \end{enumerate}

==> subsection-PS.tex <==
\subsection{Path Schemas}

We define minimal path schemas in the line of the respective definitions in~\cite{DemriDharSangnier12}.  Let
$\asys=\tuple{\states,\counters_n,\edges,\alabelling}$ be a flat counter system.  A \defstyle{path segment} $\aseg$ of $\asys$ is a finite sequence of
transitions from $\edges$ such that $\target{\aseg(i)}=\source{\aseg(i+1)}$ for all $0 \leq i < \length{\aseg}-1$. We write $\first{\aseg}$ [resp.
  $\last{\aseg}$] to denote the first [resp. last] control state of a path segment, in other words $\first{\aseg}=\source{\aseg(0)}$ and
$\last{\aseg}=\target{\aseg(\length{\aseg}-1)}$. We also write $\effect{\aseg}$ to denote the sum vector $\sum_{0 \leq i < \length{\aseg}}
\update{\aseg(i)}$ representing the total effect of the updates along the path segment. A path segment $\aseg$ is said to be \defstyle{simple} if
$\length{\aseg} >0$ and for all $0 \leq i,j < \length{\aseg}$, $\aseg(i)=\aseg(j)$ implies $i=j$ (no repetition of transitions).  A \defstyle{loop} is
a simple path segment $\aseg$ such that $\first{\aseg}=\last{\aseg}$.  If a path segment is not a loop it is called a \emph{non-loop segment}.  A
\defstyle{path schema} $\aschema$ is an $\omega$-regular expression built over the alphabet of transitions such that its language represents an
overapproximation of the set of labels obtained from infinite runs following the transitions of $\aschema$.  More precisely, a path schema $\aschema$
is of the form $\aseg_1 \aloop_1^+ \aseg_2 \aloop_2^+ \ldots \aseg_k \aloop_k^{\omega}$ verifying the following conditions:
%
\begin{enumerate}
\itemsep 0 cm
\item $\aloop_1$, \ldots, $\aloop_k$ are loops,
\item $\aseg_1 \aloop_1 \aseg_2 \aloop_2 \ldots \aseg_k \aloop_k$ 
is a path segment.
\end{enumerate}


We write $\lengthpathschema{\aschema}$ to denote $\length{\aseg_1 \aloop_1 \aseg_2 \aloop_2 \ldots \aseg_k \aloop_k}$ and $\nbloops{\aschema}$ its
number $k$ of loops.  Let $\languageof{\aschema}$ denote the set of infinite words in $\edges^\omega$ which belong to the language defined by
$\aschema$. Note that some elements of $\languageof{\aschema}$ may not correspond to any run because of constraints on counter values.  Given $\aword
\in \languageof{\aschema}$, we write $\loopsof{\aschema}{\aword}$ to denote the unique tuple in $(\nat \setminus \set{0})^{k-1}$ such that
$\aword=\aseg_1 \aloop_1^{\loopsof{\aschema}{\aword}[1]}\aseg_2 \aloop_2^{\loopsof{\aschema}{\aword}[2]}\ldots \aseg_k\aloop_k^\omega$. So, for every
$i \in \interval{1}{k-1}$, $\loopsof{\aschema}{\aword}[i]$ is the number of times the loop $\aloop_i$ is taken.  Then, for a configuration $\aconf_0$,
the set $\loopsof{\aschema}{\aconf_0}$ is the set of vectors $\set{\loopsof{\aschema}{\aword} \in (\nat \setminus \set{0})^{k-1} \mid \aword \in
  \wordof{\aschema,\aconf_0}}$. Finally, we say that a run $\arun$ starting in a configuration $\aconf_0$ \defstyle{respects} a path schema $\aschema$
if $\wordof{\arun} \in \wordof{\aschema,\aconf_0}$ and for such a run, we write $\loopsof{\aschema}{\arun}$ to denote
$\loopsof{\aschema}{\wordof{\arun}}$.  Note that by definition, if $\arun$ respects $\aschema$, then each loop $\aloop_i$ is visited at least once,
and the last one infinitely.
%

So far, a flat counter system may have an infinite set of path schemas.  To see this, it is sufficient to unroll loops in path segments.  However, we
can impose minimality conditions on path schemas without sacrificing completeness.  A path schema $\aseg_1 \aloop_1^+ \aseg_2 \aloop_2^+ \ldots
\aseg_k \aloop_k^{\omega}$ is \defstyle{minimal} whenever
\begin{enumerate}
\itemsep 0 cm
\item $\aseg_1 \cdots \aseg_k$ is  either the empty word or a simple non-loop segment,
\item $\aloop_1$, \ldots, $\aloop_k$ are loops with disjoint sets of transitions.
\end{enumerate} 

%
\begin{lemma}\cite{DemriDharSangnier12}
\label{lemma-schemata-finite}
Given a flat counter system $\asys=\tuple{\states,\counters_n,\edges,\alabelling}$, the total number of minimal path schemas of $\asys$ is finite and
is smaller than $\card{\edges}^{(2 \times \card{\edges})}$.
\end{lemma}
%
This lemma is a simple consequence of the fact that in a minimal path schema, each transition occurs at most twice.
%% 
In Figure~\ref{figure-example-minimal-path-schemas}, we present a flat counter system $\asys$ with a unique counter and one of its minimal path
schemas. Each transition $\atransition_i$ labelled by $+i$ corresponds to a transition with the guard $\top$ and the update value $+i$. The minimal
path schema shown in Figure~\ref{figure-example-minimal-path-schemas} corresponds to the $\omega$-regular expression $\atransition_1 (\atransition_2
\atransition_3)^+ \atransition_4 \atransition_5 (\atransition_6 \atransition_5)^{\omega}$.  In order to avoid confusions between path schemas and flat
counter systems that look like path schemas, simple loops in the representation are labelled by \fbox{$\omega$} or \fbox{$\geq 1$} depending whether
the simple loop is the last one or not.  Note that in the representation of path schemas, a state may occur several times, as it is the case for
$\astate_3$ (this cannot occur in the representation of counter systems).
\begin{figure}
\begin{center}
\scalebox{0.8}{
\begin{tikzpicture}[->,>=stealth',shorten >=1pt,
%auto, 
node distance=1cm, thick,auto,bend angle=60]

  \tikzstyle{every state}=[fill=white,draw=black,text=black]
  \node[state] (q0) [below]    {$\astate_0$};
  \node[state] (q1) [right= of q0]    {$\astate_1$};
  \node[state] (q2) [above= of q1]    {$\astate_2$};
  \node[state] (q3) [right=2cm of q1]    {$\astate_3$};
  \node[state] (q4) [above= of q3]    {$\astate_4$};
  \node[state] (q02) [right=2.2cm of q3]    {$\astate_0$};
  \node[state] (q12) [right= of q02]    {$\astate_1$};
  \node[state] (q22) [above= of q12]    {$\astate_2$};
  \node[state] (q32) [right= of q12]    {$\astate_3$};
  \node[state] (q42) [right=1.4cm of q32]    {$\astate_4$};
  \node[state] (q52) [above= of q42]    {$\astate_3$};
  \node (q62) [above=0.3cm of q12] {{\small \fbox{$\mathbf{\geq 1}$}}};
  \node (q72) [above=0.3cm of q42] {{\small \fbox{$\mathbf{\omega}$}}};


  \path[->] (q0) edge node {{\small $+1$}} (q1);
  \path[->] (q1) edge [bend left] node [right] {{\small $+2$}} (q2);
  \path[->] (q2) edge [bend left] node  [right] {{\small $+3$}} (q1);
  \path[->] (q1) edge node  [above] {{\small $+4$}} (q3);
  \path[->] (q3) edge  [bend left] node  [left] {{\small $+5$}} (q4);
  \path[->] (q4) edge  [bend left] node  [right] {{\small $+6$}} (q3);     
  \path[->] (q02) edge node {{\small $+1$}} (q12);
  \path[->] (q12) edge  [bend left] node {{\small $+2$}} (q22);
  \path[->] (q22) edge  [bend left] node {{\small $+3$}} (q12);
  \path[->] (q12) edge  node [below] {{\small $+4$}} (q32);
  \path[->] (q32) edge node  [above] {{\small $+5$}} (q42);
  \path[->] (q42) edge  [bend left] node  [left] {{\small $+5$}} (q52);
  \path[->] (q52) edge  [bend left] node  [right] {{\small $+6$}} (q42);     

                  
\end{tikzpicture}
}
\end{center}
\caption{A flat counter system and one of its minimal path schemas}
\label{figure-example-minimal-path-schemas}
\end{figure}
%%
%%
Minimal path schemas play a crucial role in the sequel, mainly because of the properties stated below.%
\begin{lemma} \cite{DemriDharSangnier12}
Let $\aschema$ be a path schema. There is a minimal path schema $\aschema'$ such that every run respecting $\aschema$ respects $\aschema'$ too.
\end{lemma}
%%
The proof of the above lemma is by an easy verification. Indeed, whenever a maximal number of copies of a simple loop is identified as a factor of
$\aseg_1 \aloop_1 \cdots \aseg_k \aloop_k$, this factor is replaced by the simple loop unless it is already present in the path schema.

Note that we can also represent finite runs in a flat counter system using path schemas. In this case, the path schema need not end with a loop which
is to be taken infinitely many times, but it ends with a path segment, and thus, it is actually a simple regular expression of the form $\aseg_1
\aloop_1^+ \aseg_2 \aloop_2^+ \ldots \aseg_k \aloop_k^{\omega}$. Clearly, all the above definitions and claims extends easily to finite path schemas too.
%Finally, the conditions imposed on the structure of path schemas implies the following corollary which states that the number of minimal path schemas
%for a given flat counter system is at most exponential in the size of the system (see similar statements in~\cite{Leroux&Sutre05}).


==> subsection-PSPACE.tex <==
\subsection{\pspace~Algorithm for $FO_{\varprop}$}
First we will establish the connection between a run $\arun$ in a Parikh path schema $\tuple{\aschema,\aconstraintsystem}$ and a model of $FO_{\varprop}$
formula. For a run $\arun$ respecting the path schema $\aschema$, $\aword=\statesof{\arun}$ is an infinite word over the alphabet
$\powerset{\varprop}$. Thus, $\aword$ obtained from $\arun$ is also a model of $FO_{\varprop}$ formula.
%Also, in such a run, at a position in $\arun$, specific guards are satisfied. Thus, in such a model, at every position we can label it with guards
%$\aguard\in\guards(\counters_n)$ that are satisfied at the position. Hence, we can obtain an $\omega$-sequence from $\arun$ over the alphabet
%$\Sigma=2^{AT\cup\guards(\counters_n)}$.  As a result, along with the unary predicates $(P_a)_{a\in \varprop}$ we can also have the unary predicates
%$(P_{\aguard})_{\aguard\in\guards(\counters_n)}$ defined as $P_{\aguard}=\{i\in\nat\mid~\pi_2(\aword(i))\models\aguard\}$ and the satisfaction
%relation is defined similar to $(P_a)$.  
\paragraph{Dealing with all except last loop}
By definition a run $\arun$ in Parikh path schema, respecting path schema $\aschema$ is an $\omega$-sequence of transitions. As a corollary of the stuttering theorem, we
obtain the following for runs from Parikh path schema, $\tuple{\aschema,\aconstraintsystem}$.
\begin{corollary}
\label{cor:runFO}
Given a path schema $\aschema=\aseg_1\aloop_1^{+}\aseg_2\aloop_2^{+}\cdots\aseg_k^{+}\aloop_k^{\omega}$ and a $FO_{\varprop}$ sentence $\aformula$, if
there exists a run $\arun'\models\aformula$, then there also exists a run $\arun$ respecting $\aschema$, where for all $i\in[1,k-1]$ $\loopsof{\aschema}{\arun}[i]\leq
2^{\qheight{\aformula}}$ and $\arun\models\aformula$.
\end{corollary}
By corollary \ref{cor:runFO}, we can bound the repetition of the all the loops except the last one from a path schema in a run to at most
$2^{\qheight{\aformula}}$. 

\paragraph{Dealing with the last loop}
Given a paths schema, $\aschema=\aseg_1\aloop_1^{+}\aseg_2\aloop_2^{+}\cdots\aseg_k^{+}\aloop_k^{\omega}$, a vector $\vect{y}\in\nat^{k-1}$ specifying
the number of times each loop is to be taken. Consider the path segment obtained by unfolding the $k-1$ loops in $\aschema$ denoted as
$\aseg'=\aseg_1\aloop_1^{\vect{y}[1]}\aseg_2\aloop_2^{\vect{y}[2]}\cdots\aseg_{k-1}\aloop_{k-1}^{\vect{y}[k-1]}\aseg_k$. Now, we have the ultimately
periodic path $\aschema'=\aseg'\aloop_k^{\omega}$ which is also represented as the tuple $\tuple{\aschema,\vect{y}}$. Using $\aschema'$ and
$\aformula$ we construct $\hat{\aformula}_{\aschema,\vect{y}}$ by replacing every quantifier ``$\exists x$'' in $\aformula$ by ``$\exists x<
\length{\aseg'}+ \length{\aloop_k}.\powerset{\qheight{\aformula}}$''. The following lemma says that the $\aformula$ and
$\hat{\aformula}_{\aschema,\vect{y}}$ are similar in their satisfiability on $\aschema'$.
\begin{lemma}\cite{Markey&Schnoebelen03}
\label{lem:runFO}
Given a path schema $\aschema=\aseg_1\aloop_1^{+}\aseg_2\aloop_2^{+}\cdots\aseg_k^{+}\aloop_k^{\omega}$, a vector $\vect{y}\in\nat^{k-1}$ and a
$FO_{\varprop}$ sentence $\aformula$, for any infinite $\arun$ respecting $\aschema$ with $\loopsof{\aschema}{\arun}=\vect{y}$, we can construct
$\hat{\aformula}_{\aschema,\vect{y}}$ where every variable is bounded by an integer
$M<(\length{\aseg_1\aloop_1^{\vect{y}[1]}\aseg_2\aloop_2^{\vect{y}[2]}\cdots\aseg_{k-1}\aloop_{k-1}^{\vect{y}[k-1]}})+\powerset{\qheight{\aformula}}\times\length{\aloop_k}$
such that $\arun\models\aformula$ iff $\arun\models\hat{\aformula}_{\aschema,\vect{y}}$.
\end{lemma}
The lemma allows us to examine a finite portion of a given run to check for satisfiability of $FO_{\varprop}$ formula, since, we can bound the
assignment of variables to at most $\powerset{\qheight{\aformula}}\times\length{\aschema}$. 
%The infinite run is obtained by limiting the iteration of all including the last loop to at most $2^{\qheight{\aformula}}$. Thus, the integer $M$ can
%be defined as $M=\Sigma_{1\leq i \leq k}\length{\aseg_i}+\length{\aloop_i}^{\qheight{\aformula}}$
%\begin{proof}
%Consider two variables $\avar_i, \avar_j$ in $\aformula$, such that $f(\avar_i)=a$, $f(\avar_j)=b$ and $a>b$. Let
%$\wordof{\arun(a)}\in\aseg_m\aloop_m$ and $\wordof{\arun(b)}\in\aseg_n\aloop_n$ for any $m,n[1,k]$ (it might be the case that $m=n$). We know by
%Theorem \ref{theorem:stuttering}, that if
%$a-b>\length{\aseg_m}+\length{\aloop_m}^{\qheight{\aformula}}+\cdots+\length{\aseg_n}+\length{\aloop_n}^{\qheight{\aformula}}$, then we can reduce the
%number of iterations of loops to have
%$a-b\leq\length{\aseg_m}+\length{\aloop_m}^{\qheight{\aformula}}+\cdots+\length{\aseg_n}+\length{\aloop_n}^{\qheight{\aformula}}$ and still preserving the
%satisfiability of $\aformula$. This, in effect bounds the number of times each loop has to be taken alongwith the last loop. Hence, we can get a new run
%$\arun'$ from $\arun$ by bounding the iterations of each loop to a maximum of $\qheight{\aformula}$. In that case, the maximum value of a variable can be bounded to 
%$\Sigma_{1\leq i \leq k}\length{\aseg_i}+\length{\aloop_i}^{\qheight{\aformula}}$ while still preserving the satisfiability of $\aformula$ over $\arun'$.
%Taking $M=\Sigma_{1\leq i \leq k}\length{\aseg_i}+\length{\aloop_i}^{\qheight{\aformula}}$ proves the lemma.  
%\qed
%\end{proof}

Now, we can give an algorithm for the problem $\mc{FO_{\varprop}}{\pps}$. Given a Parikh path schema $\tuple{\aschema,\aconstraintsystem}$ where
$\aschema=\aseg_1\aloop_1^{+}\aseg_2\aloop_2^{+}\cdots\aseg_k^{+}\aloop_k^{\omega}$. According to
Lemma~\ref{lem:runFO}, each loop in $\aschema$ will be taken by a run $\arun$ satisfying $\aformula$ at most $2^{\qheight{\aformula'}}$
times. Again, we non-deterministically choose the number of times each loop is taken, which is represented by $\vect{y}$. But since the path obtained
from unfolding the loops is exponential in size, we will not explicitely construct the path but instead perform model checking of $\aformula$ on the
succint representation of the path as $\tuple{\aschema,\vect{y}}$. Note that this representation can be represented in polynomial space. After
checking for satisfiability of $\aformula$, we then check for a run respecting both $\aconstraintsystem$ and the satisfiability of
$\aformula'$. Here we assume that the variables in $\aformula$, $\avar_1,\avar_2\cdots$ can be uniquely identified by their index. 

The following algorithm is for checking the satisfiability of a formula $\aformula=\hat{\aformula'}_{\aschema,\vect{y}}$ obtained from a
$FO_{\avarprop}$ formula $\aformula'$ over an infinite run $\arun$ represented as $\tuple{\aschema,\loopsof{\aschema}{\arun}}$ is given formally
below:

\begin{algorithm}
{\footnotesize
\caption{Procedure $FOSAT$ with input a path schema $\aschema$, $\vect{y}\in[1,\powerset{\qheight{\aformula}}]^{k-1}$, $\aformula$, and an assignment function $\vect{z}$}
\label{algo:FOSAT}
\begin{algorithmic}[1]
\IF{$\aformula$ is of the form $P_a(\avar_i)$, for any $a\in \varprop$}
   \STATE Calculate the node at position $\vect{z}[i]$ in $\aschema$ and return $P_a(\vect{z}[i])$.
\ELSIF{$\aformula$ is of the form $\neg \aformula'$}
   \IF{$FOSAT(\aschema,\vect{y},\aformula',\vect{z})$ is true}
      \STATE return FALSE.
   \ELSE
      \STATE return TRUE.
   \ENDIF
\ELSIF{$\aformula$ is of the form $\exists \avar_i\leq m. \aformula'(\avar_i)$}
   \STATE guess a position $k\in\interval{1}{m}$.
   \STATE set $\vect{z}=\vect{z}:[i\rightarrow k]$.
   \STATE return the $FOSAT(\aschema,\vect{y},\aformula',\vect{z})$.
\ELSIF{$\aformula$ is of the form $\avar_i=\avar_j$}
   \STATE return $\vect{z}[i]=\vect{z}[j]$.
\ELSIF{$\aformula$ is of the form $\avar_i>\avar_j$}
   \STATE return $\vect{z}[i]>\vect{z}[j]$.
\ELSIF{$\aformula$ is of the form $S(\avar_i,\avar_j)$}
   \STATE return $\vect{z}[i]=\vect{z}[j]+1$.
\ELSIF{$\aformula$ is of the form $\aformula_1\wedge\aformula_2$}
   \STATE return $FOSAT(\aschema,\vect{y},\aformula_1,\vect{z})\wedge FOSAT(\aschema,\vect{y},\aformula_2,\vect{z})$.
\ENDIF
\end{algorithmic}
}%%
\end{algorithm}

Note that $FOSAT$ is evaluated on infinite runs $\arun$ such that $\loopsof{\aschema}{\arun}=\vect{y}$ where $\vect{y}\in
[1,2^{\qheight{\aformula}}]^{k-1}$. Also, that $\aformula$ given as input to $FOSAT$ is actually a formula where the variables are bounded as described in
Lemma~\ref{lem:runFO} and $\vect{z}$ acts as the assignment function. Clearly, if $FOSAT$ with input $\aschema$, $\vect{y}$ and $\aformula$ returns
true, then the run $\arun$ such that $\loopsof{\aschema}{\arun}=\vect{y}$ satisfies $\aformula$.
\begin{claim}
\label{clm:fosat}
Procedure $FOSAT$ requires space which is polynomial in the size of $\aschema$ and $\aformula$.
\end{claim}
\begin{proof}
Note that the algorithm only needs to store $\aschema$, $\vect{y}$, $\aformula$ and $\vect{z}$. Each component of $\vect{y}$ belongs in the interval
$\interval{1}{2^{\qheight{\aformula}}}$ and since the elements of $\vect{z}$ are positions in the run represented by $\tuple{\aschema,\vect{y}}$, each
position can be at most $\length{\aschema}\times 2^{\qheight{\aformula}}$. Since, we use binary encoding to store any number, $\vect{y}$ and
$\vect{z}$ requires at most $log_2(\length{\aschema}\times 2^{\qheight{\aformula}})$ space. Thus, the total space required for running $FOSAT$ is
bounded by a polynomial in $\size{\aschema}$ and $\size{\aformula}$.
\qed
\end{proof}
Before giving the \pspace~algorithm for model checking $FO_{\varprop}$ sentence over Parikh path schema, we will the prove a theorem stating that if
the constraint system in Parikh path schema is satisfiable, it admits a small solution.
\begin{theorem}\cite{Pottier91}
Given a quantifier-free Presburger formula $\aformula(\avar_1,\ldots,\avar_n)$ and let $N=\size{\aformula(\avar_1,\ldots,\avar_n)}$ and $p^{\star}(N)=2^{2N(N+2)}$ then,
\begin{enumerate}
\item There exists sets $\basis\subseteq[-p^{\star}(N),p^{\star}(N)]^{n}$ and
  $\period=\{\aperiod_1,\ldots,\aperiod_k\}\subseteq[-p^{\star}(N),p^{\star}(N)]^{n}$ with $k\leq 2^{2N(N+1)(N+2)}$ such that
  for all $\vect{y}\in\nat^{n}$ and $\vect{y}\models\aformula(\avar_1,\ldots,\avar_n)$, there exists $\abasis\in\basis$ for which
  $\vect{y}=\abasis + \Sigma_{i\in[1,k]}a_i.\aperiod_i$ for some $(a_1,a_2,\ldots,a_k)\in\nat^{k}$.
\item If $\aformula(\avar_1,\ldots,\avar_n)$ is satisfiable, then there exists
  $\vect{y}\models\aformula(\avar_1,\ldots,\avar_n)$ such that $\vect{y}\in[-p^{\star}(N),p^{\star}(N)]^{n}$.
\end{enumerate}
\end{theorem}
\begin{algorithm}
{\footnotesize
\caption{The \pspace~algorithm with inputs Parikh path schema $\tuple{\aschema,\aconstraintsystem}$, $\aformula$}
\label{algo:FOpps}
\begin{algorithmic}[1]
%\STATE guess a minimal  path schema $\aschema$
%       of $\asys$ 
%\STATE build a resource $\aresource = \triple{\aset}{T}{B}$ coherent with $\aschema$ and $\aformula$
%\STATE guess a valid  path  schema  $\aschema' = 
%       \aseg_1 \aloop_1^+ \aseg_2 \aloop_2^+ \ldots \aseg_k \aloop_k^\omega$ 
%       such that $\aschema'\in Y_{\aschema}$. % and transform $\aformula$ to $\aformula'\in FO[\emptyset]$.
\STATE guess $\vec{y} \in \interval{1}{2^{\qheight{\aformula}}}^{k-1}$
\STATE guess $\vec{y'} \in \interval{1}{2^{p^{\star}(\size{\asys} + \size{\aformula})}}^{k-1}$ 
%\STATE check that $\aschema'$ belongs to $\asetbis_\aschema$ 
%\iflong
\STATE Let $\vect{z}=(0)$. 
\STATE Construct $\hat{\aformula_{\aschema,\vect{y}}}$ from $\aformula$, $\aschema$ and $\vect{y}$ as in Lemma~\ref{lem:runFO}
\STATE continue if $FOSAT(\aschema,\vect{y},\hat{\aformula_{\aschema,\vect{y}}}, \vect{z})$ returns true.
\STATE otherwise ABORT. 
%\STATE  build the constraint system $\aconstraintsystem$ 
%        over the variables $\avariablebis_1$, \ldots, $\avariablebis_{k-1}$
%        for $\aschema'$ with initial
%        counter values $\vec{v_0}$ (obtained from Theorem~\ref{thm:constraint})
\FOR{$i = 1 \to k-1$} 
\IF{$\vec{y}[i] = 2^{ \qheight{\aformula'}}$}
   \STATE $\aformulabis_i \gets ``\avariablebis_i \geq 2^{ \qheight{\aformula'}}"$
   \ELSE
   \STATE  $\aformulabis_i \gets ``\avariablebis_i = \vec{y}[i]"$
\ENDIF
\ENDFOR
\STATE check that $\vec{y'} \models \aconstraintsystem \wedge \aformulabis_1 \wedge \cdots
       \wedge \aformulabis_{k-1}$
\end{algorithmic}
}%%
\end{algorithm}

\begin{lemma}
Algorithm~\ref{algo:FOpps} with input Parikh path schema $\tuple{\aschema,\aconstraintsystem}$ and $\aformula$ returns true iff
$\tuple{\aschema,\aconstraintsystem}\models\aformula$.
\end{lemma}
\begin{proof}
Let us assume that $\tuple{\aschema,\aconstraintsystem}\models\aformula$. In that case, there exists at least one run $\arun$ in
$\tuple{\aschema,\aconstraintsystem}$ such that $\arun\models\aformula$. Now, $\arun$ respects the path schema $\aschema$. Let
$\vect{y}[i]=\loopsof{\aschema}{\arun}[i]$ if $\loopsof{\aschema}{\arun}[i]\leq 2^{\qheight{\aformula}}$ otherwise %TODO explain
$\vect{y}[i]=2^{\qheight{\aformula}}$. Since $\arun\models\aformula$, using Corollary~\ref{cor:runFO}, we have that $\arun'\models\aformula$ where
$\loopsof{\aschema}{\arun'}=\vect{y}$. Thus, the call to $FOSAT$ returns true as noted due to Lemma~\ref{lem:runFO}. Since, $\arun$ is a run in
$\tuple{\aschema,\aconstraintsystem}$, $\loopsof{\aschema}{\arun}$ satisfies $\aconstraintsystem$. By construction of $\vect{y}$,
$\loopsof{\aschema}{\arun}$ also satisfies $\aformulabis_1 \wedge \cdots \wedge \aformulabis_{k-1}$. Thus, $\aconstraintsystem \wedge \aformulabis_1
\wedge \cdots \wedge \aformulabis_{k-1}$ has the solution $\loopsof{\aschema}{\arun}$ and hence satisfiable. By, Theorem~\ref{thm:constraint} and
\cite{Borosh&Treybig76}, we know that there exists a solution for $\aconstraintsystem \wedge \aformulabis_1 \wedge \cdots \wedge \aformulabis_{k-1}$
where each variable has value within $\interval{1}{2^{p^{\star}(\size{\asys} + \size{\aformula'})}}$. Let the solution be the guessed vector
$\vec{y'}$. Thus, $\vec{y'}\models\aconstraintsystem \wedge \aformulabis_1 \wedge \cdots \wedge \aformulabis_{k-1}$ and hence
Algorithm~\ref{algo:FOpps} returns true.

For the other direction, let's assume the algorithm returns true with input $\tuple{\aschema,\aconstraintsystem}$ and $\aformula$. This means that there are
$\vec{y}$, $\vec{y'}$ that satisfy all the checks. Consider a run $\arun$ respecting $\aschema$ such that $\loopsof{\aschema}{\arun}=\vec{y'}$.
Since, $\vect{y'}$ is a solution for $\aconstraintsystem$ and respects $\aschema$, $\arun$ is a run in $\tuple{\aschema,\aconstraintsystem}$. Now we need to
prove that $\arun\models\aformula$. Since, $FOSAT$ returned true with input $\aschema,\vect{y}$ and $\hat{\aformula}_{\aschema,\vect{y}}$, we
know that $\aseg_1 \aloop_1^{\vec{y}[1]} \aseg_2 \aloop_2^{\vec{y}[2]} \ldots \aloop_{k-1}^{\vec{y}[k-1]} \aseg_k \aloop_k^{\omega}\models
\hat{\aformula}_{\aschema,\vect{y}}$. By Lemma~\ref{lem:runFO}, we know that $\aseg_1 \aloop_1^{\vec{y}[1]} \aseg_2 \aloop_2^{\vec{y}[2]} \ldots
\aloop_{k-1}^{\vec{y}[k-1]} \aseg_k \aloop_k^{\omega}\models\aformula$. By Corollary~\ref{cor:runFO}, we deduce that $\aseg_1 \aloop_1^{\vec{y'}[1]}
\aseg_2 \aloop_2^{\vec{y'}[2]} \ldots \aloop_{k-1}^{\vec{y'}[k-1]} \aseg_k \aloop_k^\omega\models \aformula$. Thus, $\arun$ from
$\tuple{\aschema,\aconstraintsystem}$, $\arun\models\aformula$.  
\qed
\end{proof}

\begin{theorem}
Algorithm~\ref{algo:FOpps} runs in polynomial space.
\end{theorem}
\begin{proof}
The space required by the algorithm is for storing $\aschema$, $\aschema'$, $\aformula$, $\aformula'$, $\vec{y}$, $\vec{y'}$ and
$\aconstraintsystem$. We know that $\size{\aschema}$ and $\size{\aschema'}$ is bounded by a polynomial in $\size{\asys}$. Also,
$\size{\aformula}=\size{\aformula'}$. By Claim~\ref{clm:fosat}, we know that the space required by $FOSAT$ is also bounded by a polynomial in
$\size{\aschema'}$ and $\aformula'$. As shown in the proof of Claim~\ref{clm:fosat}, $\vec{y}$ and $\vec{y'}$ can be represented using polynomially
many bits. By Theorem~\ref{thm:constraint}, $\aconstraintsystem$ can be bounded in size by $\size{\aschema'}\times\size{\aformula'}$. Thus,
Algorithm~\ref{algo:FOpps} requires space which can be bounded by a polynomial in $\size{\asys}$ and $\size{\aformula}$. Hence, the algorithm runs in
polynomial space.
\qed
\end{proof}
\pspace-hardness already occurs with finite paths of length two where there is an obvious reduction from Quantified Boolean Formula (QBF).
Thus, we have that,
\begin{theorem}
$\mc{FO}{\pps}$ is \pspace-Complete.
\end{theorem}


Now, we are in position to compare the complexity of the existential 
model-checking problem for three classes of Kripke structures when either
first-order logic is involved or when Past LTL is involved (these two logics have nevertheless the
same expressive power). Note that as a consequence
of our result, model-checking  flat Kripke structures with first-order logic is in \pspace. 

\begin{center}
\begin{tabular}{|c||c|c|c|}
\hline
& Kripke structures & Flat Kripke structures & Ultimately periodic paths\\
\hline
\hline
FO & Non-elementary~\cite{Stockmeyer74} & \pspace-complete & \pspace-complete~\cite{Markey&Schnoebelen03}\\
\hline
Past LTL & \pspace-complete~\cite{Sistla&Clarke85} & \np-complete~\cite{DemriDharSangnier12} & \ptime~\cite{Laroussinie&Markey&Schnoebelen02}\\
\hline
\end{tabular}
\end{center}

%±±±±±±±±±±±±±±±±±±±±±±±±±±±§§§§§§§§§§§§§§§§§§§§§§§§§§§§§ commented til EOF
\begin{comment}
\subsubsection{With Counters}
Let us now consider the problem of model checking FO sentences on flat counter systems. The problem encountered here is that the run $\arun$
satisfying the FO sentence $\aformula$ also has to be a valid run with respect to the guards and updates of the system. For this reason, we use a
system of equations which characterizes the runs in the path schema. This, alongwith the stuttering theorem for FO, allows us to find a run $\arun$,
which satisfies $\aformula$ as well as is a valid run in the system/path schema. From \cite{DemriDharSangnier12}, we get the following theorem:
\begin{theorem}\cite{DemriDharSangnier12}
Given a path schema $\aschema$ from a flat counter system without disjunction, we can construct a constraint system $\aconstraintsystem$ such that:
\begin{itemize}
  \item $\aconstraintsystem$ has $k-1$ variables, where $k$ is the number of loops in $\aschema$. 
  \item Every solution $(m_1,m_2,\ldots,m_{k-1})$ to $\aconstraintsystem$ implies that there exists a run $\arun$ in $\aschema$, such that
    $\loopsof{\aschema}{\arun}=(m_1,m_2,\ldots,m_{k-1})$
  \item Number of constraints or disjunction in $\aconstraintsystem$ is bounded by a polynomial in $\size{\aschema}^2$.
  \item The value of the maximum coefficient appearing in $\aconstraintsystem$ is bounded by $\size{\aschema}^2$.
  \item The time required for the construction of $\aconstraintsystem$ is bounded by a polynomial in $\size{\aschema}^2$.
\end{itemize}
\end{theorem}
First we will show that $\mc{FO}{\cps}$ is in \pspace.  Given a path schema $\aschema$ and a FO sentence $\aformula$, the algorithm proceeds by
finding a run $\arun$ in $\aschema$ represented as the tuple $\tuple{\aschema,\vect{y}}$ ignoring the counters, such that $\arun\models\aformula$
using the \pspace~algorithm for $\mc{FO}{\kps}$. Using the stuttering theorem for FO, we know that for every $i\in[1,k]$ if
$\vect{y}[i]=2^{\qheight{\aformula}}$ then for $\vect{y}[i]\geq 2^{\qheight{\aformula}}$ also $\tuple{\aschema,\vect{y}}\models\aformula$. We add
relevant constraints to $\aconstraintsystem$ and then try to guess a solution to it. If there exists a solution then the run $\arun'$ is both a valid
run and satisfies $\aformula$. The algorithm is presented formally in Algorithm~\ref{algo:FOcps}.
\end{comment}


==> subsection-buchi1.tex <==
\subsection{\np~Algorithm for \buchi~automata}

The goal of this section is to characterize the complexity of the model-checking problem
over flat counter systems with \buchi~automata. Thanks to Theorem~\ref{thm:stuttering-buchi},
we have already established the existence of $\amap_{{\rm BA}}$ for the intersection non-emptiness problem
with \buchi~automata.

So, checking whether  $\alang(\acps) \cap \alang(\bauto)$  is non-empty amounts to guess some
$\vect{n} \in \interval{0}{2.\size{\bauto}^{\size{\acps}}\times \powerset{p_1(\size{\acps})+p_2(\size{\acps})}}^{k-1}$ and check
whether 
$$\aword = \aseg_1 (\aloop_1)^{\vect{n}[1]} \cdots \aseg_{k-1} (\aloop_{k-1})^{\vect{n}[k-1]} \aseg_k (\aloop_k)^{\omega} \in 
\alang(\acps) \cap \alang(\bauto).
$$  
Checking whether $\aword \in \alang(\acps)$ can be done in polynomial time
in $\size{\acps}log(2.\size{\bauto})+p_1(\size{\acps})+p_2(\size{\acps})$ 
(and therefore in polynomial time in $log(\size{\bauto})
+ \size{\acps}$) since this amounts to verify whether $\vect{n} \models \aformula$. 
Checking whether $\aword \in \alang(\bauto)$ can be done in polynomial space in
$\size{\bauto}
+ \size{\acps}$.  
Indeed, checking whether a $\omega$-word $u\in\alang(\bauto)$ can be done by simulating $\bauto$ over $u$ in space $\mathcal{O}(\size{u} \size{\bauto})$. 
When the $\omega$-word is $\aword$ this provides a space bound in
$\mathcal{O}(\size{\acps} \times \size{\bauto}^{\size{\acps}}\times \powerset{p_1(\size{\acps})+p_2(\size{\acps})})$.
Hence, this leads to a polynomial space decision procedure for the intersection non-emptiness
problem as explained below. 

Below, we show that the membership problem with \buchi~automata can be solved in polynomial time in $\size{\acps} + \size{\bauto}$.
Given an alphabet $\aalphabet$, we will consider a \buchi~automaton $\bauto=\tuple{\states,\aalphabet,\astate_0,\edges,F}$, a constrained path schema
$\acps=\pair{\cpschema}{\aconstraintsystem}$ and a vector $\vect{y}\in(2.\size{\bauto}^{\size{\acps}}\times\powerset{p_1(\size{\acps})\times
  p_2(\size{\acps})})^{k-1}$ such that $\vect{y}\models\aconstraintsystem$. For technical convenience in the proof, we consider the set of alphabets
$\aalphabet'$ and a function $g:\aalphabet'\rightarrow\aalphabet$
%$\{a_1,a_2,\cdots,a_{n}\}\notin\aalphabet$ where $n=\length{\acps}$. We label each position of $\acps$ with an additional unique alphabet, and thus
%modify the labelling function as $\alabelling(\acps(i))=t_i$ for $i\in[1,\length{\acps}]$.
%Without loss of generality, assume that $\acps$ is defined over $\aalphabet$ and each position in $\aconstraintsystem$ has an unique alphabet. 
We take $\acps'=\pair{\aseg'_1(\aloop'_1)^{*}\ldots\aseg'_{k-1}(\aloop'_{k-1})^{*}\aseg'_k\aloop_k^{\omega}}{\aconstraintsystem}$ over the alphabet
$\aalphabet'$ such that $\alang(\acps)=g(\alang(\acps'))$ and each position of $\acps'$ is marked by an unique alphabet.  Here the map $\loopmap$ from
Section 3.3 is an exponential map. The membership problem amounts to determine whether
$\aword=\aseg_1(\aloop_1)^{\vect{y}[1]}\ldots\aseg_{k-1}(\aloop_{k-1})^{\vect{y}[k-1]}\aseg_k\aloop_k^{\omega}\in\alang(\bauto)$ holds. We follow a
procedure similar to the well-known procedure of finding a \textit{lasso} in the \buchi~automaton. This, is achieved by first taking a state
$\astate_f\in F$ and a position $j$ in $\aloop_k$. Note that an accepting run in a \buchi~automaton can be divided into two parts: one where it
reaches from initial state to the final state $\astate_f$ and the other where it starts from the final state $\astate_f$ and returns to the
same state, infinitely often. We construct two finite state automata, $\fsa_1=\tuple{\states,\aalphabet,\astate_0,\edges,\{\astate_f\}}$ and
$\fsa_2=\tuple{\states,\aalphabet,\astate_f,\edges,\{\astate_f\}}$ to recognise the respective part of the run. Next, we construct two more finite
state automata $\fsa_p,\fsa_{loop}$ such that $g(\alang(\fsa_p))=\alang(\fsa_1)\cup
g(\alang(\aseg'_1(\aloop'_1)^{*}\ldots\aseg'_{k-1}(\aloop'_{k-1})^{*}\aseg'_k\aloop'_k[1,j]))$ (the finite part of $\acps$) and
$\alang(\fsa_{loop})=\alang(\fsa_2)\cup\alang(\aloop_k[j+1,\length{\aloop_k}]\aloop_k^{*}\aloop_k[1,j])$ (iterations of the last loop of $\acps$). The
next step comprises to constructing the formula $\aformulabis(\avariable_{1}\cdots,\avariable_{k-1})$ for the Parikh image for a projection of
$\alang(\fsa_p)$. The projection function is defined for every $c\in\aalphabet'$ $\pi(c)=t_i$ when $c=\aloop_j(1)$ for any $j\in[1,k-1]$ otherwise
$\pi(c)=\epsilon$. Note that in a word $\aword\in\pi(\alang(\fsa_p))$, the number of times $t_i$ appears is exactly the number of times $\aloop'_i$
appears in $\aword'\in \alang(\fsa_p)$ where $\pi(\aword')=\aword$. We check that
$\vect{y}\models\aformulabis(\avariable_{1}\cdots,\avariable_{k-1})$. This ensures that the word described by $\acps$ excluding the last loop
$\aloop_k$, is actually part of an accepting word. On the other hand we only check that $\alang(\fsa_{loop})\neq\emptyset$. This ensures that we can
visit a final state infinitely often in the run for $\aword$ over $\bauto$. These together tells us whether $\aword\in\alang(\bauto)$.
\begin{algorithm}
\caption{Inputs $\bauto$, $\acps=\pair{\cpschema}{\aconstraintsystem}$, $\vect{y}\in(\size{\bauto}^{\size{\acps}}\times\powerset{p_1(\size{\acps})\times p_2(\size{\acps})})^{k-1}$}
\label{algo:BA-np}
\begin{algorithmic}[1]
  \FOR{each $\astate_f\in F$ and each $j\in[1,\length{\aloop_k}]$}
%  \STATE Guess $\astate_f\in F$ and $j\in[1,\length{\aloop_k}]$.
     \STATE Construct $\fsa_1=\tuple{\states,\aalphabet,\astate_0,\edges,\{\astate_f\}}$ and
         $\fsa_2=\tuple{\states,\aalphabet,\astate_f,\edges,\{\astate_f\}}$.  
     \STATE Construct $\fsa_p$ and $\fsa_{loop}$ such that\\
         $g(\alang(\fsa_p))=\alang(\fsa_1)\cap g(\alang(\aseg'_1(\aloop'_1)^{*}\ldots\aseg'_{k-1}(\aloop'_{k-1})^{*}\aseg'_k\aloop'_k[1,j]))$ and\\
         $\alang(\fsa_{loop})=\alang(\fsa_2)\cap\alang(\aloop_k[j+1,\length{\aloop_k}]\aloop_k^{+}\aloop_k[1,j])$.
     \STATE Construct $\aformulabis(\avariable_{1}\cdots,\avariable_{k-1})$ characterizing the Parikh image of $\pi(\alang(\fsa_p))$.
     \IF {$\vect{y}\models\aformulabis(\avariable_{1}\cdots,\avariable_{k-1})$ \AND $\alang(\fsa_{loop})\neq\emptyset$}
        \STATE return TRUE.
     \ENDIF
  \ENDFOR
  \STATE return FALSE.
\end{algorithmic}
\end{algorithm}

\begin{lemma}
Algorithm \ref{algo:BA-np} returns true iff $\aword=\aseg_1(\aloop_1)^{\vect{y}[1]}\ldots\aseg_{k-1}(\aloop_{k-1})^{\vect{y}[k-1]}\aseg_k\aloop_k^{\omega}\in\alang(\bauto)$.
\end{lemma}
\begin{proof}
First let us assume that
$\aword=\aseg_1(\aloop_1)^{\vect{y}[1]}\ldots\aseg_{k-1}(\aloop_{k-1})^{\vect{y}[k-1]}\aseg_k\aloop_k^{\omega}\in\alang(\bauto)$. Thus, there is an
accepting run $\arun\in\edges^{\omega}$ for $\aword$ in $\bauto$. According to the \buchi~acceptance condition there exists a state $\astate_f\in F$
which is visited infinitely often. In $\aword$ only $\aloop_k$ is taken infinitely many times. Thus, $\aloop_k$ being of finite size, there exists a
position $j\in[1,\length{\aloop_k}]$ such that transitions of the form $\astate\labtrans{\aloop_k(j)}\astate_f$ for some $\astate\in\states$ occurs
infinitely many times in $\arun$. Thus, for $\arun$ to be an accepting run, there exists
$\aword'=\alang(\aseg_1(\aloop_1)^{+}\ldots\aseg_{k-1}(\aloop_{k-1})^{+}\aseg_k\aloop_k[1,j])$, which has a run in $\bauto$ from $\astate_i$ to
$\astate_f$ and there must exists words $\aword''\in\alang(\aloop_k[j+1,\length{\aloop_k}]\aloop_k^{+}\aloop_k[1,j])$ which has a run from $\astate_f$ to
$\astate_f$. In effect, $\alang(\fsa_p)\neq \emptyset$ and $\alang(\fsa_{loop})\neq\emptyset$. Solutions to
$\aformulabis(\avariable_{1}\cdots,\avariable_{k-1})$ characterizing the Parikh image of $\pi(\alang(\fsa_p))$ gives us the number of times each loop
$\aloop'_i$ for $i\in[1,k-1]$ is taken in words from $\alang(\fsa_p)$. Note that the number of times $\aloop'_i$ is taken in any word $u
\in\alang(\fsa_p)$ is same as the number of times $\aloop_i$ is taken in $g(u)$. Since, $\aword\in\alang(\bauto)$, we know that
$\aseg_1(\aloop_1)^{\vect{y}[1]}\ldots\aseg_{k-1}(\aloop_{k-1})^{\vect{y}[k-1]}\aseg_k\aloop_k[1,j]\in g(\alang(\fsa_p))$. Hence,
$\vect{y}\models\aformulabis(\avariable_{1}\cdots,\avariable_{k-1})$. Thus, there exists at least one choice of $\astate_f$ and $j$, for which the algorithm
returns true.

Now let us assume that the algorithm returns true. Thus, there exists $\astate_f\in F$ and $j\in[1,\length{\aloop_k}]$ such that
$\vect{y}\models\aformulabis(\avariable_{1}\cdots,\avariable_{k-1})$ and $\alang(\fsa_{loop})\neq\emptyset$. Also,
$\aword'=\aseg_1(\aloop_1)^{\vect{y}[1]}\ldots\aseg_{k-1}(\aloop_{k-1})^{\vect{y}[k-1]}\aseg_k\aloop_k[1,j]\in g(\alang(\fsa_p))$. Since,
$\alang(\fsa_{loop})\neq\emptyset$, there exists a word
$\aword''=\aloop_k[j+1,\length{\aloop_k}]\aloop_k^{n}\aloop_k[1,j]\in\alang(\fsa_{loop})$. Consider the word
$\aword=\aword'.(\aword'')^{\omega}$. Clearly, $\aword\in\alang(\acps)$. Also, note that $\aword'$ has a run $\arun'$ starting from $\astate_i$ to
$\astate_f$ and $\aword''$ has a run $\arun''$ starting from $\astate_f$ to $\astate_f$. Thus, we can compose $\arun=\arun'\arun''^{\omega}$ to obtain
a run for $\aword$. Note that $\arun$ follows transitions from $\edges$ and visits $\astate_f\in F$ infinitely many times. Thus,
$\aword=\aseg_1(\aloop_1)^{\vect{y}[1]}\ldots\aseg_{k-1}(\aloop_{k-1})^{\vect{y}[k-1]}\aseg_k\aloop_k^{\omega}\in\alang(\bauto)$.  
\qed
\end{proof}

\begin{lemma}
Algorithm \ref{algo:BA-np} is in \ptime.
\end{lemma}
\begin{proof}
Note that the number of times the for loop executed is at most $\size{\bauto}\times\size{\acps}$. Now we will consider each iteration and show that
each iteration of the for loop can be completed in \ptime. At each iteration,
\begin{enumerate}
  \item $\fsa_1$ and $\fsa_2$ are essentially copies of $\bauto$. Thus, $\size{\fsa_1}=\size{\fsa_2}=\bauto$ and their construction takes \ptime.
  \item Construction of $\fsa_p$ and $\fsa_{loop}$ amounts to essentially constructing an intersection automaton from two automaton of size
    $\size{\bauto}$ and $\size{\aseg_1(\aloop_1)\cdots\aseg_k\aloop_k}$. Thus, $\size{\fsa_p}$ and $\size{\fsa_{loop}}$ is bounded by
    $\size{\bauto}\times\size{\acps}$.
  \item Construction of $\aformulabis(\avariable_{1}\cdots,\avariable_{k-1})$ can be done in time $\size{\fsa_p}^2$ thanks to the following theorem
    \begin{theorem}\cite{Verma&Seidl&Schwentick05}
      \label{thm:parikh}
      Given a finite state automaton $\fsa$, let $\aformula$ be the exsistential Presburger formula characterizing the Parikh image of
      $\alang(\fsa)$. $\aformula$ can be
      \begin{itemize}
       \item constructed in time bounded by $\size{\fsa}^{2}$.
       \item the greatest absolute value of the constant in $\aformula$ is bounded by $\size{\fsa}$.
      \end{itemize}
    \end{theorem}
  \item Checking $\vect{y}\models\aformulabis(\avariable_{1}\cdots,\avariable_{k-1})$ can be done in time bounded by
    $\size{\aformulabis(\avariable_{1}\cdots,\avariable_{k-1})}+\size{\vect{y}}$ and checking $\fsa_{loop}\neq\emptyset$ can be done in time
    $\size{\fsa_{loop}}^2$.
\end{enumerate}
Thus, the whole procedure can be completed in time bounded by $(\size{\bauto}\times\size{\acps})^3$.
\qed
\end{proof}
Thus, we have the following lemma,
\begin{lemma} 
Membership problem with \buchi~automata is \ptime.
\end{lemma}

\begin{corollary} \label{corollary-intersection-ba}
The intersection non-emptiness problem with \buchi~automata is \np-complete. 
\end{corollary}  

\np~upperbound is obtained by the fact that we guess a polynomial size vector $\vect{n}$ to obtain a path in $\alang(\acps)$.
\np-hardness follows from the \np-hardness of solving a quantifier-free Presburger formula.

It remains to  show that MC(BA,$\flatcs$) is \np-Complete too! Remember also that when counter systems are involved \buchi~automata includes 
guards. Let us start by briefly explaining what we mean by a \buchi~automata recognising runs from flat counter
systems. 


\buchi~automata recognising infinite runs of counter systems are defined as \buchi~automata over a finite alphabet from
Section~\ref{section-FO-definition} except that the alphabet set is changed in this case. In this case the \buchi~automata defines a specification for
the constrained alphabet $\triple{at}{at_n}{\powerset{at \cup ag_n}}$. Note that the alphabet can be of exponential size in the size of $\bauto$ if we
follow the developments from Section~\ref{section-model-checking-problem}. But in fact we only need to consider the set of alphabets $\aalphabet$
which appear in $\acps$ and $\bauto$. Hence, $\size{\aalphabet}$ is polynomial in the size of input. By Theorem~\ref{theorem-reduction} and following
the abstract algorithm from Section~\ref{section-main-reduction},
\begin{itemize}
\itemsep 0 cm 
\item $\asys, \aconf_0 \models \aformula$,
\item there is a constrained path schema $\acps$ of polynomial size
      over some constrained alphabet  $\triple{at}{ag_n}{\aalphabet'}$
      such that $\alang(\acps) \cap \alang(\bauto)\neq\emptyset$.
\end{itemize}
By Corollary~\ref{corollary-intersection-ba} applied on the instance
with $\acps$ and $\bauto$ and since $\acps$ and $\bauto$ is of polynomial size in $N$ , we get a \np~decision
procedure.

\begin{theorem} \label{theorem-ba-pspace-complete}
MC(BA, $\flatcs$) is \np-complete. 
\end{theorem}

\np-hardness comes from the fact that one can encode any quantifier-free Presburger formula in the guard of a flat counter system, where finding a run
satisfying the guard is equivalent to finding a solution to the Presburger formula.


==> subsection-example.tex <==
\subsection{Example}
\begin{figure}
\begin{center}
\scalebox{0.9}{
\begin{tikzpicture}[shorten >=1pt,node distance=1.7cm,auto,>=stealth']

  \node[state] (q_1)                  {$\astate_1$};
%  \node (a1)[above=0.3cm of q_1]  {\fbox{{\bf \tiny  $\alpha$}}};
  \node[state]         (q_2)  [right=of q_1]  {$\astate_2$};
%  \node (a2)[above=0.3cm of q_2]  {\fbox{{\bf \tiny  $\geq 1$}}}; 
  \node[state]         (q_3)  [right=of q_2]  {$\astate_3$};
  \node[state]         (q_4)  [below=of q_2]  {$\astate_{4}$};
  \node[state]         (q_5)  [right=of q_3]  {$\astate_5$};
  \path[->] (q_1)   edge              node  {$\top,(0,0)$} (q_2)
                    edge [swap]       node  {$\top,(0,0)$} (q_4)
            (q_2)   edge              node  {$\top,(0,0)$} (q_3)
	    	    edge [out=125,in=55,loop]       node  {$\top,(-3,0)$} ()
            (q_3)   edge [swap,bend right] node  {$\top,(1,0)$} (q_5)
            (q_5)   edge [swap,bend right] node  {$\top,(0,1)$} (q_3)
            (q_4)   edge [swap]       node  {$\top,(0,0)$} (q_3)
	    	    edge [out=125,in=55,loop]       node  {$\top,(0,-2)$} ();
\end{tikzpicture}
}
\end{center}
\caption{A flat counter system}
\label{example}
\end{figure}
Consider the flat counter system in Figure~\ref{example} with two counters and the labelling function $\alabelling(\astate_3)=\{p,q\}$ and
$\alabelling(\astate_5)=\{p\}$. We would like to check whether there exists infinite runs where after a position in the run, all even positions has
the same value for counter 1 and counter 2 and propositional variable $p$ is true. For this, we construct the linear $\mu$-caluclus formula
$\aformula=\mu\avar_1.(\mynext(\nu\avar_2.(p\wedge\avariable_1-\avariable_2=0\wedge\mynext\mynext\avar_2)\vee\mynext\avar_1)$. Clearly, as per the labelling of
the flat counter system, such a position occurs in any run after it reaches $\astate_3$ with same value in both the counters. Again, to reach
$\astate_5$, it is clear that the run starts with the initial configuration, $\tuple{\astate_1,\vect{v}}$, where $\vect{v}$ should satisfy the
Presburger equation $\aconstraintsystem=\exists y.(\avariable_1=3.y+\avariable_2)\vee(\avariable_2=2.y+\avariable_1)$.


==> subsection-muAlgo1.tex <==
\subsection{\pspace~Algorithm for model-checking of $\lmc$ sentences}

The goal of this section is to characterize the complexity of the model-checking problem over flat counter systems with linear $\mu$ calculus. We will
establish the existence of $\amap_{\mu{\rm TL}}$ for the intersection non-emptiness problem with linear $\mu$ calculus by using the bound obtained in
Theorem~\ref{thm:stuttering-buchi}. For this we transform a given $\lmc$ sentence $\aformula$ to an equivalent \buchi~automaton using the following
theorem,
\begin{theorem}\cite{Vardi88}
\label{thm:vardi}
Given an $\lmc$ sentence $\aformulabis$, we can construct a \buchi~automaton $\bauto_{\aformulabis}$ over the alphabet $\aalphabet=\powerset{\varprop}$,
whose number of states is bounded by $\powerset{19.\size{\aformulabis}^4}$ such that for any $\omega$-word $\aword\in\aalphabet^{\omega}$,
$\aword\in\alang(\bauto_{\aformulabis})$ iff $\aword\models\aformulabis$.
\end{theorem}
Thanks to Theorem~\ref{thm:vardi} and Theorem~\ref{thm:stuttering-buchi}, we have the following lemma.
\begin{lemma}
\label{map-mu}
Let $\acps$ be a constrained path schema and $\aformulabis$ be a $\lmc$ sentence.
If $\alang(\acps) \cap \alang(\aformulabis)$ is non-empty, then there is an $\omega$-word in 
$\alang(\acps) \cap \alang(\aformulabis)$ such that each loop is taken at most a number of times
bounded by
$$
2^{(19.\size{\acps}.\size{\aformulabis}^4) + p_1(\size{\acps}) + p_2(\size{\acps})}. 
$$
\end{lemma}

Note that this implies that $\amap_{\mu{\rm TL}}(\aformulabis,\acps)$ can take the value $2^{(19.\size{\acps}.\size{\aformulabis}^4) +
  (p_1+p_2)(\size{\acps})}$.

So, checking whether  $\alang(\acps) \cap \alang(\aformulabis)$  is non-empty amounts to guess some
$\vect{n} \in \interval{0}{2^{(19.\size{\acps}.\size{\aformulabis}^4) + (p_1+p_2)(\size{\acps})}}^{k-1}$ and check
whether 
$$\aword = \aseg_1 (\aloop_1)^{\vect{n}[1]} \cdots \aseg_{k-1} (\aloop_{k-1})^{\vect{n}[k-1]} \aseg_k (\aloop_k)^{\omega} \in 
\alang(\acps) \cap \alang(\aformulabis).
$$ 
Checking whether $\aword \in \alang(\acps)$ can be done in polynomial time in $(19.\size{\acps}.\size{\aformulabis}^4) + (p_1+p_2)(\size{\acps})$
(and therefore in polynomial time in $\size{\aformulabis} + \size{\acps}$) since this amounts to verify whether $\vect{n} \models \aformula$.
Checking whether $\aword \in \alang(\aformulabis)$ can be done in exponential space in $\size{\aformulabis} + \size{\acps}$ by converting
$\aformulabis$ to an exponential size \buchi~automaton, $\bauto_{\aformulabis}$ using Theorem~\ref{thm:vardi} and applying Algorithm~\ref{algo:BA-np}
for the membership problem of \buchi~automata. Hence, this leads to a nondeterministic exponential space decision procedure
for the intersection non-emptiness problem but it is possible to get down to nondeterministic polynomial space as explained below.

Clearly, to obtain a nondeterministic polynomial space algorithm for we can not construct $\bauto_{\aformulabis}$ explicitly. Thus, we would like to
do an ``on-the-fly'' construction of $\bauto_{\aformulabis}$ where we only need to store only polynomial size information at any point of simulating
the algorithm. We will essentially show that the construction of $\bauto_{\aformulabis}$ presented in \cite{Vardi88}, can be done efficiently, such
that while simulating it on a word we only need to store polynomial size information. For this, we will first define a 2-way \buchi~automaton which is
used in the constuction of the \buchi~automaton given in \cite{Vardi88}.

A 2-way \buchi~automaton represented as $\bauto_2=\tuple{\states_2,\aalphabet',\edges_2,\states^i_2,F_2}$, where $\states_2$ is the set of states,
$\states^i_2,F_2\subseteq\states_2$, $\edges_2:\states_2\times\aalphabet\rightarrow\powerset{\states_2\times\{-1,0,1\}}$. That is, for every
transition, the automaton goes to another state and move right, left or stay at the same position in the word. A \defstyle{configuration} of
$\bauto_{2}$ is a member of $\states_2\times\nat$, a pair consisting of a state and a ``position''. A \defstyle{run}
$r\in(\states_2\times\nat)^{\omega}$ of $\bauto_2$ over an infinite word $\aword\in\aalphabet^{\omega}$ is an infinite sequence of configuration such
that $r(0)\in\states^2_i\times\{0\}$, and for all $i\geq 0$ if $r(i)=(s,j)$, then there is some $(t,k)\in\edges_2(s,w(j))$ such that
$r(i+1)=(t,j+k)$. As usual $r$ is an \defstyle{accepting} run if for infinitely many $i$'s we have $r(i)\in F_2\times\nat$.

To simulate a 2-way \buchi~automaton by a 1-way \buchi~automaton, we define \defstyle{A-labellings} in the style of \cite{Vardi88}. Let
$\aalphabet_A=\states_2^2\times\{0,1\}$, i.e, pairs of states tagged by 0 or 1. Intuitively, a tuple $(s,t,0)$ denote the fact that there is a
backward run from the present position starting at state $s$ and ending in the present position in state $t$. $1$ instead of $0$ in the tuple, denotes
that the run passes through a state in $F_2$. An $A-labelling$ $l\in(\powerset{\aalphabet_A})^{\omega}$ for an infinite word
$\aword\in(\aalphabet')^{\omega}$ is an infinite sequence of sets of alphabets from $\aalphabet_A$ that satisfy the following conditions, denoted as
$\aninv_1$, for any state $s,t\in\states_2$:
\begin{itemize}
  \item $(s,t,0)\in l(i)$ iff either $(t,0)\in\edges_2(s,\aword(i))$ or $i>1$ and there are states $s',t'\in \states_2$ such that $(s',t',j)\in
    l(i-1)$, $(s',-1)\in\edges_2(s,\aword(i))$ and $(t,1)\in\edges_2(t',w(i-1))$.
  \item $(s,t,1)\in l(i)$ iff either $(t,0)\in\edges_2(s,\aword(i))$ and $t\in F_2$ or $i>1$ and there are states $s',t'\in \states_2$ such that $(s',t',j)\in
    l(i-1)$, $(s',-1)\in\edges_2(s,\aword(i))$ and $(t,1)\in\edges_2(t',w(i-1))$ and in addition either $j=1$ or one of $s',t',t$ is in $F_2$.
  \item $(s,t,0)\in l(i)$ iff there is a sequence $s_0,\ldots,s_k\in\states_2$, $k>0$, such that $s_0=s,s_k=t$ and $(s_j,s_{j+1},0)\in l(i)$ for $0\geq j>k$.
  \item $(s,t,1)\in l(i)$ iff there is a sequence $s_0,\ldots,s_k\in\states_2$, $k>0$, such that $s_0=s,s_k=t$ and $(s_j,s_{j+1},a_j)\in l(i)$ for
    $0\geq j>k$ and either one of the $a_j$ is 1 or one of the $s_j\in F_2$ for $j>0$.
\end{itemize}
\begin{theorem}\cite{Vardi88}
\label{thm:2to1}
Given a 2-way \buchi~automaton $\bauto_2$ over $\aalphabet'$, we can construct an 1-way \buchi~automaton $\bauto_{\aword}$ with $2\times|\states_2|$
states such that for any word $\aword\in(\aalphabet')^{\omega}$ and it's valid $A-labelling$ $l\in(\powerset{\aalphabet_A})^{\omega}$,
$(\aword,l)\in\alang(\bauto_{\aword})$ iff $\aword\in\alang(\bauto_2)$.
\end{theorem}
As a corollary from the above theorem and applying the result from \cite{Sistla&Vardi&Wolper87}, we get,
\begin{corollary}
\cite{Sistla&Vardi&Wolper87}
\label{cor:complement}
Given a 2-way \buchi~automaton $\bauto_2$ over $\aalphabet'$, we can construct a 1-way \buchi~automaton $\overline{\bauto_{\aword}}$ such that
\begin{enumerate}
  \item for any word $\aword\in(\aalphabet')^{\omega}$ and it's valid $A-labelling$
    $l\in(\powerset{\aalphabet_A})^{\omega}$, $(\aword,l)\notin\alang(\bauto_{\aword})$ iff $\aword\in\alang(\bauto_2)$.
  \item the size of each state of $\bauto_{\aword}$ is polynomial in the size of $\bauto_2$,
  \item it can be checked if a state is initial in space polynomial in the size of $\bauto_2$,
  \item it can be checked if a state is designated in space polynomial in the size of $\bauto_2$,
  \item each transition of $\bauto_{\aword}$ can be checked in space polynomial in the size of $\bauto_2$.
\end{enumerate}
\end{corollary}
Note that the number of states in $\overline{\bauto_{\aword}}$ is bounded by $16^{n^2}$ where $n$ is the number of states in $\bauto_2$.

For checking the validity of an $A-labelling$, with respect to any word $\aword\in(\aalphabet')^{\omega}$, we would construct another 1-way
\buchi~automaton $\bauto_l$ which reads the word $\aword$ and at each position the $A-labelling$ is stored in the state of $\bauto_l$. Note that at
any position $i$ in $\aword$, to determine the $A-labelling$ at $i$, $\bauto_l$ has only to remember $\aword(i-1)$ and the $A-labelling$ of position
$i$ to check the conditions of $\aninv_1$. Thus, $\bauto_l$ represented by the tuple $\tuple{\states_l,\aalphabet',\edges_l,\states^i_l,F_l}$, where
$\states_l=\aalphabet'\times\powerset{\aalphabet_A}$ is the set of states, $\states^i_l,F_l\subseteq\states_l$, $\edges_l$ is defined
according to the condition of $\aninv_1$. Here, the sequence of states in the run of $\bauto_l$ over a word $\aword$ gives the valid $A-labelling$,
$l$ of $\aword$. The number of staes in $\bauto_l$ is at most $|\aalphabet'|\times 4^{n^2}$ where $n$ is the number of states in $\bauto_2$.

In \cite{Vardi88}, the 2-way \buchi~automaton is used to check for ``well-foundedness'' of a model for fixpoint operators. Whereas the satisfiability
of a given formula $\aformula$ over a model is checked by a simple \buchi~automaton. We will now describe the construction of such a \buchi~automaton,
$\bauto_T$ in the line of \cite{Vardi88}. To define $\bauto_T$ for $\lmc$ sentence $\aformula$, we will define a few notations. Let $cl(\aformula)$
denote the Fischer-Ladner closure of $\aformula$ and $\vect{a}$ as a ``consistent'' subset of $cl(\aformula)$. Let the set of all such consistent
subset of $cl(\aformula)$ is denoted by $at(\aformula)$. Clearly, $at(\aformula)$ is exponential in the size of $\aformula$. For each $\vect{a}$, we
join a \defstyle{choice function} $\aformulabis$, which is a partial function on $cl(\aformula)$ defined on every disjunct in $cl(\aformula)$ and
returns one of the disjuncts. Set of all such possible pairs is denoted by $adat(\aformula)$. Now we define
$\bauto_T=\tuple{\states_T,\aalphabet,\edges_T,\states^i_T,F_T}$ where, $\states_T=\{start\}\cup adat(\aformula)\times\{0,1\}$,
$\states^i_T=\{start\}$, $F_T=adat(\aformula)\times\{1\}$. The transition function $\edges_T$ is defined as:
\begin{itemize}
  \item $\edges_T((start),c)$ for any $c\in\aalphabet$ is the set $\{(\vect{a},\aformulabis,j)\}$ such that for all $p\in\varprop$, $p\in \vect{a}$
    iff $p\in c$, $\vect{a}$ does not contain any formula of the form $\myprevious \aformula'$ and $j=1$ iff $\aformula\in\vect{a}$.
  \item $\edges_T((\vect{b},\aformulabis',i),c)$ for any $c\in\aalphabet$ is the set $\{(\vect{a},\aformulabis,j)\}$ such that for all $p\in\varprop$,
    $p\in \vect{a}$ iff $p\in c$, $j=1$ iff $\aformula\in\vect{a}$ or $i=1$ and the following holds:
    \begin{itemize}
      \item if $\mynext\aformula'\in\vect{b}$ then $\aformula'\in\vect{a}$
      \item if $\myprevious\aformula'\in\vect{a}$ then $\aformula'\in\vect{b}$
    \end{itemize}
\end{itemize}
Now we can give the construction for the \buchi~automaton recognising the models of a given $\lmc$ sentence.
\begin{lemma}
\label{thm:mu}
Given a $\lmc$ sentence $\aformula$, we can construct a \buchi~automaton $\bauto_{\aformula}$ over the alphabet $\aalphabet$, such that 
\begin{enumerate}
  \item $\alang(\bauto)$ is exactly the set of models for $\aformula$.
  \item the size of each state of $\bauto_{\aformula}$ is polynomial in the size of $\aformula$,
  \item it can be checked if a state is initial in space polynomial in the size of $\aformula$,
  \item it can be checked if a state is designated in space polynomial in the size of $\aformula$,
  \item each transition of $\bauto_{\aformula}$ can be checked in space polynomial in the size of $\aformula$.
\end{enumerate}
\end{lemma}
\begin{proof}
Given a $\lmc$ sentence $\aformula$, we first construct the 2-way \buchi~automaton $\bauto_2$ over the alphabet $adat(\aformula)$ looking for not
well-foundedness with states at most $|cl(\aformula)|^2$ as described in \cite{Vardi88}. Also, we can construct $\bauto_{\aword}$ with
$2|cl(\aformula)|^2$ states with the properties stated in Theorem~\ref{thm:2to1}. Intuitively, we would like to have a \buchi~automaton, such that for
the models of $\aformula$, there is an accepting run of $\bauto_T$ and the word described by the states of the run of $\bauto_T$ is accepted by
$\bauto_l$ and $\overline{\bauto_{\aword}}$. Let us assume the definitions of the three automata as before:
\begin{itemize}
  \item $\bauto_T=\tuple{\states_T,\aalphabet,\edges_T,\states^i_T,F_T}$ where $\states_T=\{start\}\cup adat(\aformula)\times\{0,1\}$
  \item $\bauto_l=\tuple{\states_l,adat(\aformula),\edges_l,\states^i_l,F_l}$ where $\states_l=adat(\aformula)\times\powerset{\aalphabet_A}$
  \item $\overline{\bauto_{\aword}}=\tuple{\states_{\aword},adat(\aformula)\times\powerset{\aalphabet'},\edges_{\aword},\states^i_{\aword},F_{\aword}}$
\end{itemize}
\marginpar{Please check the construction}
We construct $\bauto_{\aformula}=\tuple{\states,\aalphabet,\edges,\states^i,F}$, where
$\states=\states_T\times\states_l\times\states_{\aword}\times\{1,2,3\}$, $\states^i=\states^i_T\times\states^i_l\times\states^i_{\aword}\times\{1\}$,
$F=\states_T\times\states_l\times F_{\aword}\times\{3\}$ and
$\tuple{(\astate_T,\astate_l,\astate_{\aword},i),c,(\astate'_T,\astate'_l,\astate'_{\aword},j)}\in\edges$ if:
\begin{enumerate}
  \item $\astate_T,\astate'_T\in \states_T$, $\astate_l,\astate'_l\in \states_l$, $\astate_{\aword},\astate'_{\aword}\in \states_{\aword}$ and $c\in\aalphabet$.
  \item $\astate'_T\in\edges_T(\astate_T,c)$.
  \item $\astate'_l\in\edges_l(\astate_l,s)$ where $\astate'_T=\tuple{s,i}$, $s\in adat(\aformula)$.
  \item $\astate'_{\aword}\in\edges_{\aword}(\astate_{\aword},\tuple{s,t})$ where $\astate'_T=\tuple{s,i}$, $s\in adat(\aformula)$ and
    $\astate'_l=\tuple{s',t}$, $s'\in adat(\aformula),t\in\powerset{\aalphabet_A}$ 
  \item $j=2$ if $i=1$ and $\astate'_T\in F_T$, $j=3$ if $i=2$ and $\astate'_l\in F_l$, $j=1$ if $i=3$ and $\astate'_{\aword}\in F_{\aword}$ and $j=i$ otherwise.
\end{enumerate}
We will now prove each of the property in the lemma for $\bauto_{\aformula}$.
\begin{enumerate}
  \item Clearly, since the construction is on the same line as \cite{Vardi88}, by Theorem~\ref{thm:vardi}, $\bauto_{\aformula}$ accepts only the words
    which satisfies $\aformula$.
  \item Note that $\size{\states_T}$ is $2.\size{adat(\aformula)}$ which is atmost exponential in $\size{\aformula}$ as mentioned before. Similarly,
    from \cite{Vardi88}, we get that $\size{\states_l}=\size{adat(\aformula)}\times 4^{\size{cl(\aformula)}^4}$ which again is atmost exponential in
    $\size{\aformula}$. From Corollary~\ref{cor:complement}, we get that the size of states of $\overline{\bauto_{\aword}}$ is polynomial in
    $\size{\bauto_{\aword}}$ which again is at most $2|cl(\aformula)|^2$. Thus, $\size{\states}$ is atmost exponential in $\size{\aformula}$. Hence,
    each state is of size polynomial in the size of $\aformula$.
  \item $\bauto_T$ has a designated initial state $(start)$ and by Corollary~\ref{cor:complement},we can check the initial state of $\bauto_{\aword}$
    in space polynomial in $\size{\aformula}$. For $\bauto_l$, notice that checking for initial state amounts to the check of first 2 conditions in
    $\aninv_1$, which can be done in space polynomial in $\size{\aformula}$. Thus, the initial state $\states^i$ can be checked in polynomial space.
  \item As previous, a designated state can be checked in space polynomial in the size of $\aformula$.
  \item For checking a transition $\tuple{(\astate_T,\astate_l,\astate_{\aword},i),c,(\astate'_T,\astate'_l,\astate'_{\aword},j)}$ belongs to
    $\edges$, we will show all the checks could be performed in space polynomial in $\size{\aformula}$.
    \begin{itemize}
      \item As before checking $\astate_T,\astate'_T\in \states_T$, $\astate_l,\astate'_l\in \states_l$, $\astate_{\aword},\astate'_{\aword}\in
        \states_{\aword}$ can be done in polynomial space.
      \item From the definition of $\edges_T$, checking $\astate'_T\in\edges_T(\astate_T,c)$ requires atmost only to store $\astate'_T,\astate_T$ and
        $c$. Thus, it requires only polynomial space.
      \item Similarly from the definition of $\edges_l$ checking $\astate'_l\in\edges_l(\astate_l,s)$ requires storing $\astate'_l,\astate_l$ and $s$
        and hence can be done in polynomial space.
      \item For checking $\astate'_{\aword}\in\edges_{\aword}(\astate_{\aword},\tuple{s,t})$ where $\astate'_T=\tuple{s,i}$, $s\in adat(\aformula)$
        and $\astate'_l=\tuple{s',t}$, $s'\in adat(\aformula),t\in\powerset{\aalphabet_A}$, we first construct $\bauto_{\aword}$ whose size is atmost
        $2|cl(\aformula)|^2$ polynomial in $\size{\aformula}$. Then by Corollary~\ref{cor:complement}, we can check it for $\overline{\bauto_{\aword}}$
        in space polynomial in $\size{\aformula}$.
    \end{itemize}
\end{enumerate}
\qed
\end{proof}

Below, we show that the membership problem with linear $\mu$ caluclus can be solved in
polynomial space in $\size{\acps} + \size{\aformulabis}$. 
Let $\acps$,  $\aformulabis$ and $\vect{n} \in \Nat^{k-1}$ be an instance of the problem.
For $i \in \interval{1}{k-1}$, let $\vect{n}'[i] \egdef \mathtt{min}(\vect{n}[i],2^{(19.\size{\acps}.\size{\aformulabis}^4) + (p_1+p_2)(\size{\acps})})$. 
By  Theorem~\ref{thm:vardi} and Theorem~\ref{thm:stuttering-buchi},  the propositions below are equivalent:
\begin{itemize}
\item  $\aseg_1 (\aloop_1)^{\vect{n}[1]} \cdots \aseg_{k-1} (\aloop_{k-1})^{\vect{n}[k-1]} \aseg_k (\aloop_k)^{\omega} \in 
\alang(\aformulabis)$,
\item $\aseg_1 (\aloop_1)^{\vect{n}'[1]} \cdots \aseg_{k-1} (\aloop_{k-1})^{\vect{n}'[k-1]} \aseg_k (\aloop_k)^{\omega} \in 
\alang(\bauto_{\aformulabis})$.
\end{itemize}
Without any loss of generality, let us assume then that 
$\vect{n} \in \interval{0}{2^{(19.\size{\acps}.\size{\aformulabis}^4) + (p_1+p_2)(\size{\acps})}}^{k-1}$. 

We would actually check that $\aseg_1 (\aloop_1)^{\vect{n}[1]} \cdots \aseg_{k-1} (\aloop_{k-1})^{\vect{n}[k-1]} \aseg_k (\aloop_k)^{\omega} \in
\alang(\bauto_{\aformulabis})$. For this we try to find a ``lasso'' structure as is done in the membership problem for \buchi~automaton. Let
$\aword=\aseg_1 (\aloop_1)^{\vect{n}[1]} \cdots \aseg_{k-1} (\aloop_{k-1})^{\vect{n}[k-1]} \aseg_k (\aloop_k)^{\omega}$ and
$\bauto_{\aformulabis}=\tuple{\states,\aalphabet,\edges,\states^i,F}$. Since $F$ is finite and in an accepting run we should see infinitly many times
a state from $F$, at least one $\astate_f\in F$ appears infinitely many times in the accepting run of $\aword$ if
$\aword\in\bauto_{\aformulabis}$. Again, only $\aloop_k$ is taken infinitly many times in $\aword$ and so there exists at least one position $j$ in
$\aloop_k$ such that the transition from $\astate_f$ reading $\aloop_k(j)$ is taken infinitely many times. For this reason, we guess a state
$\astate_f\in F$ and a position $j\in[1,\length{\aloop_k}]$ and decompose $\aword$ as $\aword'=\aseg_1 (\aloop_1)^{\vect{n}[1]} \cdots \aseg_{k-1}
(\aloop_{k-1})^{\vect{n}[k-1]} \aseg_k \aloop_k[1,j]$ and $\aword''=\aloop_k[j+1,\length{\aloop_k}](\aloop_k)^*\aloop_k[1,j]$. Also, as in
Algorithm~\ref{algo:BA-np}, we construct two finite state automata as $\fsa_f=\tuple{\states,\aalphabet,\edges,\states^i,\{\astate_f\}}$ and
$\fsa_l=\tuple{\states,\aalphabet,\edges,\{\astate_f\},\{\astate_f\}}$. Intuitively, $\fsa_f$ checks that we reach $\astate_f$ from an initial state
on reading $\aword'$ and $\fsa_l$ checks that there is a way to reach $\astate_f$ from $\astate_f$ by only repeating $\aloop_k$. Thus, as in the proof
of correctness of Algorithm~\ref{algo:BA-np}, $\aword\in\alang(\bauto_{\aformulabis})$ iff $\aword'\in\alang(\fsa_f)$ and
$\alang(\aword'')\cap\alang(\fsa_l)\neq\emptyset$. Polynomial space algorithm is obtained by performing the two checking in polynomial space. Checking
$\aword'\in\alang(\fsa_f)$ is done by simulating $\fsa_f$ on $\aword'$. One can check in polynomial time what is the $i$th letter of $\aword'$ and
thanks to Theorem~\ref{thm:mu} the simulation of $\fsa_f$ can be done in polynomial space. For checking
$\alang(\aword'')\cap\alang(\fsa_l)\neq\emptyset$, note that the finite state automata $\fsa_r$ corresponding to $\aword''$ is polynomial in the size
of $\acps$ and have a single initial and final state. Thus, checking $\alang(\aword'')\cap\alang(\fsa_l)\neq\emptyset$ amounts to finding a path from
the single initial state to the single final state in $\fsa_r\cap\fsa_l$. By Theorem~\ref{thm:mu} and since the problem of finding a path in directed
graph is in \nlogspace, this can be done in polynomial space too.

\begin{lemma} 
Membership problem with linear $\mu$ calculus is \pspace-complete and it can be solved in polynomial space in $\size{\acps} + \size{\aformulabis}$.
\end{lemma}

\pspace-hardness follows from ??.\marginpar{was there a PSPACE-hardness proof for it?}

\begin{corollary} \label{corollary-intersection-mu}
The intersection non-emptiness problem with linear $\mu$-calculus is \pspace-complete. 
\end{corollary}  

It remains to  show that MC($\lmc$,$\flatcs$) is in \pspace \ too ! Remember also that when counter systems are involved $\lmc$ includes 
guards. Let us start by briefly explaining what we mean by $\lmc$ when runs from flat counter
systems are involved. 


$\lmc$ formulae interpreted over infinite runs of counter systems are defined similarly as FO formulae over a counter system from Section~4.3.  The
atomic formulae of the form $\aletter$ are replaced by atomic formulae of the form $\avarprop$ or $\aguard$ where $\avarprop$ is
an atomic formula or $\aguard$ is an atomic guard from $\guards(\counters_n)$. Hence, a formula $\aformula$ built over atomic formulae from a finite
set $at$ of atomic propositions and from a finite set $at_n$ of atomic guards from $\guards(\counters_n)$ defines a specification for the constrained
alphabet $\triple{at}{at_n}{\powerset{at \cup ag_n}}$. Note that the alphabet can be of exponential size in the size of $\aformula$ and
$\avarprop$ actually corresponds to a disjunction $\bigvee_{\avarprop \in \aletter} \aletter$ if we follow the developments from
Section~\ref{section-model-checking-problem}. Following the same procedure as in the case of FO in Section 4.3 and using the abstract algorithm from
Section~\ref{section-main-reduction}, we get a procedure for deciding the problem MC($\lmc$,$\flatcs$). Using
Corollary~\ref{corollary-intersection-mu} and Savitch's theorem, we get,
\begin{theorem} 
MC($\lmc$, $\flatcs$) is \pspace-complete. 
\end{theorem}



==> subsection-stuttering.tex <==
\subsection{Stuttering theorem for $FO_{\varprop}$}
In this section, we will prove that if in an $\omega$-sequence $\aword$, a subword $\mathbf{s}$ is repeated consecutively a large number of times then this $\omega$-word and other $\omega$-words obtained by removing some of the repetitions of $\mathbf{s}$ satisfy the same set of $FO_{\varprop}$ formulae, this is what we call the stuttering theorem for $FO_{\varprop}$. Such a result will allow us to bound the repetition of iteration of loops in path schema and thus to obtain a model-checking algorithm for the logic $FO_{\varprop}$ optimal in complexity. In order to prove the stuttering theorem, we will use EF games.

In the sequel we consider a natural $N \geq 2$ and two $\omega$-words over $\powerset{\varprop}$ of the following form $\aword = \aword_1 \mathbf{s}^M \aword_2, \aword'= \aword_1 \mathbf{s}^{M+1} \aword_2 \in (\Sigma)^{\omega}$ with $M > 2^{N+1}$ and $\mathbf{s}$ a non-empty finite word. We will now show that the game $EF_N(\astruct,\bstruct)$ is winning. The strategy for Duplicator will work as follows: at the $i$-th round (for $i \leq N$), if the point chosen by the Spoiler is close (upto a distance of $2^{N-i}$) to another previously chosen position then the Duplicator will chose a point in the other word at the exact same distance from the corresponding position and if the point is far (at a distance greater thatn $2^{N-i}$) from any other position  then in the other word the Duplicator will chose a position also far away from any other position. 

Before to provide a winning strategy for the Duplicator we define define some invariants on any $i$-round play (with $i \leq N$) that will be maintained by the Duplicator's strategy. In order to define this invariant and the Duplicator's strategy, let us mark the following positions $a_{-1}=b_{-1}=|\aword_1|$,
$a_{0}=|\aword_1\mathbf{s}^{M}|$ and $b_{0}=|\aword_1\mathbf{s}^{M+1}|$. Note that these are the positions where the repetition of $\mathbf{s}$ starts
respectively ends in each word.
 Given a play $i$-round play $Pl_i=(p_1,a_1,b_1)(p_2,a_2,b_2)\cdots(p_i,a_i,b_i)$, for each $j \in \interval{1}{i}$ such that $a_{-1} < a_j < a_{0}$, we define $\lef{a_j}=\max(a_k \mid k \in \interval{-1}{i} \mbox{ and } a_k < a_j)$ and $\rig{a_j}=\min(a_k \mid k \in \interval{-1}{i} \mbox{ and } a_j < a_k)$ (ie $\lef{a_j}$ and $\rig{a_j}$ are the closest neighbor of $a_j$). We define similarly $\lef{b_j}$ and $\rig{b_j}$. We will then say that the $i$-round play $Pl_i$ respects the invariant $\aninv$ iff the following conditions are satisfied for all $j,k \in \interval{1}{i}$:
%Consider the following invariants at round $i$, of the game. The invariant $\aninv(i)$ consists of the following
%conditions for all $\alpha\in[1,i]$,
\begin{enumerate}
  \item $a_{j} \leq a_{-1}$ iff  $b_{j} \leq b_{-1}$, and in this case  $a_{j}=b_{j}$ 
  \item $a_0 \leq a_j$ iff $b_0 \leq b_j$, and in this case $a_{j}-a_0=b_{j}-b_0$
  \item $a_{j}<a_{k}$ if and only if $b_{j}<b_{k}$
  \item if $a_{-1} < a_j < a_{0}$ (note that we have necessarily $b_{-1} < b_j < b_{0}$ )then:
    \begin{enumerate}
      \item  $a_{j}-a_{-1}=b_{j}-b_{-1}$ or $a_{0}-a_{j}=b_{0}-b_{j}$.
      \item $\rig{a_j}-a_j < 2^{N+1-i}.|\mathbf{s}|$ iff $\rig{b_{j}}-b_j< 
        2^{N+1-i}.|\mathbf{s}|$  and in this case $\rig{a_j}-a_{j} = \rig{b_j}-b_j$
      \item $ a_j-\lef{a_j} < 2^{N+1-i}.|\mathbf{s}|$ iff $b_j - \lef{b_{j}} <
        2^{N+1-i}.|\mathbf{s}|$  and in this case $a_j-\lef{a_{j}} = b_j-\lef{b_{j}}$ 
        %\item if  $\rig{a_j}-a_j > 2^{N+1-i}.|\mathbf{s}|$ and $a_j-\lef{a_j} > 2^{N+1-i}.|\mathbf{s}|$, then $a_{j}-\lef{a_j} = b_{j}-\lef{b_j}$.
            
    \end{enumerate}
%  \item For all $\alpha,\beta\in[1,i]$ $a_{\alpha}-a_{\beta}=b_{\alpha}-b_{\beta}$, whenever $a_{\alpha}-a_{\beta}\leq 2^{N-i}.|\mathbf{s}|$ or $b_{\alpha}-b_{\beta}\leq 2^{N-i}.|\mathbf{s}|$
%  \item For all $\alpha\in[1,i]$ $a_{\alpha}-|\aword_1|=b_{\alpha}-|\aword_1|$ whenever
%    $a_{\alpha}-|\aword_1|\leq 2^{N-i}.|\mathbf{s}|$ or $b_{\alpha}-|\aword_1|\leq 2^{N-i}.|\mathbf{s}|$.
%  \item For all $\alpha\in[1,i]$ $|\aword_1\mathbf{s}^{M}|-a_{\alpha}=|\aword_1\mathbf{s}^{M+1}|-b_{\alpha}$ whenever
%    $|\aword_1\mathbf{s}^{M}|-a_{\alpha}\leq 2^{N-i}.|\mathbf{s}|$ or $|\aword_1\mathbf{s}^{M+1}|-b_{\alpha}\leq 2^{N-i}.|\mathbf{s}|$.
\end{enumerate}
%
First we remark the invariant $\aninv$ is a sufficient condition for a play to be winning as stated by the following lemma.
%
\begin{lemma}
\label{lem-inv}
If a $N$-round play over $\aword$ and $\aword'$ respects $\aninv$, then it is a winning play for Duplicator.
\end{lemma}
%
\begin{proof}
Let $(p_1,a_1,b_1)(p_2,a_2,b_2)\cdots(p_N,a_N,b_N)$ be a $N$-round play over $\aword$ and $\aword'$ respecting $\aninv$. Let $i,j \in \interval{1}{N}$. First by $\aninv.3.$ we have $a_i=a_j$ iff $b_i=b_j$ and also $a_i < a_j$ iff $b_i < b_j$. We will now prove that $a_i+1=a_j$ iff $b_i+1=b_j$. First, if $a_i < a_{-1}$  or if  $a_0 \leq a_i$ this is obvious thanks to $\aninv.1$ and $\aninv.2$. Now assume $a_{-1} < a_i < a_0$, then $a_j=\rig{a_i}$ and $\rig{a_i}-{a_i} < 2.|\mathbf{s}|$, then thanks to $\aninv.4.b$ we have $a_i+1=a_j$ iff $b_i+1=b_j$.  For the last case, if $a_{-1} = a_i$, then $a_i=\lef{a_j}$ and we can conclude similarly thanks to $\aninv.4.c$. It remains now to prove that for all $i \in \interval{1}{N}$ and for $c\in \varprop$ $c\in \astruct(a_i)$ iff $c\in \bstruct(b_i)$, but this is obvious since either $a_i$ and $b_i$ are pointing at the same position in $\aword_1$ (thanks to $\aninv.1$) or at the same position in the word $\aword_2$ (thanks to $\aninv.2$) or at the same position in the word $\mathbf{s}$ (thanks to  $\aninv.4.a$). This allows us to conclude that $(p_1,a_1,b_1)(p_2,a_2,b_2)\cdots(p_N,a_N,b_N)$ is winning for Duplicator. \qed
\end{proof}
%
We define now a strategy $\hat\astrategy_D$ for Duplicator which will respect at each round the invariant $\aninv$ and this no matter what the Spoiler plays. Using the previous lemma, this will allows us to deduce that this strategy is a winning strategy for the Duplicator.Let $i \in \interval{1}{N}$ and $Pl_{i-1}=(p_1,a_1,b_1)(p_2,a_2,b_2)\cdots(p_{i-1},a_{i-1},b_{i-1})$ be a $(i-1)$-round play. First we define $b_i=\astrategy_D(Pl_i,\tuple{0,a_i})$ that is what Duplicator answers if the Spoiler chooses position $a_i$ in the $\omega$-word $\aword$. We have $b_i=\hat\astrategy_D(Pl_i,\tuple{0,a_i})$ defined as follows:
\begin{itemize}
\item If $a_i\leq a_{-1}$, then $b_i=a_i$
\item If $a_0 \leq a_{i}$, then $b_i=a_i+|\mathbf{s}|$ (same positions in word $\aword_2$)
\item If $a_{-1} < a_i < a_0$ and $a_l=\lef{a_i}$ and $a_r=\rig{a_i}$, then:
\begin{itemize}
\item  If $a_i-a_l \leq a_r-a_i$, we have $b_i=b_l+(a_i-a_l)$
\item  If $a_r-a_i < a_i-a_l$, we have $b_i=b_r-(a_r-a_i)$
\end{itemize}
%\begin{itemize}
%\item  If $a_r-a_i \leq 2^{N-i}.|\mathbf{s}|$, we have $b_i=b_r-(a_r-a_i)$
%\item  Otherwise, we have $b_i=b_l+(a_i-a_l)$.
%\end{itemize}
\end{itemize}
Similarly we have $a_i=\hat\astrategy_D(Pl_i,\tuple{1,b_i})$ defined as follows:
\begin{itemize}
\item If $b_i\leq b_{-1}$, then $a_i=b_i$
\item If $b_0 \leq b_{i}$, then $a_i=b_i-|\mathbf{s}|$ (same positions in word $\aword_2$)
\item If $b_{-1} < b_i < b_0$ and $b_l=\lef{b_i}$ and $b_r=\rig{b_i}$, then:
\begin{itemize}
\item  If $b_i-b_l \leq b_r-b_i$, we have $a_i=a_l+(b_i-b_l)$
\item  If $b_r-b_i < b_i-b_l$, we have $a_i=a_r-(b_r-b_i)$
\end{itemize}
%\begin{itemize}
%\item  If $b_r-b_i \leq 2^{N-i}.|\mathbf{s}|$, we have $a_i=a_r-(b_r-b_i)$
%\item  Otherwise, we have $a_i=a_l+(b_i-b_l)$.
%\end{itemize}
\end{itemize}
%

\begin{lemma}
\label{lem-strat-win}
For any Spoiler's strategy $\astrategy_S$ and for all $i \in \interval{0}{N}$, we have that $\play{i}{\astrategy_S,\hat\astrategy_D}{\aword,\aword'}$ respects $\aninv$.
\end{lemma}
\begin{proof}
The proof proceeds by induction on $i$. The base case for $i=0$ is obvious since the empty play respects $\aninv$. Let $\astrategy_S$ be a Spoiler's strategy and for $i \in \interval{1}{N-1}$ we assume that $\play{i-1}{\astrategy_S,\hat\astrategy_D}{\aword,\aword'}$ respects $\aninv$. Suppose that $\astrategy_S(\play{i-1}{\astrategy_S,\hat\astrategy_D}{\aword,\aword'})=\tuple{0,a_i}$ and let $b_i=\hat\astrategy_D(\play{i-1}{\astrategy_S,\hat\astrategy_D}{\aword,\aword'},\tuple{0,a_i})$. Before to probe that $\play{i}{\astrategy_S,\hat\astrategy_D}{\aword,\aword'}$ respects $\aninv$, we state some properties.

First, we prove that if $a_{-1} < a_i < a_0$ and $a_l=\lef{a_i}$ and $a_r=\rig{a_i}$, then we have $b_{-1}<b_i <b_0$ and $b_l=\lef{b_i}$ and $b_r=\rig{b_i}$ and $a_{i}-a_{-1}=b_{i}-b_{-1}$ or $a_{0}-a_{i}=b_{0}-b_{i}$. First note that by induction hypothesis and using $\aninv.2$, since $a_r < a_l$ and since there is no $m \in \interval{-1}{i-1}$ such that $a_r < a_m < a_l$, we deduce that $b_r < b_l$ and there is no $m \in \interval{-1}{i-1}$ such that $b_r < b_m < b_l$. We then proceed by the following case analysis:

\begin{enumerate}
\item \textbf{Case $a_i-a_l<  2^{N+1-i}.|\mathbf{s}|$ and $a_r-a_i < 2^{N+1-i}$}. Then we have $a_r-a_l < 2.2^{N+1-i}.|\mathbf{s}|$, ie $a_r-a_l < 2^{N+1-(i-1)}.|\mathbf{s}|$. By induction hypothesis over $\play{i-1}{\astrategy_S,\hat\astrategy_D}{\aword,\aword'}$, since $a_l=\lef{a_r}$ and $a_r=\rig{a_l}$ (note that if $a_l=a_{-1}$ or $a_r=a_0$ a similar reasoning can be done),  we also have that  $b_r-b_l < 2^{N+1-(i-1)}.|\mathbf{s}|$ and $a_r-a_l=b_r-b_l$ [using $\aninv.4.b$ and $\aninv.4.c$]. Since $a_r-a_l=b_r-b_l$, from $\hat\astrategy_D$, no matter if $a_i-a_l \leq a_r-a_i$ or $a_r-a_i < a_i-a_l$, we will have $b_r-b_i=a_r-a_i$ and $b_i-b_l=a_l-a_i$ and also $b_{-1} \leq b_l < b_i < b_r \leq b_0$. We also directly have $b_l=\lef{b_i}$ and $b_r=\rig{b_i}$. Finally since by induction hypothesis we have $a_{r}-a_{-1}=b_{r}-b_{-1}$ or $a_{0}-a_{r}=b_{0}-b_{r}$, we deduce also that $a_{i}-a_{-1}=b_{i}-b_{-1}$ or $a_{0}-a_{i}=b_{0}-b_{i}$.
\item \textbf{Case $a_i-a_l < 2^{N+1-i}.|\mathbf{s}|$ and $a_r-a_i \geq 2^{N+1-i}$ and $a_r-a_l \leq 2^{N+1-(i-1)}.|\mathbf{s}|$}. Then $b_i=b_l+(a_i-a_l)$.  By induction hypothesis over $\play{i-1}{\astrategy_S,\hat\astrategy_D}{\aword,\aword'}$, since $a_l=\lef{a_r}$ and $a_r=\rig{a_l}$ (note that if $a_l=a_{-1}$ or $a_r=a_0$ a similar reasoning can be done),  we also have that  $b_r-b_l < 2^{N+1-(i-1)}.|\mathbf{s}|$ and $a_r-a_l=b_r-b_l$ [using $\aninv.4.b$ and $\aninv.4.c$].This allows us to deduce that $b_r-b_i=a_r-a_i$ and $b_i-b_l=a_l-a_i$ and  $b_{-1} \leq b_l < b_i < b_r \leq b_0$ and $b_r-b_i \geq 2^{N+1-i}$. We also directly have $b_l=\lef{b_i}$ and $b_r=\rig{b_i}$. Finally since by induction hypothesis we have $a_{l}-a_{-1}=b_{l}-b_{-1}$ or $a_{0}-a_{l}=b_{0}-b_{l}$, we deduce also that $a_{i}-a_{-1}=b_{i}-b_{-1}$ or $a_{0}-a_{i}=b_{0}-b_{i}$.
\item \textbf{Case $a_i-a_l < 2^{N+1-i}.|\mathbf{s}|$ and $a_r-a_i \geq 2^{N+1-i}$ and $a_r-a_l \geq 2^{N+1-(i-1)}.|\mathbf{s}|$}. Then $b_i=b_l+(a_i-a_l)$.  By induction hypothesis over $\play{i-1}{\astrategy_S,\hat\astrategy_D}{\aword,\aword'}$, since $a_l=\lef{a_r}$ and $a_r=\rig{a_l}$ (note that if $a_l=a_{-1}$ or $a_r=a_0$ a similar reasoning can be done),  we also have that  $b_r-b_l \geq  2^{N+1-(i-1)}.|\mathbf{s}|$. Hence we have that $(b_r-b_i) \geq 2^{N+1-(i-1)}.|\mathbf{s}| - (b_i-b_l) \geq 2^{N+1-(i-1)}.|\mathbf{s}| -  2^{N+1-i}.|\mathbf{s}| $. From which we deduce $b_r-b_i \geq 2^{N+1-i}.|\mathbf{s}|$ This allows us to deduce that  $b_{-1} \leq b_l < b_i < b_r \leq b_0$ and $b_i-b_l=a_i-a_l$ and $b_r-b_i \geq 2^{N+1-i}$. We also directly have $b_l=\lef{b_i}$ and $b_r=\rig{b_i}$. Finally since by induction hypothesis we have $a_{l}-a_{-1}=b_{l}-b_{-1}$ or $a_{0}-a_{l}=b_{0}-b_{l}$, we deduce also that $a_{i}-a_{-1}=b_{i}-b_{-1}$ or $a_{0}-a_{i}=b_{0}-b_{i}$.
\item \textbf{Case $a_i-a_l \geq 2^{N+1-i}.|\mathbf{s}|$ and $a_r-a_i < 2^{N+1-i}$ and $a_r-a_l < 2^{N+1-(i-1)}.|\mathbf{s}|$}. Then $b_i=b_r-(a_r-a_i)$.  By induction hypothesis over $\play{i-1}{\astrategy_S,\hat\astrategy_D}{\aword,\aword'}$, since $a_l=\lef{a_r}$ and $a_r=\rig{a_l}$ (note that if $a_l=a_{-1}$ or $a_r=a_0$ a similar reasoning can be done),  we also have that  $b_r-b_l < 2^{N+1-(i-1)}.|\mathbf{s}|$ and $a_r-a_l=b_r-b_l$ [using $\aninv.4.b$ and $\aninv.4.c$].This allows us to deduce that $b_r-b_i=a_r-a_i$ and $b_i-b_l=a_l-a_i$ and  $b_{-1} \leq b_l < b_i < b_r \leq b_0$ and $b_i-b_l \geq 2^{N+1-i}$. We also directly have $b_l=\lef{b_i}$ and $b_r=\rig{b_i}$. Finally since by induction hypothesis we have $a_{l}-a_{-1}=b_{l}-b_{-1}$ or $a_{0}-a_{l}=b_{0}-b_{l}$, we deduce also that $a_{i}-a_{-1}=b_{i}-b_{-1}$ or $a_{0}-a_{i}=b_{0}-b_{i}$.
\item \textbf{Case $a_i-a_l \geq 2^{N+1-i}.|\mathbf{s}|$ and $a_r-a_i < 2^{N+1-i}.|\mathbf{s}|$ and $a_r-a_l \geq 2^{N+1-(i-1)}.|\mathbf{s}|$}. Then $b_i=b_r-(a_r-a_i)$.  By induction hypothesis over $\play{i-1}{\astrategy_S,\hat\astrategy_D}{\aword,\aword'}$, since $a_l=\lef{a_r}$ and $a_r=\rig{a_l}$ (note that if $a_l=a_{-1}$ or $a_r=a_0$ a similar reasoning can be done),  we also have that  $b_r-b_l \geq  2^{N+1-(i-1)}.|\mathbf{s}|$ . Hence we have that $(b_i-b_l)\geq 2^{N+1-(i-1)}.|\mathbf{s}| - (b_r-b_i) \geq 2^{N+1-(i-1)}.|\mathbf{s}| -  2^{N+1-i}.|\mathbf{s}| $. From which we deduce $b_i-b_l\geq 2^{N+1-i}.|\mathbf{s}|$ This allows us to deduce that  $b_{-1} \leq b_l < b_i < b_r \leq b_0$ and $b_r-b_i=a_r-a_i$ and $b_i-b_l\geq 2^{N+1-i}$. We also directly have $b_l=\lef{b_i}$ and $b_r=\rig{b_i}$. Finally since by induction hypothesis we have $a_{r}-a_{-1}=b_{r}-b_{-1}$ or $a_{0}-a_{r}=b_{0}-b_{r}$, we deduce also that $a_{i}-a_{-1}=b_{i}-b_{-1}$ or $a_{0}-a_{i}=b_{0}-b_{i}$.
\item \textbf{Case $a_i-a_l = 2^{N+1-i}.|\mathbf{s}|$ and $a_r-a_i = 2^{N+1-i}.|\mathbf{s}|$}. Then $b_i=b_l+(a_i-a_l)$. Then we have $a_r-a_l= 2^{N+1-(i-1)}.|\mathbf{s}|$. By induction hypothesis over $\play{i-1}{\astrategy_S,\hat\astrategy_D}{\aword,\aword'}$, since $a_l=\lef{a_r}$ and $a_r=\rig{a_l}$ (note that if $a_l=a_{-1}$ or $a_r=a_0$ a similar reasoning can be done),  we also have that  $b_r-b_l \geq  2^{N+1-(i-1)}.|\mathbf{s}|$ and $|(a_r-a_l)-(b_r-b_l)| \leq |\mathbf{s}|$ [using $\aninv.4.a$]. From this we deduce that $b_r-b_l \geq a_r-a_l$ (otherwise we would have $b_r-b_l < 2^{N+1-(i-1)}.|\mathbf{s}|$, which allow us to deduce immediately that  $b_r-b_i \geq a_r-a_i$ and hence  $b_r-b_i \geq 2^{N+1-i}.|\mathbf{s}|$. Hence we also have  $b_{-1} \leq b_l < b_i < b_r \leq b_0$. We also directly have $b_l=\lef{b_i}$ and $b_r=\rig{b_i}$. Finally since by induction hypothesis we have $a_{l}-a_{-1}=b_{l}-b_{-1}$ or $a_{0}-a_{l}=b_{0}-b_{l}$, we deduce also that $a_{i}-a_{-1}=b_{i}-b_{-1}$ or $a_{0}-a_{i}=b_{0}-b_{i}$.
\item \textbf{Case $a_i-a_l = 2^{N+1-i}.|\mathbf{s}|$ and $a_r-a_i > 2^{N+1-i}.|\mathbf{s}|$}. Then $b_i=b_l+(a_i-a_l)$. Then we have $a_r-a_l \geq 2^{N+1-(i-1)}.|\mathbf{s}|$. By induction hypothesis over $\play{i-1}{\astrategy_S,\hat\astrategy_D}{\aword,\aword'}$, since $a_l=\lef{a_r}$ and $a_r=\rig{a_l}$ (note that if $a_l=a_{-1}$ or $a_r=a_0$ a similar reasoning can be done),  we also have that  $b_r-b_l \geq  2^{N+1-(i-1)}.|\mathbf{s}|$. This allow us to deduce immediately that  $b_r-b_i \geq 2^{N+1-i}.|\mathbf{s}|$. Hence we also have  $b_{-1} \leq b_l < b_i < b_r \leq b_0$. We also directly have $b_l=\lef{b_i}$ and $b_r=\rig{b_i}$. Finally since by induction hypothesis we have $a_{l}-a_{-1}=b_{l}-b_{-1}$ or $a_{0}-a_{l}=b_{0}-b_{l}$, we deduce also that $a_{i}-a_{-1}=b_{i}-b_{-1}$ or $a_{0}-a_{i}=b_{0}-b_{i}$.
\item \textbf{Case $a_i-a_l > 2^{N+1-i}.|\mathbf{s}|$ and $a_r-a_i = 2^{N+1-i}.|\mathbf{s}|$}. Then $b_i=b_r-(a_r-a_i)$. Then we have $a_r-a_l \geq 2^{N+1-(i-1)}.|\mathbf{s}|$. By induction hypothesis over $\play{i-1}{\astrategy_S,\hat\astrategy_D}{\aword,\aword'}$, since $a_l=\lef{a_r}$ and $a_r=\rig{a_l}$ (note that if $a_l=a_{-1}$ or $a_r=a_0$ a similar reasoning can be done),  we also have that  $b_r-b_l \geq  2^{N+1-(i-1)}.|\mathbf{s}|$. This allow us to deduce immediately that  $b_i-b_l \geq 2^{N+1-i}.|\mathbf{s}|$. Hence we also have  $b_{-1} \leq b_l < b_i < b_r \leq b_0$. We also directly have $b_l=\lef{b_i}$ and $b_r=\rig{b_i}$. Finally since by induction hypothesis we have $a_{l}-a_{-1}=b_{l}-b_{-1}$ or $a_{0}-a_{l}=b_{0}-b_{l}$, we deduce also that $a_{i}-a_{-1}=b_{i}-b_{-1}$ or $a_{0}-a_{i}=b_{0}-b_{i}$.
\item \textbf{Case $a_i-a_l > 2^{N+1-i}.|\mathbf{s}|$ and $a_r-a_i > 2^{N+1-i}.|\mathbf{s}|$ and $a_i-a_l <a_r-a_i$ }. Then $b_i=b_l+(a_i-a_l)$. Then we have $a_r-a_l \geq 2^{N+1-(i-1)}.|\mathbf{s}|$. By induction hypothesis over $\play{i-1}{\astrategy_S,\hat\astrategy_D}{\aword,\aword'}$, since $a_l=\lef{a_r}$ and $a_r=\rig{a_l}$ (note that if $a_l=a_{-1}$ or $a_r=a_0$ a similar reasoning can be done),  we also have that  $b_r-b_l \geq  2^{N+1-(i-1)}.|\mathbf{s}|$ . This allow us to deduce immediately that  $b_i-b_l \geq 2^{N+1-i}.|\mathbf{s}|$ $|(a_r-a_l)-(b_r-b_l)| \leq |\mathbf{s}|$ [using $\aninv.4.a$]. Consequently we deduce that $b_r-b_i \geq a_r-a_i-|\mathbf{s}| \geq 2^{N+1-i}.|\mathbf{s}|$. Hence we have  $b_{-1} \leq b_l < b_i < b_r \leq b_0$. We also directly have $b_l=\lef{b_i}$ and $b_r=\rig{b_i}$. Finally since by induction hypothesis we have $a_{l}-a_{-1}=b_{l}-b_{-1}$ or $a_{0}-a_{l}=b_{0}-b_{l}$, we deduce also that $a_{i}-a_{-1}=b_{i}-b_{-1}$ or $a_{0}-a_{i}=b_{0}-b_{i}$.
\item \textbf{Case $a_i-a_l > 2^{N+1-i}.|\mathbf{s}|$ and $a_r-a_i > 2^{N+1-i}.|\mathbf{s}|$ and $a_r-a_i <a_i-a_l$ }. Then $b_i=b_r-(a_r-a_i)$. Then we have $a_r-a_l \geq 2^{N+1-(i-1)}.|\mathbf{s}|$. By induction hypothesis over $\play{i-1}{\astrategy_S,\hat\astrategy_D}{\aword,\aword'}$, since $a_l=\lef{a_r}$ and $a_r=\rig{a_l}$ (note that if $a_l=a_{-1}$ or $a_r=a_0$ a similar reasoning can be done),  we also have that  $b_r-b_l \geq  2^{N+1-(i-1)}.|\mathbf{s}|$ . This allow us to deduce immediately that  $b_i-b_l \geq 2^{N+1-i}.|\mathbf{s}|$ $|(a_r-a_l)-(b_r-b_l)| \leq |\mathbf{s}|$ [using $\aninv.4.a$]. Consequently we deduce that $b_i-b_l \geq a_i-a_l-|\mathbf{s}| \geq 2^{N+1-i}.|\mathbf{s}|$. Hence we have  $b_{-1} \leq b_l < b_i < b_r \leq b_0$. We also directly have $b_l=\lef{b_i}$ and $b_r=\rig{b_i}$. Finally since by induction hypothesis we have $a_{r}-a_{-1}=b_{r}-b_{-1}$ or $a_{0}-a_{r}=b_{0}-b_{r}$, we deduce also that $a_{i}-a_{-1}=b_{i}-b_{-1}$ or $a_{0}-a_{i}=b_{0}-b_{i}$.
 \end{enumerate}
 Thanks to the previous case analysis, it is then easy to check that $\play{i}{\astrategy_S,\hat\astrategy_D}{\aword,\aword'}$ respects $\aninv$. The case where $\astrategy_S(\play{i-1}{\astrategy_S,\hat\astrategy_D}{\aword,\aword'})=\tuple{1,b_i}$ can be treated in an equivalence manner. \qed
%\begin{enumerate}
%\item \textbf{Case $a_r-a_i \leq 2^{N-i}.|\mathbf{s}|$ and $a_r-a_l > 2^{N-(i-1)}.|\mathbf{s}|$}\\
%We have $b_i=b_r-(a_r-a_i)$. By induction hypothesis since $a_{-1} \leq a_r \leq a_0$, we also have $b_{-1} \leq b_r \leq b_0$, and consequently $b_i < b_r \leq b_0$ (in fact $a_r-a_i >0$). Since $a_r-a_l \leq 2^{N-(i-1)}.|\mathbf{s}|$, then by induction hypothesis over $\play{i-1}{\astrategy_S,\hat\astrategy_D}{\aword,\aword'}$, since $a_l=\lef{a_r}$ and $a_r=\rig{a_l}$ (note that if $a_l=a_{-1}$ or $a_r=a_0$ a similar reasoning can be done),  we also have that  $b_r-b_l \leq 2^{N+1-(i-1)}.|\mathbf{s}|$ and $a_r-a_l=b_r-b_l$ [using $\aninv.4.b$ and $\aninv.4.c$], and since $a_r-a_i < a_r-a_l$ [by definition of $a_r$ and $a_l$] we deduce that $b_r-b_i < b_r - b_l$, consequently $b_{-1} \leq b_l < b_i$. Hence we have $b_{-1} \leq b_l < b_i < b_r \leq b_0$. This allows us to conclude also that $b_l=\lef{b_i}$ and $b_r=\rig{b_i}$. Note by the way that we have also in this case $b_r-b_i=a_r-a_i$ and $b_i-b_l=a_l-a_i$.
%%
%\item \textbf{Case $a_r-a_i \leq 2^{N-i}.|\mathbf{s}|$ and $a_r-a_l > 2^{N-(i-1)}.|\mathbf{s}|$}\\
%We have $b_i=b_r-(a_r-a_i)$. Note that in this case, we also have $a_i-a_l > 2^{N-i}.|\mathbf{s}|$. By induction hypothesis since $a_{-1} \leq a_r \leq a_0$, we also have $b_{-1} \leq b_r \leq b_0$, and consequently $b_i < b_r \leq b_0$ (in fact $a_r-a_i >0$). Since $a_r-a_l > 2^{N-(i-1)}.|\mathbf{s}|$, then by induction hypothesis over $\play{i-1}{\astrategy_S,\hat\astrategy_D}{\aword,\aword'}$, since $a_l=\lef{a_r}$ and $a_r=\rig{a_l}$ (note that if $a_l=a_{-1}$ or $a_r=a_0$ a similar reasoning can be done),  we also have that  $b_r-b_l > 2^{N-(i-1)}.|\mathbf{s}|$, hence since  $a_r-a_i \leq 2^{N-i}.|\mathbf{s}|$, we deduce that $b_i > b_l$ and $b_i-b_l > 2^{N-(i-1)}.|\mathbf{s}|$.  Hence we have $b_{-1} \leq b_l < b_i < b_r \leq b_0$. This allows us to conclude also that $b_l=\lef{b_i}$ and $b_r=\rig{b_i}$. Note by the way that we have also in this case $b_r-b_i=a_r-a_i$ and $b_i-b_l>2^{N-i}.|\mathbf{s}| $ and $a_l-a_i>2^{N-i}.|\mathbf{s}| $.
%%
%\item \textbf{Case $a_r-a_i  > 2^{N-i}.|\mathbf{s}|$ and $a_r-a_l \leq 2^{N-(i-1)}.|\mathbf{s}|$}\\
%We have $b_i=b_l+(a_i-a_l)$. By induction hypothesis since $a_{-1} \leq a_l \leq a_0$, we also have $b_{-1} \leq b_l \leq b_0$, and consequently $b_{-1} \leq b_l < b_i $ (in fact $a_i-a_l >0$). Since $a_r-a_l \leq 2^{N-(i-1)}.|\mathbf{s}|$, then by induction hypothesis over $\play{i-1}{\astrategy_S,\hat\astrategy_D}{\aword,\aword'}$, since $a_l=\lef{a_r}$ and $a_r=\rig{a_l}$ (note that if $a_l=a_{-1}$ or $a_r=a_0$ a similar reasoning can be done),  we also have that  $b_r-b_l \leq 2^{N-(i-1)}.|\mathbf{s}|$ and $a_r-a_l=b_r-b_l$ [using $\aninv.4.b$ and $\aninv.4.c$], and since $a_i-a_l < a_r-a_l$ [by definition of $a_r$ and $a_l$] we deduce that $b_i-b_l < b_r - b_l$, consequently  $b_i < b_r \leq b_0$. Hence we have $b_{-1} \leq b_l < b_i < b_r \leq b_0$. This allows us to conclude also that $b_l=\lef{b_i}$ and $b_r=\rig{b_i}$. Note by the way that we have also in this case $b_r-b_i=a_r-a_i$ and $b_i-b_l=a_l-a_i$.
%
%\item \textbf{Case $a_r-a_i  > 2^{N-i}.|\mathbf{s}|$ and $a_r-a_l > 2^{N-(i-1)}.|\mathbf{s}|$}\\
%We have $b_i=b_l+(a_i-a_l)$. By induction hypothesis since $a_{-1} \leq a_l \leq a_0$, we also have $b_{-1} \leq b_l \leq b_0$, and consequently $b_{-1} \leq b_l < b_i $ (in fact $a_i-a_l >0$). Furthermore, by induction hypothesis over $\play{i-1}{\astrategy_S,\hat\astrategy_D}{\aword,\aword'}$ since $a_l=\lef{a_r}$ and $a_r=\rig{a_l}$ (note that if $a_l=a_{-1}$ or $a_r=a_0$ a similar reasoning can be done),  we also have that  $b_r-b_l > 2^{N-(i-1)}.|\mathbf{s}|$. Furthermore always by induction hypothesis,using $\aninv.4.a$, we have that $|(a_l-a_r) -(b_l-b_r)| \leq |s|$.
%
%
% and  Note that in this case, we also have $a_i-a_l > 2^{N-i}.|\mathbf{s}|$. By induction hypothesis since $a_{-1} \leq a_r \leq a_0$, we also have $b_{-1} \leq b_r \leq b_0$, and consequently $b_i < b_r \leq b_0$ (in fact $a_r-a_i >0$). Since $a_r-a_l > 2^{N-(i-1)}.|\mathbf{s}|$, then by induction hypothesis over $\play{i-1}{\astrategy_S,\hat\astrategy_D}{\aword,\aword'}$, since $a_l=\lef{a_r}$ and $a_r=\rig{a_l}$ (note that if $a_l=a_{-1}$ or $a_r=a_0$ a similar reasoning can be done),  we also have that  $b_r-b_l > 2^{N-(i-1)}.|\mathbf{s}|$, hence since  $a_r-a_i \leq 2^{N-i}.|\mathbf{s}|$, we deduce that $b_i > b_l$ and $b_i-b_l > 2^{N-(i-1)}.|\mathbf{s}|$.  Hence we have $b_{-1} \leq b_l < b_i < b_r \leq b_0$. This allows us to conclude also that $b_l=\lef{b_i}$ and $b_r=\rig{b_i}$. Note by the way that we have also in this case $b_r-b_i=a_r-a_i$ and $b_i-b_l>2^{N-i}.|\mathbf{s}| $ and $a_l-a_i>2^{N-i}.|\mathbf{s}| $.
%
%
%
%\end{enumerate}


%By induction hypothesis, we now that for all $j \in \interval{1}{i-1}$, the point $1$, $2$ and $4$ of $\aninv$ are satisfied, it is hence enough to verify that they are satisfy for the position chosen at the $i$-th round. If $a_i \leq a_{-1}$, then we have  $a_i=b_i$ and also $b_i \leq b_{-1}$.  If $a_0 \leq a_{i}$, then $b_i=a_i+|\mathbf{s}|$ and since $b_0=a_0+|\mathbf{s}|$, we deduce that $b_0 \leq b_i$ and $a_i-a_0=b_i-b_0$. 
%
%Finally we consider the case $a_{-1} < a_i < a_0$ with $a_l=\lef{a_i}$ and $a_r=\rig{a_i}$.  First if $a_r-a_i \leq 2^{N-i}.|\mathbf{s}|$, we have $b_i=b_r-(a_r-a_i)$. First let us prove that $b_{-1} < b_i < b_0$. By induction hypothesis since $a_{-1} \leq a_r \leq a_0$, we also have $b_{-1} \leq b_r \leq b_0$, and consequently $b_i <b_0$ (in fact $a_r-a_i >0$). Now we have two cases, if $a_r-a_l \leq 2^{N-(i-1)}$, then by induction hypothesis since in $\play{i-1}{\astrategy_S,\hat\astrategy_D}{\aword,\aword'}$, $a_l=\lef{a_r}$ and $a_r=\rig{a_l}$ (note that if $a_l=a_{-1}$ or $a_r=a_0$ a similar reasoning can be done),  we also have that  $b_r-b_l \leq 2^{N-(i-1)}$ and $a_r-a_l=b_r-b_l$ (by using $\aninv.4.b$ and $\aninv.4.c$), and since $a_r-a_i < a_r-a_l$ (by definition of $a_r$ and $a_l$ we deduce that $b_r-b_i < b_r - b_l$, consequently $b_i > b_l \geq b_0$. Note by the way that we have also in this case $b_r-b_i=a_r-a_i$ and $b_i-b_l=a_l-a_i$ 
%%We now assume that  Without loss of generality, we can assume that the Spoiler plays on the word
%%$\astruct$. The other case follows similar arguments.
%%
%%\textbf{Base case:} During the first move, assume the Spoiler chooses $a_1$. If $a_1\leq a_{-1}$ or $a_1> a_0$, then we can always choose the same
%%positions in the words $\aword_1$ and $\aword_2$ in $\aword'$ according to $\astrategy_{D}$. This satisfies Conditions 1 to 3 of $\aninv(Pl_1)$ in this
%%case. If $a_1$ is in the iterations of $\mathbf{s}$, then the Duplicator can select $b_1$ such that $a_{0}-a_{1}=b_0-b_{1}$ if $a_{0}-a_{1}\leq
%%2^{N-1}|\mathbf{s}|$ and $a_1-a_{-1}=b_1-b_{-1}$ otherwise, which is according to $\astrategy_{D}$. Since, $a_{-1},b_{-1},a_{0}$ and $b_{0}$ points to
%%the start and end of the iterations of the repetition of $\mathbf{s}$, $a_1$ and $b_1$ point to the same position of the word $\mathbf{s}$. Thus, the
%%Conditions 1,3 and 4 of $\aninv(Pl_1)$ holds. Hence, in both cases, $\aninv(Pl_1)$ holds.
%%
%\textbf{Induction Step:} Assume at round $i$, we have $a_1,\ldots,a_{i-1}$ and $b_1,\ldots,b_{i-1}$ and $\aninv(Pl_{i-1})$ holds. Now the Spoiler selects
%$a_i\in\astruct$. The Duplicator selects $b_i\in\bstruct$ according to $\astrategy_{D}$. We will show that $\aninv(Pl_i)$ holds.
%
%If $a_i<a_{-1}$ or $a_i>a_{0}$, then by $\astrategy_{D}$, $b_i$ points to the same position as $a_i$ in the words $\aword_1$ or $\aword_2$
%respectively. Thus, the Condition 1 and 2 of $\aninv(Pl_i)$ is satisfied. Also, from $\aninv(Pl_{i-1})$ and the choice of $b_i$ it is easy to see that
%Condition 3 of $\aninv(Pl_i)$ is also satisfied. We will now consider the case where $a_{-1}\leq a_i\leq a_0$. Note that as previous we consider
%$a_{-1}\leq a_{\alpha},a_{\beta}\leq a_{0}$ as the nearest neighbours of $a_i$ with the properties that $a_{\alpha}\leq a_i\leq a_{\beta}$ and hence there does not exists
%$\gamma\in[-1,i]$ such that $a_{\alpha}< a_{\gamma}< a_i$ or $a_i< a_{\gamma} < a_{\beta}$. We will deal with three different cases seperately,
%\begin{itemize}
%  \item One of either $|a_{i}-a_{\alpha}|\leq 2^{N-i}.|\mathbf{s}|$ or $|a_{\beta}-a_{i}|\leq 2^{N-i}.|\mathbf{s}|$ is true. Without loss of
%    generality, let us assume that $|a_{i}-a_{\alpha}|\leq 2^{N-i}.|\mathbf{s}|$, the other case follows similarly. By $\astrategy_{D}$, we have
%    $a_{i}-a_{\alpha}=b_{i}-b_{\alpha}$. By Condition 4(a) of $\aninv(Pl_{i-1})$, we know that either $a_{\alpha}-a_{-1}=b_{\alpha}-b_{-1}$ or
%    $a_{0}-a_{\alpha}=b_{0}-b_{\alpha}$ and thus respectively, either $a_{i}-a_{-1}=b_{i}-b_{-1}$ or $a_{0}-a_{i}=b_{0}-b_{i}$. This also
%    implies that $a_{i}$ and $b_{i}$ points to the same position in the word $\mathbf{s}$. Hence, we can easily
%    verify that Conditions 1, 3, 4(a), 4(b) and 4(c) of $\aninv(Pl_i)$ are satisfied.
%  \item Both $|a_{i}-a_{\alpha}|\leq 2^{N-i}.|\mathbf{s}|$ and $|a_{\beta}-a_{i}|\leq 2^{N-i}.|\mathbf{s}|$ are true, in that case,
%    $a_{\beta}-a_{\alpha}\leq 2^{N-(i-1)}.|\mathbf{s}|$. According to $\aninv(Pl_{i-1})$, $a_{\beta}-a_{\alpha}=b_{\beta}-b_{\alpha}$ and hence for
%    any $j\in\{-1,0\}$, $a_{j}-a_{\alpha}=b_{j}-b_{\alpha}$ iff $a_{j}-a_{\beta}=b_{j}-b_{\beta}$. According to $\astrategy_{D}$, if we select $b_i$
%    such that $a_{i}-a_{\alpha}=b_{i}-b_{\alpha}$, we have that $a_{\beta}-a_{i}=b_{\beta}-b_{i}$ and vice versa. Also, as previous, $a_{i}$ and
%    $b_{i}$ points to the same position in the word $\mathbf{s}$. Again, Conditions 1,3,4(a) and 4(b) of $\aninv(Pl_i)$ are satisfied.
%  \item Both $|a_{i}-a_{\alpha}|>2^{N-i}.|\mathbf{s}|$ and $|a_{\beta}-a_{i}|> 2^{N-i}.|\mathbf{s}|$ are true. In this case according to
%    $\astrategy_{D}$, we have $b_i-b_{\alpha}=a_{i}-a_{\alpha}$. Also, note that the choice of $\alpha,\beta$ guarantees that
%    $a_{\beta}-a_{\alpha}>2^{N-(i-1)}.|\mathbf{s}|$. By $\aninv(Pl_{i-1})$, we have that either $a_{\alpha}-a_{-1}=b_{\alpha}-b_{-1}$ or
%    $a_{\alpha}-a_{0}=b_{\alpha}-b_{0}$ and hence $a_{i}-a_{-1}=b_{i}-b_{-1}$ or $a_{0}-a_{i}=b_{0}-b_{i}$ respectively. Again, Conditions 1, 3, 4(a)
%    and 4(c) of $\aninv(Pl_i)$ are satisfied.
%\end{itemize}
%%\textbf{Last Step:}Conside round $n$, we have $a_1,\ldots,a_{n}$ and $b_1,\ldots,b_{n-1}$ and $\aninv(n-1)$ holds. The Duplicator selects
%%$b_n\in\bstruct$ according to $\astrategy_{D}$. We will show that $\aninv(n)$ holds. As before, if $a_n<a_{-1}$ or $a_n>a_0$, then we can see that the
%%conditions of $\aninv(n)$ are satisfied. Also, from the proof of induction it is easy to see that $\aninv(n)$ holds when at least one of
%%$|a_{i}-a_{\alpha}|\leq 2^0.|\mathbf{s}|$ and $|a_{\beta}-a_{i}|\leq 2^{0}.|\mathbf{s}|$ are true. The interesting case is when both
%%$|a_{i}-a_{\alpha}|> 2^{0}.|\mathbf{s}|$ and $|a_{\beta}-a_{i}|> 2^0.|\mathbf{s}|$ are true. In this case, note that both $|a_{i}-a_{\alpha}|$ and
%%$|a_{\beta}-a_{i}|$ are at least $2.|\mathbf{s}|$.
%\qed
\end{proof}
%
Using Lemma \ref{lem-inv} and \ref{lem-strat-win}, we deduce that Duplicator has a winning strategy against any strategy of the Spoiler in $EF_N(\astruct,\bstruct)$, so by Theorem \ref{theorem:EF}, we can conclude the main theorem of this subsection.
\begin{theorem}[Stuttering Theorem]
\label{theorem:stuttering}
Let $\aword = \aword_1 \mathbf{s}^M \aword_2, \aword'= \aword_1 \mathbf{s}^{M+1} \aword_2 \in (\Sigma)^{\omega}$  such that $N \geq 2$, $M> 2^{N+1}$ and $\mathbf{s}$ is a non-empty finite word. Then $\astruct\equivrel{N}\bstruct$.
\end{theorem}

% Arn 111212
%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%\vspace{5em}
%
%Here, we state the stuttering theorem for $FO_{\varprop}$ formulas. The stuttering theorem allows us to bound the repetition of any subword in the
%model to a number which is exponential in the size of the formula. This, helps us to characterize the complexity of the model checking problem by allowing us
%to check runs where the loops are taken a bounded number of times and thus in effect allowing us to a non-deterministic guess on the number of
%iteration. We will now use EF games to prove a stuttering theorem equivalent for FO.
%
%\begin{theorem}[Stuttering Theorem]
%\label{theorem:stuttering}
%Let $\aword = \aword_1 \mathbf{s}^M \aword_2, \aword'= \aword_1 \mathbf{s}^{M+1} \aword_2 \in (\Sigma)^{\omega}$ and $\astruct$ and $\bstruct$ be the
%models, such that $N \geq 2$, $M> 2^N$. Then, we have that $\astruct\equivrel{N}\bstruct$.
%%for every $FO$ sentence $\aformula$ with $\qheight{\aformula} \leq N$, we have $\astruct \models \aformula$ iff $\bstruct \models \aformula$. 
%\end{theorem}
%We will actually show that the Duplicator always has a winning strategy in $EF_{N}(\astruct,\bstruct)$. Using Theorem~\ref{theorem:EF}, this will in
%turn imply that, for every $FO_{\varprop}$ formula $\aformula$ with $\qheight{\aformula} \leq N$, we have $\astruct \models \aformula$ iff $\bstruct
%\models \aformula$. In the sequel, we will provide a winning strategy $\astrategy_{D}$ for Duplicator in $EF_n(\aword,\aword')$ with $\aword =
%\aword_1 \mathbf{s}^M \aword_2, \aword'= \aword_1 \mathbf{s}^{M+1} \aword_2$, where $M> 2^{N}$ for any strategy of Spoiler. Then we will show that the
%strategy ensures that we have a partial isomorphism after $N$-rounds and hence is a winning strategy for Duplicator. The strategy for Duplicator says
%to choose a point, such that if two points in a word are sufficiently close to each other (upto a distance of $2^{\qheight{\aformula}}$) then the
%corresponding points in the other word are at the same distance and if they are far from each other, then we don't care about the distance between the
%point except that they are at a distance, more than $2^{\qheight{\aformula}}$. First, we will define some invariants that would be maintained by the
%Duplicator while playing the game. For technical convinience of describing the invariant and strategy, let us fix $a_{-1}=b_{-1}=|\aword_1|$,
%$a_{0}=|\aword_1\mathbf{s}^{M}|$ and $b_{0}=|\aword_1\mathbf{s}^{M+1}|$. Note that these are the positions where the repetition of $\mathbf{s}$ starts
%and ends in each word. These positions are also used in the strategy as other positions. Hence, designating them as another indexed position in each
%word allows us to deal with only the indexed positions in the words. Given a play $Pl_i$, for some element $a_j, j\in[1,i]$, we can define
%\defstyle{two nearest neighbours} of $a_j$ as $a_k\leq a_j\leq a_l$ with $k,l\in[-1,i]$ such that there is no $m\in[-1,i]$ for which $a_k<a_m<a_j$ or
%$a_j<a_m<a_l$ holds.For $i\in[1,N]$, let $\aninv(Pl_i)$ be the invariant at round $i$ is defined over the play
%$Pl_{i}(\astrategy_{S},\astrategy_{D},\astruct,\bstruct)$, by the conjunction of the following conditions:
%%Consider the following invariants at round $i$, of the game. The invariant $\aninv(i)$ consists of the following
%%conditions for all $\alpha\in[1,i]$,
%\begin{enumerate}
%  \item For all $j\in[-1,i]$, $c\in \varprop$, $c\in\aword(a_{j})$ iff $c\in \aword'(b_{j})$.
%  \item For all $j\in[1,i]$, $a_{j}=b_{j}$ iff $a_{j}<a_{-1}$ and $|a_{j}-a_0|=|b_{j}-b_0|$ iff $a_j>a_0$.
%  \item For all $j,k\in[-1,i]$, $a_{j}<a_{k}$ iff $b_{j}<b_{k}$.
%  \item For all $k\in[-1,i]$, such that $a_{-1}\leq a_k\leq a_{0}$, we have that for $\alpha,\beta\in[-1,i]$ with $a_{\alpha}\leq a_k\leq a_{\beta}$
%    the nearest neighbour of $a_k$,
%    \begin{enumerate}
%      \item Either $a_{k}-a_{-1}=b_{k}-b_{-1}$ or $a_{0}-a_{k}=b_{0}-b_{k}$.
%      \item For any $j\in\{\alpha,\beta\}$, $a_{j}-a_{k} = b_{j}-b_{k}$ iff $|a_{j}-a_{k}|\leq 2^{N-i}.|\mathbf{s}|$ or $|b_{j}-b_{k}|\leq
%        2^{N-i}.|\mathbf{s}|$.
%      \item $|a_k-a_{\alpha}|=|b_k-b_{\alpha}|$ iff $a_{\beta}-a_{k}> 2^{N-i}.|\mathbf{s}|$ and $a_{k}-a_{\alpha}> 2^{N-i}.|\mathbf{s}|$ or $b_{\beta}-b_{k}>
%        2^{N-i}.|\mathbf{s}|$ and $b_{k}-b_{\alpha}> 2^{N-i}.|\mathbf{s}|$.
%    \end{enumerate}
%%  \item For all $\alpha,\beta\in[1,i]$ $a_{\alpha}-a_{\beta}=b_{\alpha}-b_{\beta}$, whenever $a_{\alpha}-a_{\beta}\leq 2^{N-i}.|\mathbf{s}|$ or $b_{\alpha}-b_{\beta}\leq 2^{N-i}.|\mathbf{s}|$
%%  \item For all $\alpha\in[1,i]$ $a_{\alpha}-|\aword_1|=b_{\alpha}-|\aword_1|$ whenever
%%    $a_{\alpha}-|\aword_1|\leq 2^{N-i}.|\mathbf{s}|$ or $b_{\alpha}-|\aword_1|\leq 2^{N-i}.|\mathbf{s}|$.
%%  \item For all $\alpha\in[1,i]$ $|\aword_1\mathbf{s}^{M}|-a_{\alpha}=|\aword_1\mathbf{s}^{M+1}|-b_{\alpha}$ whenever
%%    $|\aword_1\mathbf{s}^{M}|-a_{\alpha}\leq 2^{N-i}.|\mathbf{s}|$ or $|\aword_1\mathbf{s}^{M+1}|-b_{\alpha}\leq 2^{N-i}.|\mathbf{s}|$.
%\end{enumerate}
%
%Let the strategy of the Duplicator be $\astrategy_{D}$. $\astrategy_{D}$ is defined for each round $i$ as following. 
%
%Without loss of generality, we assume the Spoiler plays in $\astruct$ and chooses $a_i$.% Let $\vect{a}=(a_1,a_2,\ldots,a_{i})$ and $\vect{b}=(b_1,b_2,\ldots,b_{i-1})$. 
%If the Spoiler chooses $a_i$ in $\astruct$ such that $a_{\alpha}\leq a_i\leq a_{\beta}$ where
%$\alpha,\beta\in[1,i-1]$ are the nearest neighbour of $a_i$ (in case of absence of any of $a_{\alpha}$ or $a_{\beta}$, we set $a_{\alpha}=a_i$ or
%$a_{\beta}=a_i$ respectively), then Duplicator chooses $b_i$ in $\bstruct$ where
%$b_i=\astrategy_{D}(\tuple{(p_1,a_1,b_1),(p_2,a_2,b_2),\ldots,(p_{i-1},a_{i-1},b_{i-1})},(0,a_i))$. The position $b_i$ is chosen by the strategy iff
%the following conditions hold:
%\begin{itemize}
%  \item $b_{\alpha}\leq b_i\leq b_{\beta}$(Respect order of the values)
%  \item If $a_i\leq a_{-1}$, then $b_i=a_i$.
%  \item If $a_i> a_{0}$, then $b_i=a_i+|\mathbf{s}|$. (same positions in word $\aword_2$)
%  \item If $a_i=a_{\alpha}$ for $\alpha\in[1,i-1]$ then $b_i=b_{\alpha}$.
%  \item If $a_i> |\aword_1|$ and $a_i\leq|\aword_1\mathbf{s}^{M}|$, then
%    \begin{itemize}
%%      \item $b_i> |\aword_1|$ and $b_i\leq|\aword_1\mathbf{s}^{M+1}|$. (within the interations of $\mathbf{s}$)
%%      \item $(a_i-|\aword_1|) mod |\mathbf{s}| = (b_i-|\aword_1|) mod |\mathbf{s}|$. (same position in the word $\mathbf{s}$)
%%      \item $b_{\alpha}\leq b_i\leq b_{\beta}$. (Respect order of the values)
%      \item For $j\in \{\alpha,\beta\}$, if $|a_i - a_{j}|\leq 2^{N-i}.|\mathbf{s}|$ then $a_i - a_{j}=b_i - b_{j}$.
%%      \item If $a_{\beta}-a_{i}\leq 2^{N-i}.|\mathbf{s}|$ then $a_{\beta} - a_i=b_{\beta}-b_i$.
%      \item If $a_{\alpha} - a_{i}> 2^{N-i}.|\mathbf{s}|$ and $a_i - a_{\beta}> 2^{N-i}.|\mathbf{s}|$ then $b_i - b_{\alpha}=a_i-a_{\alpha}$.
%%      \item If $a_{\beta}-a_{i}> 2^{N-i}.|\mathbf{s}|$ then $b_{\beta}-b_i>2^{N-i}.|\mathbf{s}|$.
%%      \item If $a_i - |\aword_1|\leq 2^{N-i}.|\mathbf{s}|$ then $a_i - |\aword_1|=b_i - |\aword_1|$.
%%      \item If $|\aword_1\mathbf{s}^{M}|-a_{i}\leq 2^{N-i}.|\mathbf{s}|$ then $|\aword_1\mathbf{s}^{M}| - a_i=|\aword_1\mathbf{s}^{M+1}|-b_i$.      
%%      \item If $a_i - |\aword_1|> 2^{N-i}.|\mathbf{s}|$ then $b_i - |\aword_1|>2^{N-i}.|\mathbf{s}|$.
%%      \item If $|\aword_1\mathbf{s}^{M}|-a_{i}> 2^{N-i}.|\mathbf{s}|$ then $|\aword_1\mathbf{s}^{M+1}|-b_i>2^{N-i}.|\mathbf{s}|$.      
%    \end{itemize}
%\end{itemize}
%For the case where the Spoiler chooses $b_i$ in $\bstruct$, the move of Duplicator is defined similarly on $\astruct$.  The first condition 
%says that the order among the positions in both the words should be same. The second and third condition state that for
%positions outside the iterations of $\mathbf{s}$, we keep the positions in both the words same. The fourth condition states that for positions in the
%iterations of $\mathbf{s}$, the distance between them is same if it is less than $\powerset{\qheight{\aformula}}$, otherwise it could be anything more
%than $\powerset{\qheight{\aformula}}$. %Note that $\astrategy$ returns a set of positions and hence there could be more than one choice for Duplicator's next move. 
%\begin{lemma}
%For any game where Duplicator follows the strategy $\astrategy_{D}$, at any round $i$, $\aninv(Pl_i)$ holds.
%\end{lemma}
%\begin{proof}
%The proof proceeds by induction on the number of rounds in the game. Without loss of generality, we can assume that the Spoiler plays on the word
%$\astruct$. The other case follows similar arguments.
%
%\textbf{Base case:} During the first move, assume the Spoiler chooses $a_1$. If $a_1\leq a_{-1}$ or $a_1> a_0$, then we can always choose the same
%positions in the words $\aword_1$ and $\aword_2$ in $\aword'$ according to $\astrategy_{D}$. This satisfies Conditions 1 to 3 of $\aninv(Pl_1)$ in this
%case. If $a_1$ is in the iterations of $\mathbf{s}$, then the Duplicator can select $b_1$ such that $a_{0}-a_{1}=b_0-b_{1}$ if $a_{0}-a_{1}\leq
%2^{N-1}|\mathbf{s}|$ and $a_1-a_{-1}=b_1-b_{-1}$ otherwise, which is according to $\astrategy_{D}$. Since, $a_{-1},b_{-1},a_{0}$ and $b_{0}$ points to
%the start and end of the iterations of the repetition of $\mathbf{s}$, $a_1$ and $b_1$ point to the same position of the word $\mathbf{s}$. Thus, the
%Conditions 1,3 and 4 of $\aninv(Pl_1)$ holds. Hence, in both cases, $\aninv(Pl_1)$ holds.
%
%\textbf{Induction Step:} Assume at round $i$, we have $a_1,\ldots,a_{i-1}$ and $b_1,\ldots,b_{i-1}$ and $\aninv(Pl_{i-1})$ holds. Now the Spoiler selects
%$a_i\in\astruct$. The Duplicator selects $b_i\in\bstruct$ according to $\astrategy_{D}$. We will show that $\aninv(Pl_i)$ holds.
%
%If $a_i<a_{-1}$ or $a_i>a_{0}$, then by $\astrategy_{D}$, $b_i$ points to the same position as $a_i$ in the words $\aword_1$ or $\aword_2$
%respectively. Thus, the Condition 1 and 2 of $\aninv(Pl_i)$ is satisfied. Also, from $\aninv(Pl_{i-1})$ and the choice of $b_i$ it is easy to see that
%Condition 3 of $\aninv(Pl_i)$ is also satisfied. We will now consider the case where $a_{-1}\leq a_i\leq a_0$. Note that as previous we consider
%$a_{-1}\leq a_{\alpha},a_{\beta}\leq a_{0}$ as the nearest neighbours of $a_i$ with the properties that $a_{\alpha}\leq a_i\leq a_{\beta}$ and hence there does not exists
%$\gamma\in[-1,i]$ such that $a_{\alpha}< a_{\gamma}< a_i$ or $a_i< a_{\gamma} < a_{\beta}$. We will deal with three different cases seperately,
%\begin{itemize}
%  \item One of either $|a_{i}-a_{\alpha}|\leq 2^{N-i}.|\mathbf{s}|$ or $|a_{\beta}-a_{i}|\leq 2^{N-i}.|\mathbf{s}|$ is true. Without loss of
%    generality, let us assume that $|a_{i}-a_{\alpha}|\leq 2^{N-i}.|\mathbf{s}|$, the other case follows similarly. By $\astrategy_{D}$, we have
%    $a_{i}-a_{\alpha}=b_{i}-b_{\alpha}$. By Condition 4(a) of $\aninv(Pl_{i-1})$, we know that either $a_{\alpha}-a_{-1}=b_{\alpha}-b_{-1}$ or
%    $a_{0}-a_{\alpha}=b_{0}-b_{\alpha}$ and thus respectively, either $a_{i}-a_{-1}=b_{i}-b_{-1}$ or $a_{0}-a_{i}=b_{0}-b_{i}$. This also
%    implies that $a_{i}$ and $b_{i}$ points to the same position in the word $\mathbf{s}$. Hence, we can easily
%    verify that Conditions 1, 3, 4(a), 4(b) and 4(c) of $\aninv(Pl_i)$ are satisfied.
%  \item Both $|a_{i}-a_{\alpha}|\leq 2^{N-i}.|\mathbf{s}|$ and $|a_{\beta}-a_{i}|\leq 2^{N-i}.|\mathbf{s}|$ are true, in that case,
%    $a_{\beta}-a_{\alpha}\leq 2^{N-(i-1)}.|\mathbf{s}|$. According to $\aninv(Pl_{i-1})$, $a_{\beta}-a_{\alpha}=b_{\beta}-b_{\alpha}$ and hence for
%    any $j\in\{-1,0\}$, $a_{j}-a_{\alpha}=b_{j}-b_{\alpha}$ iff $a_{j}-a_{\beta}=b_{j}-b_{\beta}$. According to $\astrategy_{D}$, if we select $b_i$
%    such that $a_{i}-a_{\alpha}=b_{i}-b_{\alpha}$, we have that $a_{\beta}-a_{i}=b_{\beta}-b_{i}$ and vice versa. Also, as previous, $a_{i}$ and
%    $b_{i}$ points to the same position in the word $\mathbf{s}$. Again, Conditions 1,3,4(a) and 4(b) of $\aninv(Pl_i)$ are satisfied.
%  \item Both $|a_{i}-a_{\alpha}|>2^{N-i}.|\mathbf{s}|$ and $|a_{\beta}-a_{i}|> 2^{N-i}.|\mathbf{s}|$ are true. In this case according to
%    $\astrategy_{D}$, we have $b_i-b_{\alpha}=a_{i}-a_{\alpha}$. Also, note that the choice of $\alpha,\beta$ guarantees that
%    $a_{\beta}-a_{\alpha}>2^{N-(i-1)}.|\mathbf{s}|$. By $\aninv(Pl_{i-1})$, we have that either $a_{\alpha}-a_{-1}=b_{\alpha}-b_{-1}$ or
%    $a_{\alpha}-a_{0}=b_{\alpha}-b_{0}$ and hence $a_{i}-a_{-1}=b_{i}-b_{-1}$ or $a_{0}-a_{i}=b_{0}-b_{i}$ respectively. Again, Conditions 1, 3, 4(a)
%    and 4(c) of $\aninv(Pl_i)$ are satisfied.
%\end{itemize}
%%\textbf{Last Step:}Conside round $n$, we have $a_1,\ldots,a_{n}$ and $b_1,\ldots,b_{n-1}$ and $\aninv(n-1)$ holds. The Duplicator selects
%%$b_n\in\bstruct$ according to $\astrategy_{D}$. We will show that $\aninv(n)$ holds. As before, if $a_n<a_{-1}$ or $a_n>a_0$, then we can see that the
%%conditions of $\aninv(n)$ are satisfied. Also, from the proof of induction it is easy to see that $\aninv(n)$ holds when at least one of
%%$|a_{i}-a_{\alpha}|\leq 2^0.|\mathbf{s}|$ and $|a_{\beta}-a_{i}|\leq 2^{0}.|\mathbf{s}|$ are true. The interesting case is when both
%%$|a_{i}-a_{\alpha}|> 2^{0}.|\mathbf{s}|$ and $|a_{\beta}-a_{i}|> 2^0.|\mathbf{s}|$ are true. In this case, note that both $|a_{i}-a_{\alpha}|$ and
%%$|a_{\beta}-a_{i}|$ are at least $2.|\mathbf{s}|$.
%\qed
%\end{proof}
%
%We have proved that, there exists a strategy $\astrategy_{D}$, for the Duplicator in the game $EF_{N}(\astruct,\bstruct)$, such that for every
%strategy $\astrategy_{S}$ of the Spoiler, $\aninv(Pl_i)$ is maintained at every round $i\in[1,N]$. We will now show that $\aninv(Pl_N)$ actually implies
%there exists a partial isomorphism $h:\vect{a}\rightarrow\vect{b}$ where $\vect{a}=(a_1,\ldots,a_N)$ and $\vect{b}=(b_1,\ldots,b_N)$. This will prove
%that the strategy $\astrategy_{D}$, is in fact a winning strategy for the Duplicator as for every game $EF_{N}(\astruct,\bstruct)$, it has a partial
%isomorphism.
%
%\begin{lemma}
%For a fixed game $EF_{N}(\astruct,\bstruct)=(p_1,a_1,b_1)(p_2,a_2,b_2)\cdots(p_n,a_n,b_N)$ where the Duplicator plays according to $\astrategy_{D}$,
%let $\vect{a}=(a_1,a_2,\ldots,a_N)$ and $\vect{b}=(b_1,b_2,\ldots,b_N)$. If $\aninv(Pl_N)$ is satisfied at the end of $N$ round game, then there exists a
%partial isomorphism $h:\vect{a}\rightarrow\vect{b}$.
%\end{lemma}
%\begin{proof}
%First notice that for all $i\in[-1,N]$, if either $a_{0}\leq a_i$ or $a_{-1}\leq a_i$, then for all $j\in[-1,N]$, all the conditions of partial
%isomorphism are satisfied, as the $a_i$ and $b_i$ points to the same position in the words $\aword_1$ or $\aword_2$. For the case when $a_{-1}\leq
%a_{i},a_{j}\leq a_0$, note that by $\aninv(Pl_N)$, we have that, if $|a_{i}-a_{j}|\leq 2^0.\mathbf{s}$ then $|a_{i}-a_{j}|=|b_{i}-b_{j}|$. We will consider each of
%the requirements of the partial isomorphism.
%\begin{itemize}
%  \item if $a_i=a_j$ then $|a_i-a_j|=0\leq 2^0\mathbf{s}$ and so, $b_i=b_j$.
%  \item if $a_i+1=a_j$ then $|a_i-a_j|=1\leq 2^0\mathbf{s}$ and so, $b_i+1=b_j$.
%  \item By Condition 3 of $\aninv(Pl_N)$, we have that $a_i<a_j$ iff $b_i<b_j$.
%  \item By Condition 1 of $\aninv(Pl_N)$, we have that for all $c\in \varprop$, $c\in\aword(a_{i})$ iff $c\in \aword'(b_{i})$
%\end{itemize}
%Thus, there exists a partial isomorphism $h:\vect{a}\rightarrow\vect{b}$.
%\end{proof}
%
%Thus, we have the bound that in a model of a formula $\aformula$, a word $u$ can be repeated at most $2^{\qheight{\aformula}}+1$ times. If it is repeated more than that,
%we can truncate safely the number of repeatition to $2^{\qheight{\aformula}}+1$ without changing the satisfaction of $\aformula$ on the model.
%
%%If we consider infinite runs $\arun$ in path schemas in flat Kripke structures as models of FO formulae, then the above results as corollary gives us
%%that,
%%\begin{corollary}
%%\label{cor:runFO}
%%Given a path schema $\aschema=\aseg_1\aloop_1^{+}\aseg_2\aloop_2^{+}\cdots\aseg_k^{+}\aloop_k^{+}$ and a $FO[\emptyset]$ sentence $\aformula$, if there exists a
%%run $\arun'\models\aformula$, then there also exists a run $\arun$, where for all $i\in[1,k]$ the loop $\aloop_i$ is taken at most
%%$2^{\qheight{\aformula}}$ times such that $\arun\models\aformula$.
%%\end{corollary}


==> subsection-upks.tex <==
\subsection{Model Checking Ultimately Periodic Kripke Structure}

An ultimately periodic Kripke structure (UPKS) is a structurally restricted Kripke structure having the special form of a path followed by a
cycle. Let us assume that the nodes are labelled with the alphabets from $\aalphabet$. For such a system $\asys$ we denote by
$\alang(\asys)=\{\alabelling(\arun)|\arun\mbox{ is a run in }\asys\}\subseteq\aalphabet^{\omega}$, the set of infinite words formed using the labels of each
position of the runs. Thus, for deciding an instance of the model checking problem MC($\mathcal{L}$,$UPKS$) for any specification $\aspecification$ in
$\mathcal{L}$, an $UPKS$ denoted as $\asys=\tuple{\states_1,\edges_1,\alabelling}$, it amounts to finding out whether
$\alang(\aspecification)\cap\alang(\asys)=\emptyset$ or not.  We will first deal with the problem MC(ABA,$UPKS$). Given an ABA
$\fsa=\tuple{\states,\aalphabet,\edges,\astate_i,F}$ and $\asys=\tuple{\states_1,\edges_1,\alabelling}$, we will check for non-emptiness of the
alternating \buchi~automaton $\fsa'=\tuple{\states\times\{1,2,\ldots m\},\{\aletter\},\edges',\tuple{\astate_i,1},F'}$, where $m=card(\states_1)$,
$F'=\{\tuple{\astate_f,j}|\astate_f\in F,j\in[1,m]\}$ and the transition relation is defined as
$\edges'=\{\tuple{\tuple{\astate_1,j},p,\mathtt{B}[\astate\rightarrow\tuple{\astate,j+1}]}|\tuple{\astate_1,p,\mathtt{B}(\states)}\in\edges,
p=\alabelling(\astate_j)\}$. Intuitively, we compute a product of the UPKS and ABA to obtain $\fsa'$. It can be seen easily that $\alang(\fsa')$ is
non-empty iff $\alang(\fsa)\cap\alang(\asys)\neq\emptyset$. Note that $\fsa'$ is defined over one-letter alphabet and
$\size{\fsa'}=\size{\fsa}\times\size{\aschema}$. Now, from \cite[Proposition 8]{Vardi97}, we know that, checking non-emptiness of $\fsa'$ can be done
in time bounded by $\size{\fsa'}^2$. Hence, we can conclude that,
\begin{lemma}
MC(ABA,$UPKS$) is in \ptime.
\end{lemma}

For MC(ETL,$UPKS$), note that there exists a translation of any given ETL formula $\aformula$ to ABA $\fsa_\aformula$ such that the
the number of states in $\fsa_{\aformula}$ is quadratic in the size of $\aformula$ \cite{Piterman00}. But, the alphabet of $\fsa_{\aformula}$ is
exponential in the size of $\aformula$. Thus, to perform the translation in \ptime, we can only restrict the translation to the alphabets appearing in
the given $UPKS$. This gives us a polynomial size ABA $\fsa_{\aformula}$ in \ptime~and we can easily apply the method of MC(ABA,$UPKS$) to obtain a
\ptime~algorithm for MC(ETL,$UPKS$).

